TRIM: Reducing AI-Generated CodeSlop via Agent Trajectory Minimization

Coding agents are increasingly used to accelerate code generation in many downstream tasks, such as fixing bugs, building applications, and prototyping. However, despite their value as coding assistants, agent-generated code tends to be larger and more verbose than the corresponding human-written implementation. In this work, we show that the cause lies in the agent's own search process: while iterating toward a passing solution, an agent accumulates speculative edits, abandoned hypotheses, and temporary changes that persist into the final patch. This may seem harmless for a single patch, but the problem compounds as agents take responsibility for ever-larger portions of a codebase-a codebase that was once minimal and well-maintained slowly accumulates redundancy faster than it can be cleaned up, drifting to a state that is harder to maintain. Given the magnitude of this problem, we take a step towards alleviating this issue. First, we formally define this phenomenon as CodeSlop-the residual and functionally unnecessary edits commonly seen in AI-generated code. We then introduce our algorithm TRIM (Trajectory-guided Redundancy Identification and Minimization). Rather than minimizing CodeSlop directly, TRIM instead minimizes agent trajectories. As we show empirically, this indirect technique of minimizing CodeSlop is highly effective: TRIM cuts CodeSlop by 17.9%-32.9% across agentic scaffolds, with negligible performance regression. TRIM is also highly efficient, requiring roughly half the validation cost of algorithmic baselines such as Delta Debugging.

==> sections/Algorithms/backup/one_minimal.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{OneMinimal}}: Repeat reverse passes until fixpoint}
  \label{alg:oneminimal}
  \begin{algorithmic}[1]
    \REQUIRE $V$ (ordered sequence resolving the bug); $protectEnds$; $\mathcal{F}$; $\mathcal{R}$; $\mathcal{T}$
    \ENSURE $R \subseteq V$ that is 1-minimal: no single element is removable
    \STATE $R \gets V$
    \REPEAT
        \STATE $before \gets |R|$
        \STATE $R \gets$ \textsc{GreedyRemoval}($R$, $protectEnds$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \UNTIL{ $|R| = before$ } \% a full sweep dropped nothing: fixpoint reached \%
    \RETURN $R$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/final_algo.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{\algo}}: Hierarchical (three-level) Counterfactual Search to Minimize the Agent Patches}
  \label{alg:patchmin}
  \begin{algorithmic}[1]
    \REQUIRE $\mathcal{E} = \langle e_1, \ldots, e_{|\mathcal{E}|} \rangle$ (Edit sequence resolving the bug, each edit action $e_i$ contains edits made between consecutive feedback requests); $oneMin$ (guarantee 1-minimality?); $\mathcal{F}$ (feedback receiver); $\mathcal{R}$ (rule engine); $\mathcal{T}$ (truth table)
    % \ENSURE $\mathcal{MPE} \subseteq \mathcal{APE}=\textsc{Flatten}(NP)$, an order-preserved minimal edit set s.t. $\operatorname{len}(\mathcal{MPE}) < len(\mathcal{APE})$
    \ENSURE $\mathcal{MP}$ is an order-preserved minimal edit set; where $\operatorname{len}(\mathcal{MP}) < \operatorname{len}(\mathcal{AP})$. 
    \STATE \% Level 1: edit sequence-level minimization \%
    \STATE $S \gets$ \textsc{MinimumEditSequence}($\mathcal{E}$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \STATE $S \gets$ \textsc{Reduce}($S$, \textsc{true}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \STATE
    \STATE \% Level 2: file-level minimization \%
%    \STATE $E \gets$ \textsc{Flatten}($S$) \% flattened edit list of \textit{surviving} nodes
    \STATE $G \gets$ \textsc{GroupByFile}($S$) \% $G = \langle g_1, \ldots, g_k \rangle$, group list, one group per file
    \STATE $G \gets$ \textsc{Reduce}($G$, \textsc{false}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \STATE
    \STATE \% Level 3: edit-level minimization \%
    \STATE $E \gets$ \textsc{Flatten}($G$) \% order-preserved flattened list of \textit{surviving} edits
    \STATE $\mathcal{MPE} \gets$ \textsc{Reduce}($E$, \textsc{false}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \STATE $\mathcal{MP} \gets \operatorname{apply}(\mathcal{MPE}) $
    \RETURN $\mathcal{MP}$
  \end{algorithmic}
\end{algorithm}





% \begin{algorithm}[t]
%   \caption{\textbf{\emph{\algo}}: End-to-end three-level minimization of agent patches}
%   \label{alg:patchmin}
%   \begin{algorithmic}[1]
%     \REQUIRE $NP = \langle np_1, \ldots, np_{|NP|} \rangle$ (semantic node patch sequence resolving the bug, each $np_i$ contains edits made between consecutive feedback requests); $oneMin$ (guarantee 1-minimality?); $\mathcal{F}$ (feedback receiver); $\mathcal{R}$ (rule engine); $\mathcal{T}$ (truth table)
%     % \ENSURE $\mathcal{MPE} \subseteq \mathcal{APE}=\textsc{Flatten}(NP)$, an order-preserved minimal edit set s.t. $\operatorname{len}(\mathcal{MPE}) < len(\mathcal{APE})$
%     \ENSURE $\mathcal{MP}$ is an order-preserved minimal edit set; where $\mathcal{MP} = \operatorname{apply}(\mathcal{MPE})$, $\operatorname{len}(\mathcal{MP}) < \operatorname{len}(\mathcal{AP})$ \& $\mathcal{MPE} \subseteq \textsc{Flatten}(NP)=\mathcal{APE}$. 
%     \STATE \% Level 1: node-level minimization \%
%     \STATE $S \gets$ \textsc{MinimumNodeSuffix}($NP$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
%     \STATE $S \gets$ \textsc{Reduce}($S$, \textsc{true}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
%     \STATE
%     \STATE \% Level 2: file-level minimization \%
% %    \STATE $E \gets$ \textsc{Flatten}($S$) \% flattened edit list of \textit{surviving} nodes
%     \STATE $G \gets$ \textsc{GroupByFile}($S$) \% $G = \langle g_1, \ldots, g_k \rangle$, group list, one group per file
%     \STATE $G \gets$ \textsc{Reduce}($G$, \textsc{false}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
%     \STATE
%     \STATE \% Level 3: edit-level minimization \%
%     \STATE $E \gets$ \textsc{Flatten}($G$) \% order-preserved flattened list of \textit{surviving} edits
%     \STATE $\mathcal{MPE} \gets$ \textsc{Reduce}($E$, \textsc{false}, $oneMin$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
%     \STATE $\mathcal{MP} \gets \operatorname{apply}(\mathcal{MPE}) $
%     \RETURN $\mathcal{MP}$
%   \end{algorithmic}
% \end{algorithm}

==> sections/Algorithms/greedy_removal.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{GreedyRemoval}}: Single reverse pass dropping any removable element}
  \label{alg:greedy}
  \begin{algorithmic}[1]
    \REQUIRE $V=\langle x_1, \ldots, x_{|V|} \rangle$ (sequence of edits or semantic node patches); $protectEnds$ (keep $x_1$ and $x_{|V|}$?); $\mathcal{F}$ (feedback receiver) ; $\mathcal{R}$ (rule engine) ; $\mathcal{T}$ (truth table)
    \ENSURE $V_{best} \subseteq V$ and passes $TF$
    %, with no removable element
    \STATE $V_{best} \gets V$
    \IF{ $protectEnds$ }
        \STATE $high \gets |V|-1$;\quad $low \gets 2$ \% skip first and last
    \ELSE
        \STATE $high \gets |V|$;\quad\ \ $low \gets 1$
    \ENDIF
    \FOR{ $j = high$ \textbf{downto} $low$ }
        \STATE $V' \gets V_{best} \setminus \{x_j\}$ \% tentative drop, order preserved
        \IF{ $|V'| = 0$ }
            \STATE \textbf{break}
        \ENDIF
        \STATE $\mathcal{VE} \gets \textsc{Flatten}(V')$
        \STATE $\mathbf{FB} \gets$ \textsc{TryCandidate}($\mathcal{VE}$, $\mathcal{F}$)
        \IF{ $\mathbf{FB} \neq$ None }
            \STATE $(\mathcal{D}, \_) \gets \mathcal{R}(\mathbf{FB}, \_, \mathcal{T})$
            \IF{ $\mathcal{D} = $ \DROP{} }
                \STATE $V_{best} \gets V'$;
            \ENDIF
        \ENDIF
    \ENDFOR
    \RETURN $V_{best}$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/minimum_node_subsequence.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{MinimumNodeSubsequence}}: Drop intermediate nodes from the surviving suffix}
  \label{alg:minsubseq}
  \begin{algorithmic}[1]
    \REQUIRE $Q = \langle q_1, \ldots, q_{|Q|} \rangle$ (output of Alg.~\ref{alg:minsuffix}); $\mathcal{F}$ (feedback receiver); $\mathcal{R}$ (rule engine); $\mathcal{T}$ (truth table)
    \ENSURE $R \subseteq Q$ resolving the bug, where $R$ has no removable intermediate node
    \STATE $R \gets Q$, $L_{best} \gets len(Q)$
    \STATE \% the first ($q_1$) and last ($q_{|Q|}$) nodes aren't dropped \%
    \FOR{ $j = |Q|-1$ \textbf{downto} $2$ }
        \STATE \% Drop $q_j$ tentatively but preserve order \%
        \STATE $R' \gets R \setminus \{q_j\}$ 
        \STATE $\mathbf{FB} \gets$ \textsc{TryCandidate}($R'$, $\{q_j\}$, $\mathcal{F}$, $L_{best}$)
        \IF{ $\mathbf{FB} \neq$ None }
            \STATE $(\mathcal{D}, \_) \gets \mathcal{R}(\mathbf{FB}, \text{None}, \mathcal{T})$ 
            %\% $S_{best}=$ None: stop never fires \%
            \IF{ $\mathcal{D} = $ \DROP{} }
                \STATE $R \gets R'$
                \STATE $L_{best} \gets len(R)$ \% update the best length \%
            \ENDIF
        \ENDIF
    \ENDFOR
    \RETURN $R$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/minimum_suffix.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{MinimumNodeSuffix}}: Derive the smallest suffix of trajectory nodes satisfying certain properties}
  \label{alg:minsuffix}
  \begin{algorithmic}[1]
    \REQUIRE $NP = \langle np_1, \ldots, np_{|NP|} \rangle$ (semantic node patch sequence resolving the bug, each $np_i$ contains edits made between consecutive feedback requests); $\mathcal{F}$ (feedback receiver); $\mathcal{R}$ (rule engine); $\mathcal{T}$ (truth table)
    \ENSURE $NP_{best}$ is a suffix of semantic node patches that passes $TF$ and has smaller patch length
    \STATE $S_{best} \gets$ None, $k \gets |NP|$, $\mathcal{APE} \gets \textsc{Flatten}(NP)$
    \WHILE{ $k \geq 1$ }
        \STATE \% Get the last $|NP|-k+1$ nodes
        \STATE $S_k \gets \textsc{Flatten}(\langle p_k, p_{k+1}, \ldots, p_{|NP|} \rangle$) 
        \IF{ $S_k = \mathcal{APE}$ }
            \STATE break; \% Reached the whole patch sequence \%
        \ENDIF
        \STATE \% Test the subset  $S_k$ \%
        \STATE $\mathbf{FB} \gets$ \textsc{TryCandidate}($S_k$, $\mathcal{F}$)  
        \IF{ ($\mathbf{FB} \neq$ None) }
            \STATE $(\mathcal{D}, stop) \gets \mathcal{R}(\mathbf{FB}, S_{best}, \mathcal{T})$
            \IF{ $\mathcal{D} = $ \DROP{} }
                \STATE \% $S_k$ passes $TF$ and is a smaller patch
                \STATE $S_{best} \gets S_k$
            \ENDIF
            \IF{ ($stop$) }
                \STATE \% $\operatorname{len}(S_{k})>\operatorname{len}(S_{best})$, so break early
                \STATE \textbf{break}
            \ENDIF
        \ENDIF
        \STATE $k \gets k - 1$
    \ENDWHILE
    \STATE $NP_{best} \gets \operatorname{ReGroup}(S_{best})$ if $S_{best} \neq$ None, else $NP$
    \RETURN $NP_{best}$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/reduce.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{Reduce}}: One pass, or repeat until 1-minimal}
  \label{alg:reduce}
  \begin{algorithmic}[1]
    \REQUIRE $V$ (ordered sequence resolving the bug); $protectEnds$; $oneMin$; $\mathcal{F}$; $\mathcal{R}$; $\mathcal{T}$
    \ENSURE $R \subseteq V$ resolving the bug; 1-minimal if $oneMin$, else single-pass reduced
    \IF{ $\neg\, oneMin$ }
        \RETURN \textsc{GreedyRemoval}($V$, $protectEnds$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \ENDIF
    \STATE $R \gets V$
    \REPEAT
        \STATE $before \gets |R|$
        \STATE $R \gets$ \textsc{GreedyRemoval}($R$, $protectEnds$, $\mathcal{F}$, $\mathcal{R}$, $\mathcal{T}$)
    \UNTIL{ $|R| = before$ } \% a full sweep dropped nothing: fixpoint reached \%
    \RETURN $R$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/rule_engine.tex <==

\begin{table}[t]
\centering
\caption{$\mathcal{T}$: Truth table used by Rule Engine ($\mathcal{R}$) to output a decision ($\mathcal{D}$) for whether it is ``safe" to drop the edit / semantic node using $Obs_{Env}$ (runtime observation from $Env_{\operatorname{apply}(TF)}$) and $Obs_{patch}$ (patch observation from $Env_{patch}$)}
\label{tab:ruleengine}
\begin{tabular}{@{}llc cl@{}}
\toprule
\multicolumn{3}{c}{\textbf{Input}} & \multicolumn{2}{c}{\textbf{Output}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-5}
$Obs_{Env}$ & $Obs_{patch}$ & $S_{best}$ exists ? & $\mathcal{D}$ & stop \\
\midrule
\texttt{build failure} & ---              & ---           & \KEEP & \textsc{FALSE} \\
$TF$ \texttt{fails}  & ---              & ---           & \KEEP & \textsc{FALSE} \\
$TF$ \texttt{passes}    & $<L_{best}$ & ---           & \DROP & \textsc{FALSE} \\
$TF$ \texttt{passes}    & $>=L_{best}$  & \texttt{no}   & \KEEP & \textsc{FALSE} \\
$TF$ \texttt{passes}    & $>=L_{best}$  & \texttt{yes}  & \KEEP & \textsc{TRUE} \\
\bottomrule
\multicolumn{5}{l}{Rows evaluated top-to-bottom; first match wins; ``\texttt{---}" are don't-cares.}
\end{tabular}
% \vspace{-5mm}
\end{table}

% To Do 
% \alex{I need to check the simplifying assumption I made regarding dropping the phase column in Table \ref{tab:ruleengine}}


\begin{algorithm}[t]
  \caption{\textbf{RuleEngine ($\mathcal{R}$)}: Applies truth table $\mathcal{T}$ on Feedback $\mathcal{F}$}
  \label{alg:ruleengine}
  \begin{algorithmic}[1]
    \REQUIRE $\mathbf{FB}$ (aggregated feedback); $S_{best}$ (current best bug resolving patch sequence); $\mathcal{T}$ (a truth table like Table \ref{tab:ruleengine})
    % ; $L_{best}$ (current shortest patch)
    \ENSURE $(\mathcal{D}, stop)$; $\mathcal{D}\in\{\KEEP, \DROP\}$, $stop \in \{\textsc{true}, \textsc{false}\}$
    \STATE $Obs_{Env} \gets \mathbf{FB}.\text{runtime}$ \%$Env$ runtime feedback
    \STATE $Obs_{patch} \gets \mathbf{FB}.\text{patch}$ \%$Env_{patch}$ patch-length feedback 
    \STATE $(\mathcal{D}, stop) \gets$  Run $\mathcal{T}$ on $(Obs_{Env}, Obs_{patch}, S_{best})$
    \RETURN $(\mathcal{D}, stop)$
  \end{algorithmic}
\end{algorithm}

==> sections/Algorithms/try_candidate.tex <==
\begin{algorithm}[t]
  \caption{\textbf{\emph{TryCandidate}}: Validates a subset of edits}
  \label{alg:trycandidate}
  \begin{algorithmic}[1]
    \REQUIRE $S$ (candidate edit subset); $\mathcal{F}$ (feedback receiver)
    %; $E_{kernel}$ (kernel environment); $E_{patch}$ (patch environment)
    \ENSURE Aggregated feedback $\mathbf{FB} \in$ \{None\} 
    $\cup$ \{($Obs_{Env}$, $Obs_{patch}$) $\in$ $\mathcal{K} \times \mathcal{L}$  where $\mathcal{K}$ $\in$ \{build failure, $TF$-pass, $TF$-fail\} and $\mathcal{L} \in$ \{$< L_{best}$, $>= L_{best}$ \}\}; 
    \STATE $L_{best} \gets \operatorname{len}(S)$
    \IF{ $\neg$ applicable($S$) }
        \RETURN None \% return if patch is not applicable \%
    \ENDIF
    \STATE $\mathcal{MP} \gets$ $\operatorname{apply}(S)$
    % \STATE cleanRepo()
    \STATE \% collect feedback from all the environments \%
    % \STATE $(O_{kernel},O_{patch}) \gets \mathcal{F}(\Delta, S, S_{drop}, E_{kernel}, E_{patch})$ 
    \STATE $(Obs_{Env},Obs_{patch}) \gets \mathcal{F}(\mathcal{MP}, L_{best})$ 
    \STATE $\mathbf{FB}.runtime \gets Obs_{Env} $
    \STATE $\mathbf{FB}.patch \gets Obs_{patch} $
    \RETURN{$\mathbf{FB}$}
  \end{algorithmic}
\end{algorithm}

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

==> sections/backup/1_intro.tex <==
% =====================================================================
% Reducing AI-Generated CODE SLOP via Agent Trajectory Minimization
% Revised Introduction -- v2 (incorporates SlopCodeBench differentiation)
%
% Changes vs. v1 of this section:
%  (A) Novelty claim narrowed. SlopCodeBench (Orlanski et al., 2026) and a
%      surrounding cluster already "formalize" agent code slop as a static
%      quality property. We now claim only what survives: (i) defining slop
%      as *removable functional redundancy within a single patch* and
%      (ii) the first *removal* algorithm that preserves test-defined
%      correctness.
%  (B) Added an explicit static-quality vs. functional-redundancy
%      distinction (the orthogonality), separating us from the
%      verbosity/erosion line of work, not just from NLP "slop".
%  (C) Wired the SlopCodeBench prompt-intervention finding into the
%      "why deterministic" beat: quality-aware prompting lowers initial
%      quality but neither halts degradation nor is free (higher cost,
%      lower correctness).
%  (D) Replaced placeholder citations: review-burden cluster
%      (nakashima2026reject, asdaque2026overhead, watanabe2026cut) and the
%      LLM-verbosity cluster (dou2026wrong, abbassi2025taxonomy).
%  (E) Added a footnote acknowledging the SlopCodeBench naming collision.
%
% OPEN DECISION (authors): given a benchmark literally named SlopCodeBench
% that defines "slop" as redundant code, consider renaming CODE SLOP to a
% term that foregrounds *removability* (e.g., "patch residue" / "residual
% edits"). The footnote below is a stopgap if the name is kept.
%
% TODO(authors): the \cite{} key PLACEHOLDER_ai_code_share still needs a
% real source. All other new keys have bib entries at the bottom of this
% file (commented) -- paste them into your .bib.
% =====================================================================

\section{Introduction}
\label{sec:intro}

Modern coding agents are rapidly transforming software development. They can navigate repositories, write code, run tests, and iteratively repair failures, increasingly producing working patches with little human intervention. As these systems become more capable, the challenge is no longer simply generating correct code, but understanding and maintaining it afterward~\cite{roychoudhury2026agentic}. 
Yet most work on coding agents focuses on a single question:
\textit{Does the patch pass the tests?} However, test passing alone says
little about the quality of the resulting patch---developers must still
review, understand, and maintain the generated changes.

%developers still need to review, understand, and
%maintain the generated changes, making patch quality just as important as
%functional correctness.

%Yet most work on coding agents focuses on a single question: \textit{Does the patch pass the tests?} 
%Far less attention has been paid to an equally important one: 
%\textit{What does the resulting patch actually look like?}\junfeng{look like sound too vague} \alex{ray, not sure how to address this}

This question matters because many agent-generated patches appear substantially larger than necessary~\cite{ceka2025understanding}. Maintainers increasingly report spending additional effort reviewing, simplifying, and often rejecting such patches before they can be merged~\cite{nakashima2026agentic,asdaque2026novice}. We investigate this problem in the context of program repair---one of the widely studied and mature workloads for coding agents---where agents iteratively modify code and validate their changes through testing. This setting provides a natural lens for studying how unnecessary changes accumulate during the search for a successful fix.

When we examined these repair trajectories, one pattern stood out. Agents often arrive at a correct fix only after a sequence of edits, test executions, and revisions.
% \franjo{should we explicitly mention that this may be due to trying out different hypothesis to figure out a root cause?} 
% \alex{Mentioned later}
This iterative behavior is entirely expected and well studied~\cite{kim2026trajeval, xiao2025trajectory}. What surprised us was what happened after the fix was found. Once a passing solution is reached, agents rarely remove the exploratory changes that helped them get there. As such, traces of the search process  remain embedded in the final patch alongside the modifications that actually resolve the defect.


Figure~\ref{fig:kernel_motivating_example} illustrates this phenomenon. When resolving a Linux kernel vulnerability \cite{mem_leak}, \swe \cite{yang2024swe} produces 21 modified lines across three feedback cycles, yet \textit{only three} of those lines are required for the fix. The remaining changes are remnants of the search process---speculative edits, abandoned hypotheses, and temporary modifications that persist simply because the agent has no reason to remove them once a passing solution is found. Interestingly, these three lines happen to coincide with the ground-truth human patch, although our approach does not assume such a reference implementation is available. We refer to these residual search artifacts that survive into the final patch as \emph{\aislop}.

The problem is not simply that agent-generated patches are larger. It is that \aislop obscures the change that actually matters. As a result, developers spend more effort reviewing patches, understanding root causes, and maintaining the resulting code~\cite{watanabe2026cut,nakashima2026agentic}. Moreover, the motivating example is not an isolated incident. Across our benchmarks, we find that agent-generated patches routinely contain substantial amounts of \aislop, consistent with recent reports that AI-generated code is often more verbose~\cite{orlanski2026slop,dou2026wrong} and accumulates redundancy faster than human-written code~\cite{he2025speed, ehsani2026faster}.

\textbf{\textit{Key Insight.}} Reasoning about the phenomenon above requires a notion of slop that goes beyond traditional code quality metrics. A change may be perfectly readable, well-structured, and free of duplication, yet still be unnecessary for resolving the task. What matters is not whether the retained code appears verbose or complex, but whether portions of the patch can be removed entirely while preserving correctness. This perspective differs from prior work, which characterizes slop primarily through static properties of the resulting code artifact, such as verbosity, redundancy, or the accumulation of complexity over time~\cite{orlanski2026slop,dou2026wrong,abbassi2025taxonomy}. We instead define \aislop as \emph{removable functional redundancy}: changes that arise during an agent's search process but are ultimately unnecessary for the final solution for task $T$. 
%\alex{mention that this is with respect to a task T}. 
Under this definition, identifying \aislop requires reasoning about the agent's trajectory and validating candidate removals through execution, rather than analyzing the final code artifact in isolation. To our knowledge, this is the first work to formalize and systematically remove such redundancy from agent patches.
%\franjo{I think we may want to change the absolute view on "functional redundancy" and instead make it more relative to the bug being addressed. As a simple example, adding a log statement isnt necessarily functionally redundant: it provides additional observability and forensic capabilities in the future. However, it may be unnecessary for this particular bug. So maybe it should be functional redundancy with respect to fixing a particualr bug minimally.}
% \alex{addressed}

\aislop\ also introduces a fundamentally different minimization problem.
Traditional techniques such as Delta Debugging~\cite{10.1145/318774.318946}
and \texttt{git-bisect}~\cite{git_bisect} search \emph{across} versions or
commits to identify failure-inducing changes. These histories are typically
authored by developers and therefore reflect relatively clean, intentional
evolution. In contrast, \aislop\ arises \emph{within} a single
agent-generated patch, which often contains exploratory edits accumulated
during the repair process. The objective is therefore not to localize the
cause of a failure, but to identify the minimal subset of edits required to
preserve the successful repair.

% \aislop also gives rise to a new minimization problem. Traditional techniques such as 
% Delta Debugging~\cite{10.1145/318774.318946} and \texttt{git-bisect}~\cite{git_bisect} reason \textit{across} versions or commits. \alex{Developer commits also tend to be leaner than agent commits, as they are not polluted with code changes made during the developers' debugging process. Hence, these works search over a ``cleaner" linear history.}
% \junfeng{need to explain more here. developer commits don't have the exploratory codeslops -- they are removed already by the developers, so the commits that delta debugging works with often form a clean linear history} 
% In contrast, \aislop arises \textit{within} a single agent patch, where the goal is not to
% identify what caused a failure, but to determine which changes are actually necessary for the fix.

% \textbf{\textit{Challenges.}} Defining \textsc{Code Slop} is only the first step; determining which edits are actually redundant is substantially harder. Unlike traditional code-quality issues, \textsc{Code Slop} is inherently a \emph{counterfactual} property. Once a patch passes its tests, both necessary edits and residual search artifacts appear equally valid. Determining whether an edit is truly slop requires \emph{causal reasoning} about what would happen if that edit were removed, while accounting for dependencies among edits and preserving the behavior of the original solution.

\textbf{\textit{Challenges.}} Defining \aislop is only the first step; identifying it is substantially harder. Once a patch passes its tests, both essential changes and residual search artifacts appear equally successful. As a result, \aislop cannot be identified reliably from the final patch alone. The problem is further complicated by dependencies among changes, where the necessity of one modification may depend on the presence of others. This challenge is difficult even for state-of-the-art coding agents. While agents can generate successful patches, they are not explicitly trained to determine the minimal set of changes required for a solution. We validate this notion by running agent-driven patch minimization experiments and observe that agents are very
%Consequently, we find agent-driven patch minimization\junfeng{unclear what this means} to be surprisingly 
unreliable: in $17.5\%$--$44.9\%$ of cases, the resulting patch either fails to preserve the behavior of the original solution or is larger in size than the original.

\textbf{\textit{Methodology.}} 
To address this challenge, we formulate \aislop\ identification as a
counterfactual search problem over the agent's \emph{repair trajectory},
rather than over the final patch alone. Traditional minimization techniques,
such as Delta Debugging, implicitly assume a relatively clean, linear change
history in which candidate changes can be explored largely independently. In
contrast, an agent's repair trajectory records an exploratory debugging
process: edits are proposed, refined, reverted, and superseded by later
repair hypotheses, creating rich dependencies among changes. Rather than
searching over individual patch fragments, \algo\ exploits this structure by
organizing the search hierarchically according to the repair trajectory,
progressively refining from coarse repair hypotheses to finer-grained
changes. Candidate removals are validated through execution, producing a
minimal patch that preserves the behavior of the original repair while
eliminating artifacts of the agent's search process.

% \textbf{\textit{Methodology.}} To address this challenge, we formulate \aislop identification as a counterfactual reasoning problem. Determining whether a change is redundant requires reasoning about what would happen if that change were removed,
% %\junfeng{this sounds a lot like delta debugging formulation?} 
% % \alex{it is a form of hierarchical delta debugging using trajectory groupings}
% while accounting for dependencies among changes and preserving the behavior of the original solution. This observation suggests that \aislop cannot be reliably identified through static inspection alone, nor by simply asking an agent to revise its own patch. Instead, it requires systematically exploring alternative patch variants and validating them through execution. Guided by this insight, we develop a framework that automatically removes \aislop from successful agent-generated patches. Our approach progressively eliminates candidate changes while continuously validating behavioral equivalence, thus producing a smaller patch that preserves the functionality of the original solution while removing artifacts of the search process.\junfeng{need to talk a little bit about delta debugging assumes linear history of commits, where agent exploratory changes form DAG etc. also, need to explain the high-level algorithm of our system and what's new in it.} \alex{Ray, this paragraph is missing the point that we do minimization in the trajectory action space. Correctly pointed out by Junfeng. We may need to introduce the concept of trajectory here. This way Franjo's comment below will also get addressed.}



\textbf{\textit{Results.}} We evaluate our approach across four agent scaffolds (\crashfixer, \swe, \mini, and \openhands) on Live-kBench \cite{huang2026outrunningllmcutoffslive} and \textsc{Swe-Bench}\cite{jimenez2023swe}. Our approach reduces patch size by $17.3\%$--$32.9\%$, achieving a $1.6$$\times$--$2.8$$\times$ improvement over agent-based minimization baselines while introducing negligible regressions in correctness. For scaffolds run in assisted settings (access to buggy files), it also increases agreement with human-written patches.


In summary, this paper makes the following contributions:

\begin{itemize}
\item We introduce \emph{\textsc{Code Slop}}, a new formulation of removable functional redundancy in agent-generated patches.


%\item We propose \emph{\textsc{Patch Minimize}}, a reference-free objective for minimizing agent-generated patches.

\item We develop \algo, a trajectory-aware algorithm for removing unnecessary edits while preserving correctness.\franjo{I think we need to say something about what we mean by trajectory here.} \alex{Will get addressed if we add that trajectory part to the above methodology para.}

\item We empirically show that substantial amounts of \textsc{Code Slop} can be removed from agent-generated patches across multiple agents and benchmarks.


\end{itemize}


% The term ``slop'' has been used in two prior senses that we are careful to
% separate from ours. In the NLP community it characterizes low-quality,
% verbose, or stylistically degraded AI-generated \emph{text}~\cite{shaib2025slop}.
% More relevant to us, a growing line of software-engineering work studies the
% \emph{quality degradation} of agent-generated code --- redundant
% constructions, duplication, and the concentration of complexity in
% already-complex functions --- and shows that these properties worsen as
% agents extend their own code over long
% horizons~\cite{orlanski2026slop,dou2026wrong,abbassi2025taxonomy}. That work
% characterizes slop as a \emph{static quality property of the code an agent
% retains}: verbose or over-complex code that nonetheless still performs work,
% and that is measured directly on the surviving source. Our notion is
% orthogonal. \textsc{Code Slop} is \emph{functional redundancy} --- edits that
% can be removed \emph{in their entirety} while the patch still passes its
% tests --- and it is a \emph{structural artifact of the agent's search
% trajectory} rather than a stylistic property of any one line. The two are
% genuinely different: a removable edit may be perfectly clean code (so static
% quality metrics would never flag it), while an eroded but irreducible
% function is not removable at all. Crucially, identifying removable edits
% cannot be done by inspecting the final code statically; it requires the
% agent's trajectory together with runtime validation. To our knowledge, we
% are the first to formalize slop as removable functional redundancy within a
% single agent patch, and the first to propose algorithms that \emph{remove}
% it while preserving test-defined correctness.

% Addressing \textsc{Code Slop} is also fundamentally different from
% traditional software minimization problems. Existing techniques such as Delta
% Debugging \cite{10.1145/318774.318946} and \texttt{git-bisect} \cite{git_bisect}
% operate across program versions, commits, or configurations --- designed to
% isolate failure-inducing changes in human-authored histories. \textsc{Code
% Slop}, by contrast, originates \emph{within} a single agent-generated patch.
% Unlike human-authored commits, which typically expose only the final
% implementation, agent trajectories preserve the full sequence of intermediate
% edits, failed attempts, and validation steps that produced the final
% solution. This trajectory structure provides a unique opportunity to reason
% about the causal relationship between the agent's search process and the
% final patch --- one that version-history methods cannot exploit.

% In this paper, we formalize \textsc{Code Slop} and introduce
% \emph{\textsc{Patch Minimize}} --- a benchmark-independent objective that
% seeks the smallest subset of an agent patch preserving task correctness.
% Because the human-patch length is a constant, this objective shares its
% optimum with \textsc{Code Slop} minimization (a duality we make precise in
% \S\ref{subsec:problem_formulation}); the practical consequence is that \textsc{Patch
% Minimize} never references a human-written reference and so applies directly
% in the blind settings that arise whenever a user interacts with an agent.
% Building on this formulation, we present \textsc{TrajMinimize}, a
% trajectory-aware minimization framework that constructs a hierarchical
% representation of the agent's execution trace and progressively removes
% unnecessary edits at the semantic-node, file, and edit levels, using runtime
% feedback to preserve the agent's own test-defined correctness throughout.
% A natural alternative is to ask the agent to clean up its own patch, but this
% is unreliable: prompting an agent to minimize its patch fails one of our
% validity criteria on 17.5\%--44.9\% of instances (\S\ref{sec:rq1}), and even
% quality-aware prompting, while it lowers the \emph{initial} verbosity of
% agent code, neither halts the underlying degradation nor comes for free,
% raising per-checkpoint cost and reducing
% correctness~\cite{orlanski2026slop}. This motivates a deterministic,
% trajectory-grounded removal pass that is applied \emph{after} the agent
% succeeds and is verified by execution rather than by prompting. We evaluate
% \textsc{TrajMinimize} across four agent scaffolds (\textsc{CrashFixer},
% \textsc{Swe-Agent}, \textsc{MiniSwe-Agent}, \textsc{OpenHands}) on
% Live-kBench and \textsc{Swe-Bench}. At the edit level, \textsc{TrajMinimize}
% achieves a 17.3\%--29.3\% per-scaffold patch size reduction --- a
% 1.6$\times$--2.6$\times$ improvement over agentic minimization baselines ---
% with negligible oracle regressions and, in assisted settings, measurable
% gains in human-patch equivalence rate.

% In summary, this paper makes the following contributions:
% \begin{itemize}
%   \item We identify and formalize \emph{\textsc{Code Slop}} as
%   \emph{removable functional redundancy within a single agent patch},
%   distinguishing it both from slop in natural language
%   generation~\cite{shaib2025slop} and from the static code-quality
%   degradation (verbosity, structural erosion) studied in recent
%   agent-coding work~\cite{orlanski2026slop,dou2026wrong,abbassi2025taxonomy}.
%   To our knowledge, we are the first to target slop \emph{removal} rather
%   than only its measurement.

%   \item We introduce \emph{\textsc{Patch Minimize}}, a benchmark-independent
%   formulation for minimizing AI-generated patches, and show that it shares
%   its optimum with \textsc{Code Slop} minimization --- a duality that, by
%   removing any dependence on a human reference, makes the objective
%   applicable to blind settings.

%   \item We present \textsc{TrajMinimize}, a trajectory-aware minimization
%   algorithm that progressively removes unnecessary edits using runtime
%   feedback while preserving test-defined correctness, and analyze its cost
%   complexity. We further show that the obvious agentic alternative ---
%   asking the model to minimize its own patch --- is unreliable, motivating
%   our deterministic design.

%   \item We demonstrate empirically that agent trajectories contain
%   sufficient structural information to substantially reduce patch verbosity
%   while preserving functional correctness across scaffolds and benchmarks.
% \end{itemize}



==> sections/backup/2_motiv.tex <==
\section{Motivating Example} % \& Problem Formulation}
\label{sec:motiv}

In this section, we use a real-world repair trajectory to illustrate how
\aislop\ emerges during agent-driven program repair.
Figure~\ref{fig:kernel_motivating_example} shows the trajectory and final
patch generated by \swe~\cite{yang2024swe} while repairing a Linux kernel
memory leak vulnerability~\cite{mem_leak} caused by an \texttt{if} branch
that fails to free a \texttt{map} structure.

Now consider a developer reviewing the patch in Figure~\ref{fig:kernel_motivating_example} (right). It modifies a single file, \texttt{kernel/bpf/syscall.c}, but changes $21$ lines across five hunks: (1) a block of code is relocated $15$ lines down (this change spans two hunks), (2) a call to a memory-deallocation routine is deleted on Lines $1363,1615$ and added on line $1617$, and (3) \texttt{goto} statements are inserted at three disparate locations. The patch passes the crash-reproducing test, so by construction it resolves the vulnerability. 
But passing the test is only the beginning of the developer's
task. Every modified line demands attention: the developer must understand
what each change does, why it was introduced, and whether it interacts with
the rest of the patch. Consequently, unnecessary edits 
increase the cognitive effort required to review and maintain the repair.

%But passing is not the developer's only concern. To review, understand, and ultimately trust the change, the developer must answer a more basic question: which of these $21$ lines actually fix the bug? From the agent's perspective, all the modified lines made before the final success led to the successful solution. But $\ldots$ the developer knows better.

We tried to reason about how these unnecessary lines are inserted by the agent; we looked into the agent trajectory (Figure~\ref{fig:kernel_motivating_example} left) and found that  
the agent doesn't discover the fix immediately. Instead, it progresses through three rounds of edit sequences ($\mathcal{E}_{1}$, $\mathcal{E}_{2}$, and $\mathcal{E}_{3}$), each followed by validation through test execution. The first two rounds ($\mathcal{E}_{1}$ and $\mathcal{E}_{2}$) fail validation, prompting further modifications, while the third round ($\mathcal{E}_{3}$) ultimately passes all tests. %We notice a 
~\Cref{fig:kernel_motivating_example} shows the map between the agent edits in the trajectory and the final cumulative patch (marked by bounding boxes).  The %purple/gold 
%bounding boxes indicate which lines originated from $\mathcal{E}_{1}$, $\mathcal{E}_{2}$, and $\mathcal{E}_{3}$.  
More specifically, $\mathcal{E}_{1}$---an edit sequence with a single edit ($e_{11}$), moves a block of code down $15$ lines. $\mathcal{E}_{2}$---containing a single edit ($e_{21}$), removes a call to a memory de-allocation function on Line $1363$. Finally, $\mathcal{E}_{3}$---a sequence of three edit actions ($e_{31}$,$e_{32}$,$e_{33}$), adds ``\texttt{go to}" statements to a memory de-allocation function at three disparate locations.

At first glance, all of these changes appear equally important because they coexist in the final passing patch. However, a closer inspection reveals a striking observation: only the starred region, corresponding to edit $e_{31}$ from sequence $\mathcal{E}_{3}$, is actually required to resolve the vulnerability and matches the human-written fix. The remaining modifications neither contribute to the fix nor affect correctness, yet they persist in the patch because the agent has no incentive to remove them once a passing solution is found. As mentioned earlier, we refer to these residual code changes as \aislop. 

%, one of which ($e_{31}$) is the actual solution to this vulnerability. The code changes caused by $e_{31}$ are also equivalent to the human fix. 
%\franjo{Could you add a bit of info about the three edits and how they relate to the bug (either here or in the next para)? For example, I looked at e1 and initially was very confused because the deleted code and the added code are identical. it took me a bit to understand that the code was moved by some 15 lines. Lets make it easier for the reader to follow along. } 
% Figure~\ref{fig:kernel_motivating_example} also shows the final agent-generated patch.\franjo{Does it?}
%\junfeng{agreed. the example needs more concrete details for people to get the intuitions. you want to actually show the lines. if space is a problem simply the code}
% This example reveals an important limitation of agent-generated patches. Although the agent eventually succeeds, the trajectory alone does not tell us which modifications were actually responsible for fixing the vulnerability. From the agent's perspective, all edits made before the final \texttt{PASS} lead to the successful solution.


\begin{figure}[t]
\centering

\begin{subfigure}{0.95\linewidth}
  \centering
  \includegraphics[width=\linewidth]{images/coherent_trajectory_figure_7.pdf}
  \caption{Linux vulnerability~\cite{mem_leak}; here the human patch is edit $e_{31}$.}
  \label{fig:kernel_motivating_example}
\end{subfigure}

\vspace{1.5mm}

\begin{subfigure}{0.95\linewidth}
  \centering
  \includegraphics[width=\linewidth]{images/coherent_trajectory_sympy_5.pdf}
  \caption{SWE-Bench \texttt{sympy\_\_sympy-15017}.
  %: \texttt{len()} of a rank-0 array returns $0$ instead of $1$. 
  The agent patch spans three files and five hunks, yet the true fix is a single
  line ($e_{11}$); \algo eliminates two files and prunes the patch down to that one edit,
  identical to the human fix.}
  \label{fig:sympy_motivating_example}

\vspace{-2mm}
\end{subfigure}

\caption{Two motivating examples of \aislop. \algo recovers the human-equivalent fix hidden inside a
larger agent patch. In each, edits in the trajectory map to regions of the final patch.
The starred region ($\star$) is the human patch, while the purple-bordered regions are
\aislop---residual edits from the agent's search process that \algo prunes away.}
\label{fig:motivating_examples}
\vspace{-4mm}
\end{figure}

%Figure~\ref{fig:kernel_motivating_example} (right) provides a closer look at the resulting patch. 
% To visualize the relationship between the trajectory and the final patch, we map each round of edits (left) to the corresponding modified regions in the code (right). 


\textbf{Trajectory-Guided Search.} One way to answer the developer's question is to enumerate over the $2^5 = 32$ plausible subsets of the five-hunk patch, with the hope of finding the minimal code changes within a reasonable amount of time. However, as we show in this paper, we can do better than a \textit{blind} hunk-subset search. By leveraging the inherent structure of this trajectory, \algo finds the optimal hunk in three steps---it first applies the code changes from the last edit sequence $\mathcal{E}_3$ and validates its correctness. It then systematically removes the code changes from edits $e_{33}$ and $e_{32}$, leaving the final ground-truth edit $e_{31}$. As each validation call for a Linux kernel wastes $30$ minutes (on a very high-compute machine), this reduction in validation attempts makes a substantial impact.

\alex{Ray, how to bridge now ?}

%\shobini{I think the previous sentence was already defined in an earlier paragraph, not sure if restating here was intentional. Also, the term "residual search artifacts" was confusing for me because in the traj reconstruction section, we talk about removing actions like "repository search" (which is really a type of residual search artifact)} 
While the human patch serves as a useful illustration in this example, in reality, such a reference is not available. As coding agents become responsible for an increasing fraction of software development, understanding and eliminating such \aislop will be critical for producing patches that remain understandable, reviewable, and maintainable by developers. \junfeng{the example needs to illustrate (1) code slop from exploratory agent attempts; (2) why delta debugging won't work; (3) why trajectory minimization is important / how our approach works. that is, the example needs to drive home the contributions.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BACK UP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we illustrate with a real-world motivating example how \aislop emerges during agent-driven program repair. Consider the repair trajectory (Figure~\ref{fig:kernel_motivating_example} left) and the resulting patch (Figure~\ref{fig:kernel_motivating_example} right) generated by \swe~\cite{yang2024swe} for a Linux kernel vulnerability~\cite{mem_leak}. 
% The associated crash-triggering script leaks memory by exercising an \texttt{if} block that fails to free a \texttt{map} structure.
% %The crash-triggering script causes a memory leak because it runs specific inputs that execute an \texttt{if} block which is missing code to free a \texttt{map} structure. % ~\rayb{can you give one line description of the vulnerability} % \franjo{Maybe even more than a one-liner}. 
% As evident by the agent trajectory (Figure~\ref{fig:kernel_motivating_example} left), the agent doesn't discover the fix immediately. Instead, it progresses through three rounds of edit sequences ($\mathcal{E}_{1}$, $\mathcal{E}_{2}$, and $\mathcal{E}_{3}$), each followed by validation through test execution. The first two rounds ($\mathcal{E}_{1}$ and $\mathcal{E}_{2}$) fail validation, prompting further modifications, while the third round ($\mathcal{E}_{3}$) ultimately passes all tests. 
% %, one of which ($e_{31}$) is the actual solution to this vulnerability. The code changes caused by $e_{31}$ are also equivalent to the human fix. 
% %\franjo{Could you add a bit of info about the three edits and how they relate to the bug (either here or in the next para)? For example, I looked at e1 and initially was very confused because the deleted code and the added code are identical. it took me a bit to understand that the code was moved by some 15 lines. Lets make it easier for the reader to follow along. } 
% % Figure~\ref{fig:kernel_motivating_example} also shows the final agent-generated patch.\franjo{Does it?}
% %\junfeng{agreed. the example needs more concrete details for people to get the intuitions. you want to actually show the lines. if space is a problem simply the code}
% This example reveals an important limitation of agent-generated patches. Although the agent eventually succeeds, the trajectory alone does not tell us which modifications were actually responsible for fixing the vulnerability. From the agent's perspective, all edits made before the final \texttt{PASS} lead to the successful solution.


% \begin{figure}[t]
% \centering

% \begin{subfigure}{0.95\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/coherent_trajectory_figure_4.pdf}
%   \caption{Linux vulnerability~\cite{mem_leak}; here the human patch is edit $e_{31}$.}
%   \label{fig:kernel_motivating_example}
% \end{subfigure}

% \vspace{1.5mm}

% \begin{subfigure}{0.95\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/coherent_trajectory_sympy_3.pdf}
%   \caption{SWE-Bench \texttt{sympy\_\_sympy-15017}.
%   %: \texttt{len()} of a rank-0 array returns $0$ instead of $1$. 
%   The agent patch spans three files and five hunks, yet the true fix is a single
%   line ($e_{11}$); \algo eliminates two files and prunes the patch down to that one edit,
%   identical to the human fix.}
%   \label{fig:sympy_motivating_example}

% \vspace{-2mm}
% \end{subfigure}

% \caption{Two motivating examples where \algo recovers the human-equivalent fix hidden inside a
% larger agent patch. In each, edits in the trajectory (left) map to regions of the final patch
% (right): the starred region ($\star$) is the human patch, while the purple-bordered regions are
% \aislop---residual edits from the agent's search process that \algo prunes away.}
% \label{fig:motivating_examples}
% \vspace{-4mm}
% \end{figure}

% Figure~\ref{fig:kernel_motivating_example} (right) provides a closer look at the resulting patch. To visualize the relationship between the trajectory and the final patch, we map each round of edits (left) to the corresponding modified regions in the code (right). The purple/gold bounding boxes indicate which lines originated from $\mathcal{E}_{1}$, $\mathcal{E}_{2}$, and $\mathcal{E}_{3}$. \alex{Added more descriptions now.}
% More specifically, $\mathcal{E}_{1}$---an edit sequence with a single edit ($e_{11}$), moves a block of code down $15$ lines. $\mathcal{E}_{2}$---containing a single edit ($e_{21}$), removes a call to a memory de-allocation function on Line $1363$. Finally, $\mathcal{E}_{3}$---a sequence of three edit actions ($e_{31}$-$e_{33}$), adds ``\texttt{go to}" statements to a memory de-allocation function at three disparate locations.
% At first glance, all of these changes appear equally important because they coexist in the final passing patch. However, a closer inspection reveals a striking observation: only the starred region, corresponding to edit $e_{31}$ from sequence $\mathcal{E}_{3}$, is actually required to resolve the vulnerability and matches the human-written fix. The remaining modifications neither contribute to the fix nor affect correctness, yet they persist in the patch because the agent has no incentive to remove them once a passing solution is found.

% We refer to these residual code changes as \aislop. %\shobini{I think the previous sentence was already defined in an earlier paragraph, not sure if restating here was intentional. Also, the term "residual search artifacts" was confusing for me because in the traj reconstruction section, we talk about removing actions like "repository search" (which is really a type of residual search artifact)} 
% While the human patch serves as a useful illustration in this example, in reality, such a reference is not available. As coding agents become responsible for an increasing fraction of software development, understanding and eliminating such \aislop will be critical for producing patches that remain understandable, reviewable, and maintainable by developers.
% \alex{Ray, can we add a line saying blindly trying all combinations of hunks would be too slow? How to show a problem in DD-Hunk in this example? Like what Junfeng says below.}
% \junfeng{the example needs to illustrate (1) code slop from exploratory agent attempts; (2) why delta debugging won't work; (3) why trajectory minimization is important / how our approach works. that is, the example needs to drive home the contributions.}

==> sections/backup/4_method.tex <==
\section{Methodology}
\label{sec:method}

% In this section, we deep dive into our end-to-end minimization system. We start with a high-level overview (\S\ref{subsec:system_overview}) of our algorithm, \algo. We then elaborate on each system component, including data pre-processing and the \algo algorithm. Finally, we end with a theoretical analysis of two variants of \algo. 

% Section~\ref{sec:problem_formulation} formulates Patch Minimization as an optimization problem whose solution is the minimal behavior-preserving patch $\mathcal{AP}^*$. 
This section presents \algo, an approximation algorithm for Patch Minimization. We start with a high-level overview (\S\ref{subsec:system_overview}) of the algorithm. We then elaborate on each of its components in the rest of the section.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{images/system-overview-30th-June.pdf}
  \caption{Overview of \algo. ~\protect\blackcircled{0} An agent fixes a bug and emits a patch and a trajectory---a sequence of actions like searching code, editing code, and running test files via feedback requests ($FR$) to receive \texttt{pass}/\texttt{fail} observations. 
  ~\protect\blackcircled{1} We preprocess the trajectory to keep only the edits and feedback requests, discarding the rest---resulting in a list of edits ($e_1,\dots,e_5$) separated by $FR$s. 
  We then create ``edit sequences" by grouping edits made between consecutive $FR$s (shown as $\mathcal{E}_1$-$\mathcal{E}_3$), to derive a structured search space $Traj_R$ (for our motivating example in \S\ref{sec:motiv}). 
  ~\protect\blackcircled{2} \algo then progressively minimizes the patch, first dropping edit sequences, then files, and finally single edits---~\protect\blackcircled{3} accepting a drop only if the candidate patch passes the test and has a shorter patch length. 
  We draw the agent patch as a stack of changed lines: the orange line is the fix, and the gray lines are unrelated edits (\aislop) that are dropped until only the fix remains. 
  ~\protect\blackcircled{4} The minimized patch is then evaluated against hidden tests (semantic check) and, optionally, checked for equivalence to the human patch.
  %Section~\ref{sec:expr} reports \patchdiff and how often this match occurs. 
  %The $Traj_R$ corresponds to our motivating example in Figures~\ref{fig:agent_traj} and ~\ref{fig:motiv_fig}.
  }
  \label{fig:system_overview}
\vspace{-5mm}
\end{figure*}

\subsection{System Overview}
\label{subsec:system_overview}


As formulated in Section~\ref{sec:problem_formulation},
\patchmin\ seeks to recover the minimal behavior-preserving patch
$\mathcal{AP}^*$. Solving this optimization exactly, requires searching over an
exponential number of candidate patches (for a patch of length $n$, the candidate patches can be $2^n$) and is therefore computationally
intractable.



% We observe that \patchmin\ can be viewed as a
% \emph{counterfactual reasoning} problem. Determining whether a modification is
% necessary requires asking: \emph{What would happen if this modification had
% never been made?} In principle, answering this question requires evaluating an
% exponential number of counterfactual patches---for a patch of length $n$, the number of counterfactual patches can be $2^n$. \alex{Baishkahi, the last line of the first para and last line of this para read similar to me}


We observe that \patchmin\ can be viewed as a
\emph{counterfactual reasoning} problem. Determining whether a modification is
necessary requires asking: \emph{What would happen if this modification had never been made (i.e., a counterfactual patch)?} 
Each such question corresponds to evaluating a
counterfactual patch obtained by removing one or more modifications from the original agent-generated patch 
% \shobini{Should we more clearly introduce what is meant by counterfactual since it's used so much later throughout the paper?}. 
% \alex{solved}
The challenge is that these counterfactuals are
not independent---the necessity of one modification may depend on the presence
or absence of others.


\emph{Our key insight} is that the agent's trajectory provides a natural
structure for exploring these dependent counterfactuals. Rather than
considering arbitrary subsets of modifications, we exploit the fact that every
modification was introduced as part of the agent's iterative edit-and-feedback
process. Modifications introduced together %\alex{before a test?} 
often represent a single repair
hypothesis and therefore exhibit strong dependencies. 
To this end, we introduce \algo\ (\textbf{T}rajectory-guided \textbf{R}edundancy \textbf{I}dentification and \textbf{M}inimization), which systematically
revisits this trajectory, progressively constructing counterfactual patches by
removing groups of related modifications and validating whether the resulting
patch still satisfies the task. By leveraging the trajectory to guide the
search, \algo\ efficiently approximates the minimal behavior-preserving patch
without exhaustively enumerating all candidate subsets.

At a high level, \algo consists of three steps (see~\Cref{fig:system_overview}):


\noindent\protect\blackcircled{1}~\textit{Trajectory-derived search space construction.} Starting from the agent's execution trajectory, \algo reconstructs the modifications that contribute to the final patch, removes trajectory actions that do not affect the patch, and organizes the remaining modifications into a hierarchical search space that captures their temporal and semantic dependencies.

\noindent\protect\blackcircled{2}~\textit{Hierarchical counterfactual search.} \textsc{TRIM} explores the trajectory-derived search space from coarse to fine-grained modification groups, iteratively constructing candidate counterfactual patches by un-doing related modifications. 

\noindent\protect\blackcircled{3}~\textit{Counterfactual validation.} Each candidate patch is validated by executing it in the target execution environment. A candidate is accepted if it correctly satisfies the task while reducing the patch size; otherwise, the removed modifications are restored. The search terminates when no further modifications can be eliminated.

The remainder of this section describes each of these three stages in detail.




\subsection{Trajectory-Guided Search Space Construction}
\label{subsec:search_space}

The first stage of \algo\ constructs the search space over which
counterfactual reasoning is performed. Recall from
Section~\ref{sec:problem_formulation} that Patch Minimization seeks the
smallest behavior-preserving subset of an agent-generated patch
$\mathcal{AP}$. While the optimization is defined over patches,
\algo\ exploits the observation that the agent's trajectory captures
\textit{how} the final patch evolved through successive interactions with the execution
environment. Unlike the final patch, which records only the end result of the
repair process, the execution trajectory preserves the temporal and causal
relationships among modifications, revealing which edits were introduced,
refined, and validated together as the agent explored candidate solutions.
\algo\ leverages this additional structure to transform Patch Minimization from
an unstructured search over patch subsets into a trajectory-guided search over
related counterfactuals.



An \emph{execution trajectory}, $Traj$,  records the sequence of interactions between a
coding agent and its execution environment while solving a task. These
interactions include repository search, file inspection, code editing, command
execution, and test execution. Consequently, $Traj$ captures
not only the final agent-generated patch, but also the sequence of repair
hypotheses \shobini{Repair hypotheses was only informally defined on pg 4, which made 'sequence of repair hypotheses' confusing for me to understand. are these just a series of edits followed by feedback requests?}, interactions with the execution environment, and iterative
refinements that led to it.

While the execution trajectory contains rich information about the agent's
repair process, it is not directly suitable for Patch Minimization. In
particular, many trajectory actions do not contribute to the final patch, while
the remaining actions must be organized to expose the dependencies needed for
counterfactual reasoning. The goal of the first stage of \algo is
therefore to transform the raw execution trajectory into a structured search
space over which Patch Minimization can be performed.


\subsubsection{Trajectory Reconstruction}


Not all actions in $Traj$ are relevant for Patch Minimization.
Therefore, \algo first projects the execution trajectory onto a
reduced trajectory, denoted by $Traj_R$ (See~\Cref{fig:kernel_motivating_example}), by retaining only

\begin{itemize}
    \item $\mathcal{E}$: sequences of code edits performed between consecutive
    feedback requests, and
    \item $\mathcal{FR}$: feedback requests corresponding to executions of the
    task-related test suite.
\end{itemize}



All remaining actions, including repository search, file inspection,
directory navigation, and other non-modifying operations, are discarded because
they do not affect the resulting patch. The reduced trajectory is represented
as
\[
Traj_R
=
\left\langle
(\mathcal{E}_1,\mathcal{FR}_1),
(\mathcal{E}_2,\mathcal{FR}_2),
\ldots,
(\mathcal{E}_k,\mathcal{FR}_k)
\right\rangle,
\]

where
\[
\mathcal{E}_i=\langle e_{i1},e_{i2},\ldots,e_{in}\rangle
\]
denotes the \emph{ordered sequence} of edit actions performed after
$\mathcal{FR}_{i-1}$ and before $\mathcal{FR}_i$, where
$\mathcal{FR}_0=\emptyset$. Each edit action $e_{ij}$ corresponds to a single
editing operation issued by the agent (e.g., a search-and-replace operation or
a code insertion/deletion). 
%Although represented as a single action in the trajectory, 
$e_{ij}$ may modify multiple lines or multiple locations within one file using a standard search-and-replace operation. The corresponding $\mathcal{FR}_i$ denotes the
feedback request issued after completing the edit sequence
$\mathcal{E}_i$.

For illustration, consider the reduced trajectory corresponding to the motivating example in~\Cref{fig:kernel_motivating_example}. The reduced trajectory is
$Traj_R=\langle(\mathcal{E}_1,\mathcal{FR}_1),(\mathcal{E}_2,\mathcal{FR}_2),(\mathcal{E}_3,\mathcal{FR}_3)\rangle)$,
where $(\mathcal{E}_1=\langle e_{11}\rangle)$, $(\mathcal{E}_2=\langle e_{21}\rangle)$, and $(\mathcal{E}_3=\langle e_{31},e_{32},e_{33}\rangle)$. As described next, \algo\ performs Patch Minimization by searching over this trajectory representation, progressively refining the search from edit sequences to individual files and, ultimately, individual edit actions.



\textit{Implementation Challenges.} %\junfeng{these challenges don't seem that difficult} 
Recovering edit actions is non-trivial because different coding agents expose
different editing primitives (e.g., shell commands such as \texttt{sed} versus
structured editing tools such as \texttt{str\_replace\_editor} or
\texttt{replace}). To enable a single reduction algorithm across heterogeneous
agent scaffolds, we normalize every editing action into a common
representation consisting of the target file together with its corresponding
before- and after-text. All subsequent stages of \algo\ operate exclusively on
this normalized representation.

A second challenge is that execution trajectories record the agent's entire
search process, including exploratory edits that are later reverted. Agents may
undo individual edits, restore files (e.g., \texttt{git checkout},
\texttt{git restore}), discard outstanding changes (e.g.,
\texttt{git reset}), temporarily shelve edits (e.g., \texttt{git stash}), or
issue edits that ultimately have no effect. Consequently, simply treating every extracted editing action as contributing to the final patch would fail to correctly attribute which edits survive into the final submitted patch, because agents may revert, restore, or overwrite earlier edits.
%Consequently, simply extracting every editing action would fail to reconstruct the final submitted patch \shobini{Maybe "concatenating" instead of "extracting"? Also this last sentence generally could be confusing to a reader, since earlier we say we only retain edit actions and feedback requests. Can we instead say something like "Consequently, simply treating every extracted editing action as contributing to the final patch would fail to correctly attribute which edits survive into the final submitted patch, because agents may revert, restore, or overwrite earlier edits." I think the grouping of edit and undo operations as "Edit actions" is confusing, and here in this last sentence we say "editing action" which is also confusing.}.

To recover the true construction process, \algo\ faithfully replays the editing
history in $Traj$, applying both editing and undo operations in temporal order.
The resulting reduced trajectory $Traj_R$ retains only the edit actions that
survive in the final patch while preserving the order in which they were
introduced, thereby faithfully reconstructing the sequence of repair
hypotheses leading to the submitted patch.




\subsubsection{Trajectory-derived Search Space}

The reduced trajectory $Traj_R$ defines the search space explored by \algo.
The key observation is that coding agents naturally organize repairs into
successive \emph{edit--feedback\_request} iterations. Before issuing a feedback
request, the agent typically develops and refines a single repair hypothesis
through a sequence of edit actions.

Accordingly, each pair $(\mathcal{E}_i,\mathcal{FR}_i)$ in $Traj_R$ represents
one repair hypothesis together with the corresponding feedback request used to
validate it \shobini{Use of repair hypothesis paired with corresponding feedback request makes the earlier note about "sequence of repair hypotheses" more confusing.}. Thus, rather than enumerating arbitrary subsets of edits, \algo\ first
reasons about these edit--feedback request iterations as the basic units of
counterfactual search before progressively refining the search to individual
files and, ultimately, individual edit actions.

\begin{comment}




\alex{
Linux Motivating Example showcases -- (1) node-level minimum suffix, and (2) edit-level reduce operation.
SWE-Bench Example showcases -- (1) node-level reduce operation, (2) file-level reduce operation, and (3) edit-level reduce operation. Together they show all kinds of minimization operations.
}


For illustration, consider the preprocessed trajectory shown below:

\[
\begin{aligned}
Traj' = [&E_{11}^{D},\, FR_1,\,
E_{21}^{A},\, E_{22}^{B},\, FR_2,\,
E_{31}^{C},\, E_{32}^{C},\, FR_3,\\
&
E_{41}^{B},\, E_{42}^{E},\, FR_4,\,
E_{51}^{A},\, FR_5 ].
\end{aligned}
\]

Here, $FR_i$ denotes the $i^{th}$ feedback request (i.e., execution of the
task test suite). We use $E_{ij}^{F}$ solely as illustrative notation to
denote the $j^{th}$ edit made after the $(i-1)^{th}$ feedback request and
before the $i^{th}$ feedback request, where the superscript $F$ indicates the
file being modified.

This notation mirrors the motivating example in
Figures~\ref{fig:agent_traj} and~\ref{fig:motiv_fig}. There, the agent produces
three edit--test iterations containing the edit groups
$\{E_{11}\}$, $\{E_{21}\}$, and
$\{E_{31},E_{32},E_{33}\}$. The only difference is that the motivating example
contains edits to a single file, whereas the illustrative trajectory above
shows edits distributed across multiple files.



\end{comment}




\subsection{Hierarchical Counterfactual Search}
\label{subsec:method-B}


This section presents the design principles underlying \algo. At a high
level, \algo formulates Patch Minimization as a constrained optimization
problem: remove as much \aislop\ as possible while preserving program
behavior and keeping the minimization process computationally practical.

\subsubsection*{Optimization Objective}

As established in Section~\ref{sec:problem_formulation}, the objective of
\algo is to approximate the minimal behavior-preserving patch of an
agent-generated patch \agentp\ for a given task $T$. Rather than minimizing
\agentp\ as an unstructured collection of edits, \algo performs
\emph{trajectory-guided optimization}, exploiting the temporal organization
and repair hypotheses encoded in the repair trajectory to identify
functionally unnecessary edits. Thus, instead of synthesizing a new repair,
\algo seeks a \emph{one-minimal} edit action subset of the original trajectory edits that still satisfies the task (\S\ref{subsec:one_minimal}).
%\shobini{Link to one-minimal section?}
\subsubsection*{Correctness Constraint}

Since the ideal notion of behavior preservation cannot be established
directly, \algo adopts the same execution-based approximation used by coding
agents: every accepted counterfactual patch must continue to pass the
task-specific test suite $TF$. This execution invariant ensures that edits are
eliminated safely without changing the observable behavior of the repair.

\subsubsection*{Efficiency Constraint}

Maintaining the execution invariant requires executing $TF$ for every
candidate counterfactual. In many repair settings, this dominates the cost of
minimization. For example, validating a Linux kernel repair requires
rebuilding the kernel ($\sim$20 minutes) and replaying the crashing workload
($\sim$10 minutes), resulting in roughly 30 minutes per
validation~\cite{mathai2024kgym}. Since minimization evaluates many
counterfactuals, these costs quickly accumulate.

Consequently, the effectiveness of a minimization algorithm depends not only
on the amount of \aislop\ removed (measured by \patchdiff), but also on the
number of validation executions. This efficiency constraint motivates the
hierarchical coarse-to-fine search strategy described next.



\input{sections/Algorithms/ray_overview}

% \begin{figure}[t]
% \centering
% \begin{tikzpicture}[
%   e/.style={draw, rounded corners=2pt, minimum width=7mm, minimum height=5mm,
%             font=\scriptsize, inner sep=1pt},
%   f1/.style={e, fill=orange!18},          % file f_1
%   f2/.style={e, fill=blue!12},            % file f_2 (buggy file)
%   dead/.style={e, fill=black!8, text=black!45},
%   fix/.style={f2, very thick},            % the two fix edits
%   row/.style={font=\footnotesize, anchor=west},
%   drop/.style={font=\scriptsize, anchor=west, gray},
%   every node/.style={outer sep=0pt},
% ]
% \def\rs{1.6}   % row spacing (was 1.05 — opened up to stop overlap)
% \def\dy{0.7}   % how far the gray "drop" caption sits below its row

% % --- Row 1: agent patch, by hypothesis ---
% \node[row] at (-0.5,0) {Agent patch \agentp};
% \node[dead] (a11) at (3.2,0) {$e_{11}$};
% \node[f1, right=2mm of a11] (a21) {$e_{21}$};
% \node[f2, right=0.6mm of a21] (a22) {$e_{22}$};
% \node[dead, right=2mm of a22] (a31) {$e_{31}$};
% \node[fix, right=2mm of a31] (a41) {$e_{41}^\star$};
% \node[f1, right=0.6mm of a41] (a42) {$e_{42}$};
% \node[fix, right=0.6mm of a42] (a43) {$e_{43}^\star$};
% \node[font=\scriptsize, yshift=4mm] at (a11) {$\mathcal{E}_1$};
% \node[font=\scriptsize, yshift=4mm] at ($(a21)!0.5!(a22)$) {$\mathcal{E}_2$};
% \node[font=\scriptsize, yshift=4mm] at (a31) {$\mathcal{E}_3$};
% \node[font=\scriptsize, yshift=4mm] at ($(a41)!0.5!(a43)$) {$\mathcal{E}_4$};
% \node[drop] at (3.2,-\dy) {seq level: drop dead hypotheses $\mathcal{E}_1,\mathcal{E}_3$};

% % --- Row 2: after seq, by file ---
% \node[row] at (-0.5,-\rs) {Post Seq-based Removal};
% \node[f1] (b21) at (3.2,-\rs) {$e_{21}$};
% \node[f1, right=0.6mm of b21] (b42) {$e_{42}$};
% \node[f2, right=4mm of b42] (b22) {$e_{22}$};
% \node[fix, right=0.6mm of b22] (b41) {$e_{41}^\star$};
% \node[fix, right=0.6mm of b41] (b43) {$e_{43}^\star$};
% \node[font=\scriptsize, yshift=4mm] at ($(b21)!0.5!(b42)$) {file $f_1$};
% \node[font=\scriptsize, yshift=4mm] at ($(b22)!0.5!(b43)$) {file $f_2$};
% \node[drop] at (3.2,-\rs-\dy) {file level: drop unrelated $f_1$ ($e_{21},e_{42}$ leave together)};

% % --- Row 3: after file, individual edits ---
% \node[row] at (-0.5,-2*\rs) {Post File-based Removal};
% \node[f2] (c22) at (3.2,-2*\rs) {$e_{22}$};
% \node[fix, right=0.6mm of c22] (c41) {$e_{41}^\star$};
% \node[fix, right=0.6mm of c41] (c43) {$e_{43}^\star$};
% \node[drop] at (3.2,-2*\rs-\dy) {edit level: drop residual slop $e_{22}$};

% % --- Row 4: minimal patch ---
% \node[row] at (-0.5,-3*\rs) {Post action-based Removal};
% \node[fix] (d41) at (3.2,-3*\rs) {$e_{41}^\star$};
% \node[fix, right=0.6mm of d41] (d43) {$e_{43}^\star$};

% % --- arrows between rows (span the gap, clear of labels) ---
% \foreach \y in {0,1,2}
%   \draw[-{Latex[length=1.5mm]}] (2.9,-\y*\rs-\dy-0.18) -- (2.9,-\y*\rs-\rs+0.30);
% \end{tikzpicture}
% \caption{Example shows how \algo\ works on recovering the minimal patch from an agent patch containing 7 edit sequences. Different node colors indicate different files.
% Starred edit actions ($e_{41},e_{43}$) are the true fix; all others are \aislop.}
% \label{fig:trim-example}
% \end{figure}


\begin{figure}[t]
\centering
% Needs: \usetikzlibrary{positioning, calc, arrows.meta, shadows}
\resizebox{0.9\columnwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  e/.style={draw=black!35, line width=0.5pt, rounded corners=2.5pt,
            minimum width=11mm, minimum height=8.5mm, inner sep=2pt, font=\normalsize},
  pill/.style={rounded corners=3pt, inner xsep=4pt, inner ysep=2pt,
            font=\small\bfseries, text=white},
  gdesc/.style={anchor=west, font=\footnotesize, text=black!55},
  glab/.style={font=\small\itshape, text=black!60},
  rowL/.style={anchor=west, align=left, text=black!80},
  sh/.style={drop shadow={shadow xshift=0.4pt, shadow yshift=-0.5pt,
            opacity=0.22, fill=black!60}},
  f1/.style={e, sh, fill=orange!18, draw=orange!60, text=black!85},
  f2/.style={e, sh, fill=blue!12,  draw=blue!55,   text=black!85},
  fix/.style={e, sh, fill=blue!25, draw=blue!75!black, line width=1pt, text=black!90},
  dead/.style={e, fill=black!6, draw=black!30,
            dash pattern=on 1.5pt off 1pt, text=black!50},
  glab/.style={font=\small\itshape, text=black!60},
  grp/.style={rounded corners=4pt, draw=black!40, line width=0.6pt, fill=black!5},
  gdesc/.style={anchor=west, font=\small, text=black!55},
  tip/.style={-{Latex[length=2mm]}, draw=black!45, line width=0.7pt},
]

% ---- invisible anchor nodes first (define positions, draw nothing) ----
\path (3.4,0)    node[e, draw=none, fill=none] (a11) {}
      ([xshift=12mm]a11.center) node[e, draw=none, fill=none] (a21) {};
% (we instead place real nodes below; anchors not needed) 

% ======== Row 1: agent patch, by hypothesis ========
\node[rowL] at (-1.95,0)
  {\normalsize\bfseries Agent patch \agentp\\[2pt]\textcolor{black!50}{\small 7 edits}};

% place real nodes
\node[dead] (a11) at (3.4,0) {$e_{11}$};
\node[f1, right=7mm of a11]   (a21) {$e_{21}$};
\node[f2, right=0.8mm of a21] (a22) {$e_{22}$};
\node[dead, right=7mm of a22] (a31) {$e_{31}$};
\node[fix, right=7mm of a31]  (a41) {$e_{41}^{\star}$};
\node[f1, right=0.8mm of a41] (a42) {$e_{42}$};
\node[fix, right=0.8mm of a42] (a43) {$e_{43}^{\star}$};
% group boxes BEHIND, then RE-DRAW the nodes on top
\gbox{a11}{a11}{$\mathcal{E}_1$}
\gbox{a21}{a22}{$\mathcal{E}_2$}
\gbox{a31}{a31}{$\mathcal{E}_3$}
\gbox{a41}{a43}{$\mathcal{E}_4$}
\node[dead] at (a11) {$e_{11}$};
\node[f1]  at (a21) {$e_{21}$};
\node[f2]  at (a22) {$e_{22}$};
\node[dead] at (a31) {$e_{31}$};
\node[fix] at (a41) {$e_{41}^{\star}$};
\node[f1]  at (a42) {$e_{42}$};
\node[fix] at (a43) {$e_{43}^{\star}$};

% ======== Row 2: after seq, by file ========
\node[rowL] at (-1.95,-2.4)
  {\small\bfseries After Edit Seq removal\\[2pt]\textcolor{black!50}{\footnotesize 5 edits}};
\node[f1] (b21) at (3.4,-2.4) {$e_{21}$};
\node[f1, right=0.8mm of b21] (b42) {$e_{42}$};
\node[f2, right=6mm of b42]   (b22) {$e_{22}$};
\node[fix, right=0.8mm of b22] (b41) {$e_{41}^{\star}$};
\node[fix, right=0.8mm of b41] (b43) {$e_{43}^{\star}$};
\gbox{b21}{b42}{File $f_1$}
\gbox{b22}{b43}{File $f_2$}
\node[f1]  at (b21) {$e_{21}$};
\node[f1]  at (b42) {$e_{42}$};
\node[f2]  at (b22) {$e_{22}$};
\node[fix] at (b41) {$e_{41}^{\star}$};
\node[fix] at (b43) {$e_{43}^{\star}$};

% ======== Row 3: after file, individual edits ========
\node[rowL] at (-1.95,-4.8)
  {\small\bfseries After File removal\\[2pt]\textcolor{black!50}{\footnotesize 3 edits}};
\node[f2] (c22) at (3.4,-4.8) {$e_{22}$};
\node[fix, right=7mm of c22] (c41) {$e_{41}^{\star}$};
\node[fix, right=7mm of c41] (c43) {$e_{43}^{\star}$};
\gbox{c22}{c22}{}
\gbox{c41}{c41}{}
\gbox{c43}{c43}{}
\node[f2]  at (c22) {$e_{22}$};
\node[fix] at (c41) {$e_{41}^{\star}$};
\node[fix] at (c43) {$e_{43}^{\star}$};

% ======== Row 4: minimal patch ========
\node[rowL] at (-1.95,-7.2)
  {\small\bfseries After edit action removal \\ (Minimal patch)\\[2pt]\textcolor{black!50}{\footnotesize 2 edits = fix}};
\node[fix] (d41) at (3.4,-7.2) {$e_{41}^{\star}$};
\node[fix, right=0.8mm of d41] (d43) {$e_{43}^{\star}$};
\draw[grp, draw=blue!60, fill=blue!6]
  ([xshift=-2.5mm,yshift=-2.8mm]d41.south west)
  rectangle ([xshift=2.5mm,yshift=2.8mm]d43.north east);
\node[fix] at (d41) {$e_{41}^{\star}$};
\node[fix] at (d43) {$e_{43}^{\star}$};

% ======== arrows + level pills ========
\draw[tip] (5.0,-0.7) -- (5.0,-1.7);
\node[pill, fill=purple!65, anchor=west] (p0) at (5.5,-0.95) {Seq};
\node[gdesc] at (p0.east) {\,drop $\mathcal{E}_1,\mathcal{E}_3$};

\draw[tip] (5.0,-3.1) -- (5.0,-4.1);
\node[pill, fill=teal!60!black, anchor=west] (p1) at (5.5,-3.6) {File};
\node[gdesc] at (p1.east) {\,drop $f_1$ ($e_{21},e_{42}$)};

\draw[tip] (5.0,-5.5) -- (5.0,-6.5);
\node[pill, fill=orange!75!black, anchor=west] (p2) at (5.5,-6.0) {Edit};
\node[gdesc] at (p2.east) {\,drop $e_{22}$};

% ======== legend ========
\node[f1,  minimum width=6mm, minimum height=5mm] (l1) at (-1.6,-8.7) {};
\node[gdesc] at (l1.east) {\,$file_1$};
\node[f2,  minimum width=6mm, minimum height=5mm] (l2) at (0.2,-8.7) {};
\node[gdesc] at (l2.east) {\,$file_2$};
\node[fix, minimum width=6mm, minimum height=5mm] (l3) at (2.1,-8.7) {};
\node[gdesc] at (l3.east) {\,fix ($\star$)};
\node[dead,minimum width=6mm, minimum height=5mm] (l4) at (4.4,-8.7) {};
\node[gdesc] at (l4.east) {\,dead};

\end{tikzpicture}%
}
\caption{\algo\ recovering the minimal patch from a 7-edit agent patch.
Different rows represent the granularity \algo\ reasons about at each level---edit sequence, then files,
then individual edit actions. Node color denotes the edited file; starred edits
($e_{41},e_{43}$) are the true edit actions and all others are \aislop. The patch shrinks
$7\!\to\!5\!\to\!3\!\to\!2$.}
\label{fig:trim-example}
\vspace{-5mm}
\end{figure}


\subsubsection*{Minimization Strategy}

Algorithm~\ref{alg:patchmin} presents the overall hierarchical
counterfactual search procedure.~\Cref{fig:trim-example} also pictorially describes how the algorithm works. Starting from the repair
trajectory $Traj_R$, \algo progressively searches for functionally
unnecessary edits by constructing and evaluating \emph{counterfactual
patches}. Rather than reasoning over individual modifications from the outset,
\algo first searches over larger removal candidates (e.g., an edit sequence like $\mathcal{E}$), allowing a
single successful validation to eliminate many edit actions simultaneously.
Only when no further removals are possible does the search refine to
smaller candidate units, thereby reducing the number of expensive
validation executions.

The search consists of three successive phases corresponding to the
hierarchy
$\textit{edit sequence} \rightarrow \textit{file} \rightarrow
\textit{edit action}$ (see the outer loop, Line~\ref{alg:outerloop}).
At the beginning of each phase, the surviving edits are \emph{regrouped}
(Line~\ref{alg:regroup}) according to the current search granularity (\textit{edit sequence},  \textit{file}, or \textit{edit action}),
thereby defining the ``unit" of a candidate removal for that phase.
During sequence-level search, each candidate consists of the edits
introduced between two consecutive feedback requests (See row 1 of~\Cref{fig:trim-example}).
During file-level search, the surviving edits are repartitioned so that
each candidate contains all edits affecting a particular file,
irrespective of when they were introduced (See row 2 of~\Cref{fig:trim-example}).
Finally, edit action-level search treats every surviving edit action as an independent
candidate, enabling fine-grained minimization (See row 3 of~\Cref{fig:trim-example}).
Thus, while the grouping of modifications changes across phases, the underlying
search procedure remains identical.

For each grouping, \algo performs the same iterative elimination
procedure. The algorithm traverses the candidate units in reverse
trajectory order and temporarily removes one unit at a time,
thereby constructing a \emph{counterfactual patch} that represents the ``hypothetical repair" had that candidate never been introduced.

\textit{Counterfactual Validation.} 
The counterfactual is accepted only if (i) it continues to satisfy the
task-specific test suite $TF$, thereby preserving the execution
invariant, and (ii) it produces a strictly smaller patch than the
current solution (Line~\ref{alg:accept}).
Otherwise, the candidate is rejected and the removed edits are restored. 
The elimination process repeats until no additional candidate units can
be removed at the current granularity (Line~\ref{alg:termination}),
thereby reaching a local fixpoint. The last row of~\Cref{fig:trim-example}) shows the final required edit actions following this algorithm. 
% If the one-minimality guarantee (see below) is enabled (\algo-G), the algorithm
% repeatedly revisits the current grouping until this fixpoint is reached.
% Otherwise (\algo-NG), a single pass is performed before refining the
% search to the next granularity.
% After all three phases complete, the surviving edits are replayed to
% construct the minimized patch $\mathcal{MP}$.


\subsubsection*{One-Minimality Guarantee}
\label{subsec:one_minimal}

The hierarchical search described above efficiently removes unnecessary
edits. However, a single pass does not necessarily recover a
\emph{one-minimal edit subset}, since an edit that could not be removed
earlier may become removable after other edits have been eliminated.

To recover a one-minimal edit subset, \algo optionally enables the
\textit{oneMin} flag. When enabled, each search phase repeats until no
additional candidate unit can be eliminated
(Line~\ref{alg:termination}). Since every accepted removal strictly reduces
the patch while preserving the execution invariant, termination implies that
no remaining candidate at the current granularity can be safely removed.
After the final edit-level phase, this guarantees that no individual edit
can be removed while still satisfying the task-specific test suite $TF$,
thereby recovering a one-minimal edit subset.

When \textit{oneMin} is disabled (\algo-NG), each granularity is explored
only once, reducing validation cost at the expense of the one-minimality
guarantee.


\subsubsection*{Algorithmic Analysis}
\label{subsec:algorithmic_analysis}

The dominant cost of patch
minimization is executing the task-specific test suite $TF$. We therefore
measure the cost complexity $\mathcal{C}$ of \algo as the number of
$TF$ executions.\junfeng{unclear what's non obvious in the algorithm. what's hard?}


\textbf{Cost Complexity.} Without the one-minimality guarantee (\algoNG), each search phase performs a
single pass over its candidate units, yielding $
\mathcal{C}_{\algoNG}
=
\mathcal{O}(|Traj_R|+|F|+|E|)
=
\mathcal{O}(|E|),
$ since $|E| \gg |Traj_R| > |F|$.~\rayb{What is E and F?}

With the one-minimality guarantee enabled (\algoG), each phase repeats until
reaching a local fixpoint. In the worst case, each candidate may be revisited
once for every remaining candidate, giving $
\mathcal{C}_{\algoG}
=
\mathcal{O}(|Traj_R|^2+|F|^2+|E|^2)
=
\mathcal{O}(|E|^2).
$

Thus, enabling one-minimality increases the worst-case cost complexity from
linear to quadratic in the number of edits. As shown in
Section~\ref{sec:expr}, however, the practical overhead is much smaller,
making \algoG empirically close to linear while providing the stronger
guarantee.

\textbf{Time Complexity.}
The same analysis applies to runtime, yielding
$\mathcal{O}(|E|)$ for \algoNG and
$\mathcal{O}(|E|^2)$ for \algoG.


% \textbf{Cost Complexity.} Without the one-minimality guarantee (\algoNG), each search phase performs a
% single pass over its candidate units. The sequence-, file-, and edit-level
% phases therefore contribute $\mathcal{O}(|Traj_R|)$, $\mathcal{O}(|F|)$, and
% $\mathcal{O}(|E|)$ candidate evaluations, respectively, while regrouping and
% patch reconstruction incur no additional $TF$ executions.
% Consequently,
% \[
% \mathcal{C}_{\algoNG}
% =
% \mathcal{O}(|Traj_R|+|F|+|E|)
% =
% \mathcal{O}(|E|),
% \]
% since $|E| \gg |Traj_R| > |F|$.
% With the one-minimality guarantee enabled (\algoG), each search phase repeats
% until reaching a local fixpoint. In the worst case, this requires revisiting
% each candidate once for every remaining candidate, increasing the complexity
% of each phase from linear to quadratic. Therefore,
% \[
% \mathcal{C}_{\algoG}
% =
% \mathcal{O}(|Traj_R|^2+|F|^2+|E|^2)
% =
% \mathcal{O}(|E|^2).
% \]
% Thus, the one-minimality guarantee increases the worst-case cost complexity
% from linear to quadratic in the number of edits.

% In Section~\ref{sec:expr}, however, we show that the practical overhead of
% \algoG is substantially smaller than this worst-case bound. The number of
% additional $TF$ executions remains modest, making \algoG
% empirically close to linear while providing the stronger one-minimality
% guarantee.

% \textbf{Time Complexity.}
% The same analysis applies to runtime, yielding
% $\mathcal{O}(|E|)$ for \algoNG and
% $\mathcal{O}(|E|^2)$ for \algoG.







%\input{sections/methodology_minimization_system}

%\input{sections/methodology_algorithm_analysis}

==> sections/backup/5_exp.tex <==
\section{Experimental Design}
\label{sec:expr}

In this section, we explain the setup to evaluate \algo.
% \subsection{Common Setups across RQs}
% \label{subsec:rq_setup}


\subsection{Study Subjects}
\label{subsec:rq_setup}

% We evaluate \algo across two benchmarks and four agentic scaffolds to assess
% its effectiveness, efficiency, and generality. 
% Our evaluation uses two complementary benchmarks. \textbf{Live-kBench}
% \cite{huang2026outrunningllmcutoffslive} contains $534$ recent Linux kernel
% vulnerabilities, evaluating repair agents on security-critical debugging tasks
% in a large C codebase. Since \algo is a post-processing technique, 
% it is applicable only to bugs for which the repair agent successfully generates a valid patch. 
% Across all evaluated scaffolds, this yields $433$ repaired bugs. Among these, $140$ bugs have patches consisting of a single edit action and are therefore already trivially one-minimal, leaving $293$ bugs 
% on which patch minimization is applicable. \textbf{SWE-Bench-Verified}~\cite{jimenez2023swe} 
% contains $500$ manually verified GitHub issues from popular Python repositories, 
% evaluating repository-level software engineering tasks under executable test suites.

We evaluate \algo across two benchmarks and four agentic scaffolds to assess
its effectiveness, efficiency, and generality. Our evaluation uses two
complementary benchmarks. \textbf{Live-kBench}
\cite{huang2026outrunningllmcutoffslive} contains $534$ recent Linux kernel
vulnerabilities, evaluating repair agents on security-critical debugging tasks
in a large C codebase. We use Live-kBench as our primary evaluation benchmark because Patch
Minimization is particularly important for security fixes, where smaller,
more focused patches reduce unnecessary attack surface and simplify
developer review and security auditing. Since \algo\ is a
post-processing technique, it is applicable only to bugs for which the repair
agent successfully generates a valid patch. Across all evaluated scaffolds,
this yields $433$ repaired bugs. Among these, $140$ bugs have patches
consisting of a single edit action and are therefore already trivially
one-minimal, leaving $293$ bugs on which patch minimization is applicable.
To evaluate the generality of \algo, we additionally consider

\textbf{SWE-Bench-Verified}~\cite{jimenez2023swe} contains $500$ manually
verified GitHub issues from popular Python repositories, evaluating
repository-level software engineering tasks under executable test suites. We
evaluate \algoG (edit-action level) on $333$ \swe\ (Claude-Sonnet-4)
trajectories downloaded from the SWE-Bench leaderboard, all of which have
been verified to pass the hidden oracle. 

To demonstrate the generality of \algo, we evaluate patches generated by four
state-of-the-art agentic scaffolds: \crashfixer
\cite{mathai2025crashfixer}, \swe, \mini
\cite{yang2024swe}, and \openhands
\cite{wang2024openhands}. Across all benchmark--scaffold combinations, we
run \algo on a total of $4,544$ repair trajectories. The trajectories are 
generated using LLMs like Gemini-3-Pro and Claude-Opus-4.5.



\subsection{Evaluation Metrics}
\label{sec:eval_metric}

We evaluate \algo\ along three dimensions. The first two quantify the
\emph{effectiveness} of Patch Minimization: (i) Code Slop reduction
(\patchdiff) and (ii) correctness with respect to the evaluation oracle. 
The third quantifies \emph{efficiency} using the total number of $TF$ executions
performed during minimization.
%(i) the amount of \aislop\ removed
% (\patchdiff), (ii) the cost of minimization, measured by the number of test
% suite executions ($TF$), and (iii) the correctness of the minimized patch,
% measured using benchmark-specific \emph{oracle tests}.


\textbf{(i) \aislop Reduction (\patchdiff).}
For each benchmark--scaffold combination, we quantify the amount of
\aislop\ removed by a minimization method (\algo or a baseline) as the
average normalized reduction in the patch length:

\begin{equation}
\Delta_{\text{Slop}} (\%)
=
\frac{
\operatorname{avg}\left(
  \operatorname{len}(\mathcal{AP})- \operatorname{len}(\mathcal{MP})
  \right)
}
{
\operatorname{avg}\!\left(\operatorname{len}(\mathcal{AP})\right)
} \times 100
\end{equation}

Here, $\mathcal{AP}$ denotes the original agent-generated patch and
$\mathcal{MP}$ the minimized patch produced by the method under evaluation.
Higher values of \patchdiff\ indicate that more \aislop has been
eliminated.

Note that, the test suites $TF$ are the only correctness signal available to \algo\
during minimization and correspond exactly to the tests executed by the
repair agent. For Live-kBench, the machine-generated crash-reproducing script
serves as $TF$. For SWE-Bench-Verified, $TF$ comprises the tests generated
and executed by the agent throughout its repair trajectory. Unless otherwise
specified, all reported \patchdiff\ results are obtained using only $TF$ as
the validation signal. Importantly, $TF$ is distinct from the oracle tests
described below, which are used solely for evaluation.



\textbf{(ii) Oracle Tests.}
Oracle tests are reserved exclusively for evaluation and are never available
to \algo during minimization. For Live-kBench, the oracle consists of (a) the
crash-reproducing script and (b) an LLM judge that determines whether the
minimized patch is semantically equivalent to the developer patch. The crash
script alone is insufficient because multiple patches may eliminate the crash
while exhibiting different behavior. Following
\citet{huang2026outrunningllmcutoffslive}, we use Gemini-3-Flash to
sample nine independent judgments and classify two patches as equivalent when
a majority vote returns an ``equivalent'' verdict.

For SWE-Bench-Verified, the oracle is the benchmark's hidden
\emph{fail-to-pass} test suite. Since these hidden tests comprehensively
validate functional correctness, no additional semantic judge is required.

\textbf{(iii) Cost of Minimization.}
As discussed in Section~\ref{subsec:algorithmic_analysis}, the dominant cost
of Patch Minimization is validating candidate patches by executing the
task-specific test suite $TF$. We therefore treat a single execution of
$TF$ as one unit of validation cost, regardless of the number of individual
test cases it contains. The total number of $TF$ executions thus provides a
\emph{machine-independent} approximation of computational cost. Unlike
wall-clock time, which depends on the underlying hardware and system
configuration, the number of $TF$ executions reflects the intrinsic
efficiency of the minimization algorithm and enables fair comparison across
different execution environments. Within a benchmark, where each $TF$
represents a fixed validation procedure, this metric is directly
proportional to both execution time and hardware cost.






% \textbf{LLM Judge.}
% Following \citet{huang2026outrunningllmcutoffslive}, we use Gemini-3-Flash to
% sample nine independent judgments and classify two patches as equivalent when
% a majority vote returns an ``equivalent'' verdict.





%\alex{To add numbers of trajs for each scaffold.}

% \textbf{LLMs}.  We use Gemini-3-Flash for our baselines on agentic minimization. We run \algo on trajectories generated using LLMs like Gemini-3-Pro and Claude-Opus-4.5~\rayb{It looks like baseline is suboptimal with Gemini-3-Flash.}.

\subsection{Baselines}
\label{subsec:baselines}

We compare \algo against two classes of baselines: \emph{agentic}
minimization and \emph{deterministic} patch minimization.

\textbf{Agentic Minimization.}
Our first baseline evaluates whether a general-purpose coding agent can
minimize its own patches without an explicit minimization algorithm. We use
\mini\ with Gemini-3-Flash as the minimization agent. The agent is given the
same execution environment as \algo, including access to the task-specific
test suite $TF$ for validating candidate patches. Each minimization run is
allocated a maximum budget of 6 hours and \$5.6 (following~\cite{huang2026outrunningllmcutoffslive}). We evaluate three prompting
configurations:
(a) \emph{Only Diff}, where the agent receives only the final patch;
(b) \emph{Only Traj}, where it receives only the repair trajectory; and
(c) \emph{Both}, where it receives both the final patch and repair
trajectory.

\textbf{Deterministic Minimization.}
Our second baseline is a deterministic adaptation of Delta Debugging
(DD-Hunk)~\cite{10.1145/1134285.1134307}. Since traditional Delta Debugging
operates over program inputs rather than agent-generated patches, we modify
it to perform patch minimization over patch hunks. Like
\algo, DD-Hunk validates candidates patch using the task-specific test
suite $TF$, enabling a direct comparison between trajectory-guided and
direct patch-based minimization strategies.

\textbf{\algo Variants.}
We evaluate two variants of \algo.
\algoNG performs a single elimination pass at each search granularity,
whereas \algoG repeatedly applies minimization until a local fixpoint is
reached, thereby guaranteeing a one-minimal solution. We also report
the intermediate results after each stage of the hierarchical search:
\emph{Sequence} (edit-sequence minimization only),
%\emph{Sequence-File} (sequence followed by file-level minimization), 
\emph{Edit} (the complete coarse-to-fine search through edit actions), and \emph{Hybrid} (a policy that chooses \emph{Sequence} if its reduction outputs one sequence, else \emph{Edit}).




\subsection{Research Question}
\label{sec:rq}
\textbf{Research Questions}. We structure the rest of the experiments section around four main research questions (RQs).



\begin{itemize}
    \item RQ1: How effectively does \algo\ reduce \aislop\ for security program repair (\S\ref{subsec:rq1})?
    \item RQ2: How does \algo\ compare against agentic minimization in reducing \aislop\ (\S\ref{subsec:rq2})?
    \item RQ3: How does \algo\ compare against deterministic patch minimization algorithms (\S\ref{subsec:rq3})? 
    \item RQ4: Does \algo\ generalize to general-purpose program repair benchmarks (\S\ref{subsec:rq4})?
\end{itemize}

==> sections/backup/experiments.tex <==
\section{Experiments}
\label{sec:expr}

In this section, we perform \aislop 
%\shobini{should this be CodeSlop instead of 'slop'?} 
minimization experiments across four agentic scaffolds and two benchmarks, to showcase the generalization capability of \algo. We measure performance using metrics like (a) the reduction in \aislop (\patchdiff), and (b) the cost of execution. We also compare against two baselines - (i) agentic minimization to check if agents minimize patches effectively and reliably, and (ii) deterministic algorithms like the Delta Debugging routine that we modify to perform patch hunk minimization. 

\subsection{Common Setup across RQs}
\label{subsec:rq_setup}

\textbf{Datasets}. We run \algo on two datasets. The first is Live-kBench \cite{huang2026outrunningllmcutoffslive}, a benchmark of $534$ recent Linux kernel vulnerabilities. The second is SWE-Bench-Verified \cite{jimenez2023swe}, a dataset of $500$ real-world Github issues in popular Python repositories~\rayb{Add one line what each of these dataset does. especially ppl may not know kbench}. 

\textbf{Metrics}. In addition to \patchdiff and the cost of execution, we also evaluate oracle performance ($O$) of the minimized patch to measure any regressions using ``oracle tests". 
For Live-kBench, the oracle test is a combination of (i) passing the crash reproducing script, and (ii) passing an LLM-Judge that checks for equivalence between the minimized patch and the human patch~\rayb{explain why do you need LLM judge?}. 
For SWE-Bench-Verified, the oracle test is the hidden fail-to-pass testcase associated with each issue~\rayb{Why SWE Bench does not need LLM as judge?}.

\textbf{\textsc{TF}s} (test files). For SWE-Bench-Verified, $TF$ are the test files the agent creates and executes during its trajectory. This is distinct from the ``oracle tests" mentioned earlier, which are hidden fail-to-pass tests. For Live-kBench, given the ``fuzzer" origin of its bugs, each bug receives a crash-reproducing script that is \textit{machine-generated} during the fuzzing process. Hence, this script is provided to the agent and is thus the $TF$. Note, as mentioned above, the crash-reproducing script is also part of the Oracle checking criteria. So for Live-kBench, the same script is used as a test file and an oracle. 


\textbf{Scaffolds}. We experiment with four agentic scaffolds - \crashfixer \cite{mathai2025crashfixer}, \swe \& \mini \cite{yang2024swe}, and \openhands \cite{wang2024openhands}, to test algorithmic generalization. We run \algo on a total of $4544$ trajectories. 
%\alex{To add numbers of trajs for each scaffold.}

\textbf{LLMs}.  We use Gemini-3-Flash for our baselines on agentic minimization. We run \algo on trajectories generated using LLMs like Gemini-3-Pro and Claude-Opus-4.5~\rayb{It looks like baseline is suboptimal with Gemini-3-Flash.}.

\textbf{LLM Judge}. We follow \citet{huang2026outrunningllmcutoffslive} and use Gemini-3-Flash to sample nine votes, and consider a patch equivalent when majority support the ``equivalent verdict".

\textbf{Compute}. To run our experiments for Live-kBench, we deploy a cluster of $37$ 88-vCPU Google Compute Engine machines. This high-performance cluster helps build and run Linux kernels, which is a time-consuming and expensive task.


\textbf{Research Questions}. We structure the rest of the experiments section around five main research questions (RQs).

\begin{itemize}
    \item RQ1: Can AI agents self-identify \aislop (\S\ref{subsec:rq1}) ?
    \item RQ2: How do variants of \algoG perform on reducing \aislop ? And how do they compare against agentic minimization (\S\ref{subsec:rq2})?
    % \item RQ3: How does \algoG compare against agentic minimization (\S\ref{subsec:rq2}) ?
    % \item RQ3: Does \algo generalize across agentic scaffolds (\S\ref{subsec:rq3}) ?
    \item RQ3: How similar are \algoG and \algoNG patches (\S\ref{subsec:rq3})? 
    \item RQ4: How does \algo compare to patch minimization algorithms (\S\ref{subsec:rq4})?  
    \item RQ5: Does \algo generalize to non-security~\rayb{Why suddenly security?} benchmarks (\S\ref{subsec:rq5})? 
\end{itemize}

\subsection{RQ1: Can AI agents self-identify \aislop ?}
\label{subsec:rq1}

\noindent \textbf{Setup.} We use Live-kBench and trajectories from four scaffolds - \crashfixer, \swe, \mini, and \openhands. We then use \mini paired with Gemini-3-Flash as an agentic minimization baseline. We provide the agent with the \texttt{run\_kernel} tool to perform patch validation, by using the ``kernel environment (kEnv)" docker image from Live-kBench. We run the minimization agent for a maximum time budget of $6$ hours and a budget of $5.6\$$ per trajectory using the three configurations below.
%\franjo{Is the budget in terms of actual dollars or something like tokens that are converted into dollars?} 
%\alex{actual dollars}
 
\begin{itemize}
\item \texttt{Only Diff}: In this setting, the agent is provided with the bug artifacts and the original agent patch, and is explicitly asked to minimize the patch. 
\item \texttt{Only Traj}: Similar to \texttt{Only Diff}, except that instead of the agent patch, we provide the trajectory $Traj$. 
\item \texttt{Both}: Where we provide both inputs to the agent.
\end{itemize}

% \begin{table}
% \centering
% \caption{\% of Agentic Minimized Live-kBench Patches filtered out due to failing criteria}
% \label{tab:filtered_out}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   cell{1}{3} = {c},
%   cell{1}{4} = {c=4}{c},
%   cell{3}{2} = {r=4}{},
%   cell{7}{2} = {r=4}{},
%   cell{11}{2} = {r=4}{},
%   hlines,
%   vlines,
% }
%   &        &                & \% of Invalid $\mathcal{MP}$ in each Category &               &                     &                      & Total   \\
%   & \makecell[tc]{Min \\ Type}       & Agent          & Anomaly                                     & \makecell[tl]{File \\ Mismatch} & \makecell[tl]{Bug \\ Triggered} & \makecell[tl]{Patch  \\ Length $\uparrow$} &         \\
% 1 & \makecell[tc]{Min \\ Diff}  & CrashFixer     & 2.1\%                                       & 0.5\%         & 2.5\%               & 0.5\%                & 5.6\%   \\
% 2 &           & SWE Agent      & 1.0\%                                       & 1.3\%         & 3.8\%               & 0.7\%                & \textbf{6.8\%}   \\
% 3 &           & Mini-SWE & 1.0\%                                       & 0.5\%         & 1.3\%               & 1.0\%                & 3.8\%   \\
% 4 &           & OpenHands      & 1.8\%                                       & 0.2\%         & 3.0\%               & 1.2\%                & 6.2\%   \\
% 5 & \makecell[tc]{Min \\ Both}  & CrashFixer     & 3.0\%                                       & 4.8\%         & 4.1\%               & 2.3\%                & 14.2\%  \\
% 6 &           & SWE Agent      & 1.6\%                                       & 6.2\%         & 6.1\%               & 3.6\%                & \textbf{17.5\%}  \\
% 7 &           & Mini-SWE & 1.5\%                                       & 3.0\%         & 3.8\%               & 3.8\%                & 12.1\%  \\
% 8 &           & OpenHands      & 1.2\%                                       & 3.1\%         & 5.2\%               & 2.1\%                & 11.6\%  \\
% 9 & \makecell[tc]{Min \\ Traj}  & CrashFixer     & 2.1\%                                       & 8.0\%         & 11.1\%              & 11.9\%               & 33.1\%  \\
% 10 &          & SWE Agent      & 3.2\%                                       & 14.6\%        & 14.6\%              & 12.5\%               & \textbf{44.9\%}  \\
% 11 &          & Mini-SWE & 1.8\%                                       & 4.8\%         & 8.3\%               & 10.6\%               & 25.5\%  \\
% 12 &          & OpenHands      & 3.0\%                                       & 5.5\%         & 12.2\%              & 16.5\%               & 37.2\%  
% \end{tblr}
% }
% \vspace{-5mm}
% \end{table}


\begin{table}[h]
\centering
\caption{\% of Agentic Minimized Patches in Live-kBench filtered out due to failing criteria. Crash (\crashfixer), Mini (\mini), SWE (\swe), and OH (\openhands) are the four scaffolds.~\rayb{What is total?}}
\label{tab:filtered_out}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccc}
\toprule
\rowcolor{gray!15}
 & & \multicolumn{4}{c}{\textbf{\% of Invalid Minimizations in each Category}} & \\
\cmidrule(lr){3-6}
\rowcolor{gray!15}
\textbf{\makecell{Agentic \\ Setting}} & \textbf{Scaffold} & \textbf{Anomaly} & \textbf{\makecell{File \\ Mismatch}} & \textbf{\makecell{Bug \\ Triggered}} & \textbf{\makecell{Patch \\ Length $\uparrow$}} & \textbf{Total} \\
\midrule
\multirow{4}{*}{\makecell{Only \\ Diff}} & Crash & 2.1\% & 0.5\%  & 2.5\%  & 0.5\%  & 5.6\%  \\
 & SWE & 1.0\% & 1.3\%  & 3.8\%  & 0.7\%  & \textbf{6.8\%}  \\
 & Mini  & 1.0\% & 0.5\%  & 1.3\%  & 1.0\%  & 3.8\%  \\
 & OH  & 1.8\% & 0.2\%  & 3.0\%  & 1.2\%  & 6.2\%  \\
\midrule
\multirow{4}{*}{\makecell{Only \\ Traj}} & Crash & 2.1\% & 8.0\%  & 11.1\% & 11.9\% & 33.1\% \\
 & SWE & 3.2\% & 14.6\% & 14.6\% & 12.5\% & \textbf{44.9\%} \\
 & Mini  & 1.8\% & 4.8\%  & 8.3\%  & 10.6\% & 25.5\% \\
 & OH  & 3.0\% & 5.5\%  & 12.2\% & 16.5\% & 37.2\% \\
\midrule
\multirow{4}{*}{\makecell{Both}} & Crash & 3.0\% & 4.8\%  & 4.1\%  & 2.3\%  & 14.2\% \\
 & SWE & 1.6\% & 6.2\%  & 6.1\%  & 3.6\%  & \textbf{17.5\%} \\
 & Mini  & 1.5\% & 3.0\%  & 3.8\%  & 3.8\%  & 12.1\% \\
 & OH  & 1.2\% & 3.1\%  & 5.2\%  & 2.1\%  & 11.6\% \\
\bottomrule
\end{tabular}
}
% \vspace{-5mm}
\end{table}

\noindent \textbf{Results.} We study two key aspects of agentic minimization. 

\noindent \textbf{(1) \% Successful Minimization.} The first is the effect of neural non-determinism. As seen in Table \ref{tab:filtered_out}, a large \% of ``minimized patches" are unsuccessful as they fail at least one of the success criteria detailed in \S\ref{subsec:problem_statement}. The four failure modes we identify are (i) \textit{Anomaly} - the agent increases patch length by more than a $100$ lines, (ii) \textit{File Mismatch} - the agent modifies a new file not present in the original, (iii) \textit{Bug Triggered} - the agent over-minimizes and as a result reintroduces the bug, and (iv) \textit{Patch Length $\uparrow$} - the agent increases patch length, though not as extreme as the anomalies. All these failures together categorize a meaningful number of instances as ``unsuccessful minimizations".

We see the highest failure rate for \texttt{Only Traj} ($25.5\%$-$44.9\%$), followed by \texttt{Both} ($11.6\%$-$17.5\%$), and finally \texttt{Only Diff}  ($3.8\%$-$6.8\%$). Thus, neural models, given their non-determinism, frequently fail to minimize patches successfully.

% \begin{table}[h]
% \centering
% \caption{Live-kBench \patchdiff \% for Agentic Minimization (+ Filters) on all scaffold-min-type combinations.}
% \label{tab:agent_min_results}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%    hlines,
%    vlines,
% }

%   Min-Type & CrashFixer & SWE Agent & OpenHands & Mini-SWE Agent \\
%   Min-Diff & 4.0\%      & 2.0\%     & 3.1\%     & 2.4\%          \\
%   Min-Both & 2.2\%      & 2.6\%     & 2.4\%     & 6.4\%          \\
%   Min-Traj & \textbf{11.4\%}     & \textbf{11.0\%}    & \textbf{14.1\%}    & \textbf{12.2\%}     

% \end{tblr}
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Live-kBench \% \patchdiff for all agentic scaffolds using (i) Agentic Minimization (+ Filters) with different min-type combinations \& (ii) \algoG with different minimization granularity.
%~\rayb{use this table format for all the tables}
}
\label{tab:agent_min_results}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\rowcolor{gray!15}
 & \textbf{Crash-} & \textbf{SWE } & \textbf{Open-} & \textbf{Mini-SWE } \\
\rowcolor{gray!15}
 & \textbf{Fixer} & \textbf{Agent} & \textbf{Hands} & \textbf{ Agent} \\
\midrule
\rowcolor{gray!15}
\midrule
\multicolumn{3}{l}{ \textbf{Agentic Minimization \patchdiff}\% } & & \\
Only Diff & 4.0\% & 2.0\% & 3.1\% & 2.4\% \\
Only Traj & \textbf{11.4\%} & \textbf{11.0\%} & \textbf{14.1\%} & \textbf{12.2\%} \\
Both & 2.2\% & 2.6\% & 2.4\% & 6.4\% \\
\midrule
\rowcolor{gray!15}
\midrule
\multicolumn{3}{l}{ \textbf{\algoG Minimization \patchdiff}\% } & & \\
Sequence  & 15.0\%  & 4.8\%  & 10.4\%   & 16.2\%         \\
\textit{Hybrid} & 20.7\%    & 8.3\%     & 15.6\%    & 16.7\%  \\
Edit  & \textbf{30.1}\%    & \textbf{17.3\%}    & \textbf{24.0\%}    & \textbf{23.8\%}  \\
$\times$ Ratio $\uparrow$ & \textbf{2.6x}       & \textbf{1.6x}      & \textbf{1.7x}      & \textbf{2.0x} \\
\bottomrule
\end{tabular}
}
\vspace{-1mm}
\end{table}

\noindent \textbf{(2) \% \patchdiff Results.} After considering the original patch as the fallback value for all unsuccessful minimizations in Table \ref{tab:filtered_out}, we arrive at \% \patchdiff results in Table \ref{tab:agent_min_results}. As seen, while \texttt{Only Traj} shows meaningful \patchdiff results ($11$-$14.1\%$), both \texttt{Only Diff} \& \texttt{Both}  are not effective. 
%We note that the corresponding results (without filtering) were much less performant.


\subsection{RQ2: How much does \algoG reduce \aislop ? And how do they compare against agentic minimization?}
\label{subsec:rq2}
\textbf{Setup.} We run \algoG on Live-kBench for all agentic scaffolds. To measure the impact of minimization granularity, we run two versions of the \algoG algorithm. The first stops at the edit-sequence level (i.e. $\mathcal{E}$). The second is the complete \algoG that runs until the edit-action level. We also show results for a \textit{hybrid} approach, which uses a policy to select between the sequence-level and edit-action level results based on the characteristics of the minimized patch. Specifically, \textit{hybrid} chooses the sequence-level minimized patch only if a single sequence remains after sequence-level minimization \shobini{Maybe one sentence giving the intuition why?}.

% \begin{table}[h]
% \centering
% \caption{Live-kBench \patchdiff \% for \algoG with different minimization granularity.}
% \label{tab:trajmin_results}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   hlines,
%   vlines,
% }
%   Strategy                     & CrashFixer & SWE Agent & OpenHands & Mini-SWE Agent \\
%   \algoG (Node)                  & 15.0\%     & 4.8\%     & 10.4\%    & 16.2\%         \\
%   \algoG (Hybrid)                & 20.7\%    & 8.3\%     & 15.6\%    & 16.7\%         \\
%   \algoG (Edit)                  & \textbf{30.1}\%    & \textbf{17.3\%}    & \textbf{24.0\%}    & \textbf{23.8\%}         \\
%   Min-Traj (Agentic)   & 11.4\%     & 11.0\%    & 14.1\%    & 12.2\%         \\
%   Improvement Ratio $\uparrow$        & \textbf{2.6x}       & \textbf{1.6x}      & \textbf{1.7x}      & \textbf{2.0x}           
% \end{tblr}
% }
% % \vspace{-5mm}
% \end{table}


\textbf{\% \patchdiff Results.} As shown in Table \ref{tab:agent_min_results}, the edit-action level \algoG achieves the most aggressive minimization with \% \patchdiff of $17.3$-$30.1\%$. This is a meaningful improvement over the best agentic minimization results (\texttt{Only Traj})—the relative improvement ranging from $60\%$ to $160\%$.  Thus \algoG can aggressively minimize across agentic scaffolds. Table \ref{tab:agent_min_results} also depicts how different phases minimize patches to different extents. As expected, the edit-action level minimization is the most aggressive, the sequence-level minimization is the least, and \textit{hybrid} is in between. 

\textbf{Note}. As \algo is deterministic, every minimization is valid. 
%In the cases where $\mathcal{AP}$ cannot be minimized, \algo will safely return the original $\mathcal{AP}$.

% \begin{table}[h]
% \centering
% \caption{Live-kBench Oracle Performance for \algoG: Equivalent Patch \& Crash Resolved Rate}
% \label{tab:oracle_check}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   hlines,
%   vlines,
% }
%   Strategy                     & CrashFixer \alex{Curr NG}          & SWE Agent           & OpenHands           & Mini-SWE Agent      \\
%   Unminimized                  & 22.47\%             & 23.03\%             & 21.54\%             & 20.04\%             \\
%   Node-Level                  & 25.09\% \textcolor{improvgreen}{(+2.62)}     & 23.41\% \textcolor{improvgreen}{(+0.38)}     & 21.72\% \textcolor{improvgreen}{(+0.18)}     & 20.22\% \textcolor{improvgreen}{(+0.18)}     \\
%   Hybrid                & 25.66\% \textcolor{improvgreen}{(+3.19)}     & 23.41\% \textcolor{improvgreen}{(+0.38)}     & 21.72\% \textcolor{improvgreen}{(+0.18)}     & 20.41\% \textcolor{improvgreen}{(+0.37)}     \\
%   Edit-Level                  & 23.60\% \textcolor{improvgreen}{(+1.13)}     & 22.85\% (-0.18)     & 20.41\% (-1.13)     & 19.66\% (-0.38)   
% \end{tblr}
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Live-kBench Oracle Performance for \algoG: \% of patches equivalent to human fix \& that resolve the crash 
%\alex{CrashFixer results need to be changed}
}
\label{tab:oracle_check}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\rowcolor{gray!15}
 & \multicolumn{4}{c}{\textbf{Equivalent Patch \& Crash Resolved Rate}} \\
\cmidrule(lr){2-5}
\rowcolor{gray!15}
\textbf{Strategy/} & \textbf{Crash}& 
\textbf{SWE} & \textbf{Open} & \textbf{MiniSWE} \\
\rowcolor{gray!15}
\textbf{Phase} & \textbf{Fixer} & 
\textbf{Agent} &  \textbf{Hands} &  \textbf{Agent} \\
% \midrule
Agent Patch & 22.47\% & 23.03\% & 21.54\% & 20.04\% \\
Sequence  & 24.91\% \textcolor{improvgreen}{(+2.44)} & 23.41\% \textcolor{improvgreen}{(+0.38)} & 21.72\% \textcolor{improvgreen}{(+0.18)} & 20.22\% \textcolor{improvgreen}{(+0.18)} \\
\textit{Hybrid}   & 25.09\% \textcolor{improvgreen}{(+2.62)} & 23.41\% \textcolor{improvgreen}{(+0.38)} & 21.72\% \textcolor{improvgreen}{(+0.18)} & 20.41\% \textcolor{improvgreen}{(+0.37)} \\
Edit  & 23.41\% \textcolor{improvgreen}{(+0.94)} & 22.85\% (-0.18) & 20.41\% (-1.13) & 19.66\% (-0.38) \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\end{table}


\textbf{Oracle Performance.} We also note that \algoG's efficacy comes at almost no cost to the oracle performance (Table \ref{tab:oracle_check}). 
For Live-kBench, the oracle performance is evaluated by running the crash-inducing script and the LLM judge. Minimizations that resolve the crash and are deemed identical to the human patch by the LLM judge pass the oracle check. 

As seen, for certain scaffolds like \crashfixer, \algoG improves the oracle performance ($\sim$$1\%$-$2.6\%$). We attribute this rise in part to \crashfixer's evaluation setting. As \crashfixer accesses the correct buggy file a priori \cite{mathai2025crashfixer}, its patches are often a superset of the human fix. Thus, minimizing slop brings the patches closer to the human fix, increasing LLM judge equivalence. 

The other scaffolds work in an unassisted setting, allowing the agent patches to be markedly different than the human fix. Thus, for these scaffolds, the aim is to decrease \aislop without causing a drop in oracle performance.
As shown in Table \ref{tab:oracle_check}, \algoG achieves this nuance, despite aggressive minimization. For sequence-level and \textit{hybrid}, the oracle performance is roughly constant. For the edit-action level, this is broadly true except for a minimal drop of $1\%$ in \openhands.

% \subsection{RQ2: Does \algo generalize across agentic scaffolds?}
% \label{subsec:rq3}
% \textbf{Setup.} Lorem Ipsum is simply dummy text. Lorem Ipsum is simply dummy text.
% \textbf{Results.} Lorem Ipsum is simply dummy text. Lorem Ipsum is simply dummy text.

\subsection{RQ3: How similar are \algoG and \algoNG patches?} 
\label{subsec:rq3}
\textbf{Setup.} We compare the patches from two \algo variants - (i) \algoNG (without one-minimal guarantee), and (ii) \algoG (with guarantees). To study the impact of the one-minimal guarantee, we measure the difference in the \patchdiff metric and the additional cost incurred to provide minimality guarantees.

% \begin{table}[h]
% \centering
% \caption{Comparison between minimization results using \algoG and \algoNG}
% \label{tab:to_g_or_not_to_g}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   hlines,
%   vlines,
% }
%   Variant  & \patchdiff \% & Avg $E$/$\mathcal{MP}$ & $O$ check  & \% Identical & Cost (\# $TF$) \\
%   \algoNG & 28.1\%    & 1.35      & 23.60\% &    \SetCell[r=2]{c} 96.4\%          & 2386 \\
%   \algoG    & 30.1\%    & 1.35      & 23.78\% &  & 2578 \\
% \end{tblr}
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Comparison between \algoG and \algoNG minimized patches.}
\label{tab:to_g_or_not_to_g}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\rowcolor{gray!15}
& & \textbf{Avg} & & \textbf{\%} & \textbf{Cost} %\textbf{\makecell{Cost \\ (\# $TF$)}} 
\\
\rowcolor{gray!15}
\textbf{Variant} & \textbf{\patchdiff \%} & \textbf{$E$ / Patch} & \textbf{Check} & \textbf{Identical} & \textbf{(\# $TF$)} \\
%\midrule
\algoNG & 28.1\% & 1.35 & 23.60\% & \multirow{2}{*}{96.4\%} & 2386 \\
\algoG  & 30.1\% & 1.35 & 23.41\% &                         & 2578 \\
\bottomrule
\end{tabular}
}
\vspace{-1mm}
\end{table}

\textbf{Results.} As shown in Table \ref{tab:to_g_or_not_to_g}, the difference in \patchdiff \% between the variants is only $2\%$. Other minimization measures, like average edits per patch and oracle performance, are nearly identical. The cost (\# of kernel jobs) incurred when running these variants differs by only about $8\%$. 
Thus, in practice, ensuring a one-minimal guarantee does not incur much additional cost despite \algoG's quadratic theoretical bound. 
%This is empirical evidence that although \algoG has a theoretical quadratic cost complexity, in practice, the extra cost is not much higher. 
Conversely, \algoNG---which has a linear cost complexity, is as performant as \algoG for most trajectories ($96.4\%$ of patches are identical). Hence, for time-sensitive applications, where a guaranteed turnaround time is important (even for adversarial inputs), \algoNG is an obvious choice.
% However, more importantly, \algoNG is a linear-cost and linear-time algorithm, while \algoG is quadratic. Hence, for extremely time-sensitive applications, \algoNG \textbf{guarantees} an excellent turnaround time (even in the worst case), while producing patches that are almost equivalent to \algoG (as noted empirically).  

\subsection{RQ4:  How does \algo compare to patch minimization algorithms?}
\label{subsec:rq4}
\textbf{Setup.} We empirically study the cost of running all the variations of \algo and compare them to a derived baseline we call DD-Hunk (Delta Debugging Hunk Minimization). To implement DD-Hunk, we clone a popular optimized implementation of Delta Debugging \cite{picire}. We then make small modifications to the core algorithm to perform hunk minimization instead of change-set minimization, leaving the rest untouched. We then run DD-Hunk on \crashfixer's trajectories and measure the extent of minimization and the number of test file invocations. We compare this against all variants of \algo to understand the tradeoff between cost and \patchdiff \%.

% \begin{table}[h]
% \centering
% \caption{Cost (\# kernel jobs) of running \algo's variants and DD-Hunk Baseline on \crashfixer trajectories for Live-kBench}
% \label{tab:cost}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   cell{1}{1} = {c},
%   cell{1}{2} = {c=3}{c},
%   cell{1}{5} = {c=3}{c},
%   hlines,
%   vlines,
% }
%                             & \algoNG                          &                                  &                                  & \algoG      &             &                                  & DD-Hunk \\
%                             & Sequence                             & Hybrid                           & Edit                             & Sequence        & Hybrid      & Edit                             & Hunk \\
%   \patchdiff                & $11.2\%$                           & $19.2\%$                         & $28.1\%$                         & $15\%$    & $20.7\%$ & $30.1\%$                         & $27.3\%$ \\
%   Cost (\# $TF$)            & $927$                            & $1401$                      & $2386$                             & $1221$        & $1495$ & $2578$                             & $5192$ \textcolor{regressred}{($2 \times$)}
% \end{tblr}
% }
% \end{table}

% %%%%%%%% Temporarily Commented Out %%%%%%%%
% \begin{table}[h]
% \centering
% \caption{Cost (\# kernel jobs) of running \algo's variants and DD-Hunk Baseline on \crashfixer trajectories for Live-kBench}
% \label{tab:cost}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccccc}
% \toprule
% \rowcolor{gray!15}
%  & \multicolumn{3}{c}{\textbf{\algoNG}} & \multicolumn{3}{c}{\textbf{\algoG}} & \textbf{DD-Hunk} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
% \rowcolor{gray!15}
%  Metric & \textbf{Sequence} & \textbf{Hybrid} & \textbf{Edit} & \textbf{Sequence} & \textbf{Hybrid} & \textbf{Edit} & \textbf{Hunk} \\
% % \midrule
% \patchdiff     & $11.2\%$ & $19.2\%$ & $28.1\%$ & $15.0\%$ & $20.7\%$ & $30.1\%$ & $27.3\%$ \\
% Cost (\# $TF$) & $927$ & $1401$ & $2386$ & $1221$ & $1495$ & $2578$ & $5192$\,\textcolor{regressred}{($2\times$)} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
\centering
\resizebox{0.7\columnwidth}{!}{

% \begin{tikzpicture}
% \begin{axis}[
%     width=\columnwidth, height=7.6cm,
%     xlabel={Cost (\# kernel jobs, $TF$)},
%     ylabel={\patchdiff\ (\%)},
%     xmin=600, xmax=5800,
%     ymin=8,  ymax=33,
%     xtick={1000,2000,3000,4000,5000},
%     xticklabels={1k,2k,3k,4k,5k},
%     grid=both,
%     grid style={gray!18},
%     legend pos=south east,
%     legend cell align=left,
%     legend style={font=\footnotesize, fill=white, draw=gray!40},
%     label style={font=\small},
%     tick label style={font=\footnotesize},
% ]
% \addplot[mark=*, thick, blue!70!black, mark size=2.4pt, line join=round] coordinates {
%     (927, 11.2) (1401, 19.2) (2386, 28.1)
% };
% \addlegendentry{\algoNG}

% \addplot[mark=square*, thick, improvgreen, mark size=2.4pt] coordinates {
%     (1221, 15.0) (1495, 20.7) (2578, 30.1)
% };
% \addlegendentry{\algoG}

% \addplot[only marks, mark=triangle*, regressred, mark size=4pt] coordinates {
%     (5192, 27.3)
% };
% \addlegendentry{DD-Hunk}

% % ---- stage names ----
% \node[font=\scriptsize, anchor=west] at (axis cs:1015,12.8) {Sequence};
% \node[font=\scriptsize, anchor=west] at (axis cs:1560,19.6) {Hybrid};
% \node[font=\scriptsize, anchor=west] at (axis cs:2720,29.0) {Edit};

% % ---- exact values: TRIM-NG (blue), stacked, down-and-right ----
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west] at (axis cs:955,11.1)  {0.9k\\11.2\%};
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west] at (axis cs:1430,18.9) {1.4k\\19.2\%};
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west] at (axis cs:2415,27.8) {2.4k\\28.1\%};

% % ---- exact values: TRIM-G (green), stacked, up-and-left ----
% \node[font=\scriptsize, improvgreen, align=center, anchor=east]       at (axis cs:1190,16.4) {1.2k\\15.0\%};
% \node[font=\scriptsize, improvgreen, align=center, anchor=south east] at (axis cs:1455,21.2) {1.5k\\20.7\%};
% \node[font=\scriptsize, improvgreen, align=center, anchor=south east] at (axis cs:2545,30) {2.6k\\30.1\%};

% % ---- DD-Hunk label + value ----
% \node[font=\scriptsize\bfseries, regressred, align=center, anchor=east] at (axis cs:5070,27.3) {DD-Hunk\\[1pt]\mdseries 5.2k\\27.3\%};

% % ---- 2x cost annotation ----
% \draw[<->, regressred, dashed, thick]
%     (axis cs:2578,23.0) -- (axis cs:5192,23.0);
% \node[regressred, font=\scriptsize\bfseries, fill=white, inner sep=1.5pt, anchor=south]
%     at (axis cs:3885,23.0) {$\approx 2\times$ cost};
% \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     width=\columnwidth, height=7.6cm,
%     xlabel={Cost (\# kernel jobs, $TF$)},
%     ylabel={\patchdiff\ (\%)},
%     xmin=600, xmax=5800,
%     ymin=8,  ymax=33,
%     xtick={1000,2000,3000,4000,5000},
%     xticklabels={1k,2k,3k,4k,5k},
%     grid=both,
%     grid style={gray!18},
%     legend pos=south east,
%     legend cell align=left,
%     legend style={font=\footnotesize, fill=white, draw=gray!40},
%     label style={font=\small},
%     tick label style={font=\footnotesize},
% ]
% % ---- "better than DD-Hunk" dominance region (behind everything) ----
% \fill[improvgreen, opacity=0.18] (axis cs:600,27.3) rectangle (axis cs:5192,33);
% \addplot[mark=*, thick, blue!70!black, mark size=2.4pt, line join=round] coordinates {
%     (927, 11.2) (1401, 19.2) (2386, 28.1)
% };
% \addlegendentry{\algoNG}
% \addplot[mark=square*, thick, improvgreen, mark size=2.4pt] coordinates {
%     (1221, 15.0) (1495, 20.7) (2578, 30.1)
% };
% \addlegendentry{\algoG}
% \addplot[only marks, mark=triangle*, regressred, mark size=4pt] coordinates {
%     (5192, 27.3)
% };
% \addlegendentry{DD-Hunk}
% % ---- DD-Hunk quality level (reference line) ----
% \draw[regressred, dashed, semithick] (axis cs:600,27.3) -- (axis cs:5192,27.3);
% % ---- region label ----
% \node[font=\scriptsize\itshape, improvgreen!55!black, align=center]
%     at (axis cs:4020,30.3) {\textbf{Better than DD-Hunk:}\\\textbf{lower cost, higher \patchdiff}};
% % ---- stage names ----
% \node[font=\scriptsize, anchor=west] at (axis cs:1015,12.8) {\textbf{Sequence}};
% \node[font=\scriptsize, anchor=west] at (axis cs:1560,19.6) {  \textbf{Hybrid}};
% \node[font=\scriptsize, anchor=west] at (axis cs:2720,28.7) {
% \textbf{Edit}};
% % ---- exact values: TRIM-NG (blue), stacked, down-and-right ----
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west] at (axis cs:955,11.1)  {0.9k\\11.2\%};
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west] at (axis cs:1430,18.9) {1.4k\\19.2\%};
% \node[font=\scriptsize, blue!70!black, align=center, anchor=north west, fill=white, inner sep=0.8pt] at (axis cs:2415,27.8) {2.4k\\28.1\%};
% % ---- exact values: TRIM-G (green), stacked, up-and-left ----
% \node[font=\scriptsize, improvgreen, align=center, anchor=east]       at (axis cs:1190,16.4) {1.2k\\15.0\%};
% \node[font=\scriptsize, improvgreen, align=center, anchor=south east] at (axis cs:1455,21.2) {1.5k\\20.7\%};
% \node[font=\scriptsize, improvgreen, align=center, anchor=south east] at (axis cs:2545,30) {2.6k\\30.1\%};
% % ---- DD-Hunk label + value (below the point; line runs unbroken into the marker) ----
% \node[font=\scriptsize\bfseries, regressred, align=center, anchor=north] at (axis cs:5192,26.7) {DD-Hunk\\[1pt]\mdseries 5.2k\\27.3\%};
% % ---- 2x cost annotation ----
% \draw[<->, regressred, dashed, thick]
%     (axis cs:2578,21.0) -- (axis cs:5192,21.0);
% \node[regressred, font=\scriptsize\bfseries, fill=white, inner sep=1.5pt, anchor=south]
%     at (axis cs:3885,21.0) {$\approx 2\times$ cost};
% \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[
    width=\columnwidth, height=7.6cm,
    xlabel={Cost (\# kernel jobs, $TF$)},
    ylabel={\patchdiff\ (\%)},
    xmin=600, xmax=5800,
    ymin=8,  ymax=33,
    xtick={1000,2000,3000,4000,5000},
    xticklabels={1k,2k,3k,4k,5k},
    grid=both,
    grid style={gray!18},
    legend pos=south east,
    legend cell align=left,
    legend style={font=\footnotesize, fill=white, draw=gray!40},
    label style={font=\small},
    tick label style={font=\footnotesize},
]
\addplot[mark=*, thick, blue!70!black, mark size=2.4pt, line join=round] coordinates {
    (927, 11.2) (1401, 19.2) (2386, 28.1)
};
\addlegendentry{\algoNG}
\addplot[mark=square*, thick, improvgreen, mark size=2.4pt] coordinates {
    (1221, 15.0) (1495, 20.7) (2578, 30.1)
};
\addlegendentry{\algoG}
\addplot[only marks, mark=triangle*, regressred, mark size=4pt] coordinates {
    (5192, 27.3)
};
\addlegendentry{DD-Hunk}
% ---- DD-Hunk quality level (reference line) ----
\draw[regressred, dashed, semithick] (axis cs:600,27.3) -- (axis cs:5192,27.3);
% ---- region label ----
\node[font=\scriptsize\itshape, improvgreen, align=center]
    at (axis cs:4020,30.8) {\textbf{Better than DD-Hunk:}\\\textbf{lower cost, higher \patchdiff}};
% ---- stage names ----
\node[font=\scriptsize, anchor=west] at (axis cs:1015,12.8) {Sequence};
\node[font=\scriptsize, anchor=west] at (axis cs:1560,19.6) {Hybrid};
\node[font=\scriptsize, anchor=west] at (axis cs:2720,29.0) {Edit};
% ---- exact values: TRIM-NG (blue), stacked, down-and-right ----
\node[font=\scriptsize\bfseries, blue!70!black, align=center, anchor=north west] at (axis cs:955,11.1)  {0.9k\\11.2\%};
\node[font=\scriptsize\bfseries, blue!70!black, align=center, anchor=north west] at (axis cs:1430,18.9) {1.4k\\19.2\%};
\node[font=\scriptsize\bfseries, blue!70!black, align=center, anchor=north west, fill=white, inner sep=0.8pt] at (axis cs:2415,27.8) {2.4k\\28.1\%};
% ---- exact values: TRIM-G (green), stacked, up-and-left ----
\node[font=\scriptsize\bfseries, improvgreen, align=center, anchor=east]       at (axis cs:1200,16.4) {1.2k\\15.0\%};
\node[font=\scriptsize\bfseries, improvgreen, align=center, anchor=south east] at (axis cs:1455,21.2) {1.5k\\20.7\%};
\node[font=\scriptsize\bfseries, improvgreen, align=center, anchor=south east] at (axis cs:2545,30) {2.6k\\30.1\%};
% ---- DD-Hunk label + value (below the point; line runs unbroken into the marker) ----
\node[font=\scriptsize\bfseries, regressred, align=center, anchor=north] at (axis cs:5192,26.7) {DD-Hunk\\[1pt]\mdseries 5.2k\\27.3\%};
% ---- 2x cost annotation ----
\draw[<->, regressred, dashed, thick]
    (axis cs:2578,21.0) -- (axis cs:5192,21.0);
\node[regressred, font=\scriptsize\bfseries, fill=white, inner sep=1.5pt, anchor=south]
    at (axis cs:3885,21.0) {$\approx$ 2$\times$ COST};
\end{axis}
\end{tikzpicture}

}
\caption{\patchdiff\% vs Cost for \algo's variants and DD-Hunk on \crashfixer\ trajectories (Live-kBench). 
\algo variants reach comparable \patchdiff at half the cost of DD-Hunk.}
\label{fig:cost}
\vspace{-3mm}
\end{figure}

\textbf{Results.} As seen in Figure \ref{fig:cost}, our most effective combination---\algoG at edit-action level minimizes patches by $30.1\%$ while spending $\sim2.5k$ kernel jobs. Similarly, DD-Hunk minimizes patches by $27.3\%$ but for \textbf{twice} the cost ($\sim5.2k$ kernel jobs). Thus, reasoning over a structured search space like $Traj_R$ allows for much higher efficiency gains than blind search. Figure \ref{fig:cost} also depicts the relation between the \patchdiff \% and cost. 
\algoNG at the sequence-level has the lowest \patchdiff \% ($11.2$) and thus the lowest cost ($\sim0.9k$ kernel jobs). On the other end, \algoG at the edit-level has the highest \patchdiff \% ($30.1\%$) and the highest cost ($\sim2.5k$ kernel jobs). Thus, a user can choose a \algo variant based on the allocated budget. Larger budgets afford higher \patchdiff.

\subsection{RQ5: Does \algo generalize to non-security benchmarks?}
\label{subsec:rq5}
\textbf{Setup.} To test whether \algo generalizes beyond security patches (like Linux vulnerabilities), we run \algo on $333$ \swe  (Claude-Sonnet-4) trajectories for SWE-Bench-Verified \cite{jimenez2023swe}. We download these trajectories from the SWE-Bench Leaderboard, which verified that they pass the oracle test. As mentioned in \S\ref{subsec:rq_setup}, the test files $TF$ are the tests that \swe authored and ran during the trajectory. The oracle $O$ is a hidden fail-to-pass test suite, which \algo never sees. Using this, we run \algoG at the edit-action level and measure \patchdiff\% in Table \ref{tab:swebench_pdiff}. 

\textbf{Why SWE-Bench generalizes Live-kBench.} Live-kBench is an ideal testbed for
minimization because of four properties unique to kernel testing:  feedback request parsing is (i) \textit{well-defined} (every $FR$ is a \texttt{run\_kernel} call), (ii) the test file is
\emph{singular} (one crash-reproducing script), and (iii) \emph{static} (its content never changes)---(iv) thus making each feedback request identical. The same does not hold for SWE-Bench.

\textbf{(1)} \emph{Feedback Request parsing is ill-defined.} Python is easy to test. Hence, \swe performs validation in many ways---running existing suites, creating test files, inline \texttt{python -c} commands, and throwaway shell scripts. \textbf{Solution.} We harden our trajectory pre-processing to recognize multiple test invocation actions---including \texttt{pytest}, \texttt{python <script>.py}, \texttt{python -c}, or \texttt{python -m} etc.

\textbf{(2)} \emph{Multiple TFs.} Over the course of a trajectory, an agent invokes many feedback requests (described previously) to test its implementation thoroughly. Thus, it uses many intermediary test files, resulting in many $TF$s. We have seen instances where agents use more than $10$ test files for a repair trajectory. However, some of these test files turn ``stale" as the agent discards erroneous or incomplete 
%\shobini{erroneous or incomplete, maybe? sometimes the test will be partially correct not fully comprehensive.}
%\alex{solved}
hypotheses. Hence, we need to \textit{select valid test files}. \textbf{Solution.} To solve this, we run all the test files against the final submitted patch, retaining only those that pass on the final solution. This removes stale tests.

\textbf{(3)} \emph{Evolving Tests.} Test files do not stay constant during a trajectory. As agents routinely update their own test files mid-trajectory, the tests undergo transformations. \textbf{Solution.} When a test file is edited more than once, we pin the $TF$ to its final version at the end of the trajectory, rather than recording multiple versions.

\textbf{(4)} \emph{Each feedback request is unique.} During the trajectory, the agent invokes different subsets of test files to test aspects of its implementation. As such, each feedback request is unique. \textbf{Solution.} We analyze each feedback request and only associate the executed test files with it. Typically, a single feedback request calls up to three test files ($TF$s). %\shobini{should we use the notation for TFs here?}.
% \alex{solved}

\textbf{Note.} Using the above solutions in the trajectory pre-processing phase, we can generalize \algo to non-security domains, leaving the core algorithm untouched.

% \begin{itemize}
% \item \emph{Feedback Request parsing is ill-defined.} Python is easy to test. Hence, \swe performs validation in many ways---running existing suites, creating test files, inline \texttt{python -c} commands, and throwaway shell scripts, so no single action marks an $FR$.

% \item \emph{Multiple Oracles.} Over the course of a trajectory, an agent invokes many feedback requests (described previously) to concretely test its implementation in different ways. Thus, it uses many intermediary test files, resulting in multiple oracles. We have seen instances of agents using more than $10$ unique oracle files for a repair trajectory. and each feedback request invokes only a subset (typically two or three) of them.

% \item \emph{The oracle is not static.} \swe edits its own test files mid-trajectory,
% so the same oracle exists in several versions.
% \end{itemize}

% \textbf{Adapting \algo to SWE-Bench.} We absorb all three issues during trajectory
% pre-processing (\S\ref{subsec:minimization_system}), leaving the algorithm of \S\ref{sec:min_algo} unchanged.

% \begin{itemize}
% \item \emph{Extracting candidate oracles.} We scan each feedback command for the
% \texttt{.py} files it names (stripping any \texttt{pytest} selector) and snapshot
% their content.

% \item \emph{Selecting a valid subset.} We run every command against the full submitted patch in the instance's Docker image and keep only those whose files resolve and exit successfully, so \algo minimizes against a non-empty $TF$ that is known to pass on $\mathcal{AP}$.

% \item \emph{Choosing the oracle version.} When a test file is edited more than once, we pin $TF$ to its final in-trajectory version rather than a moving target.

% \item \emph{Characterizing a feedback call.} A bash step is an $FR$ iff it matches a test invocation (\texttt{pytest}, \texttt{python <script>.py}, \texttt{python -c}, or \texttt{python -m}; these
% $FR$ delimit the semantic nodes. When testing a candidate we inject the selected oracle files (except where the candidate already modifies that path) and mark $TF$ satisfied only if every surviving command exits successfully, yielding the PASS/FAIL $Obs_{Env}$ that the rule engine $\mathcal{R}$ consumes, exactly as in the kernel setting.
% \end{itemize}


\textbf{Results.} Table~\ref{tab:swebench_pdiff} reports \patchdiff \% after accounting for the changes introduced by the SWE-Bench evaluation script, so reductions reflect solely the agent's own changes. 
We report two \patchdiff numbers. 
The first is the \patchdiff upper bound, derived by measuring the total line reduction, which is $63.5\%$. 
The second is the \patchdiff lower bound, derived by measuring the total line reduction in \textit{pre-existing codebase files} (thus we discard any new files), which is $20\%$---with $23.6\%$ of edits and $17.8\%$ of hunks removed.
%The \emph{upper bound} (no filtering, over the whole submitted patch) is a $63.5\%$ line reduction, \shobini{Alex, not sure how to phrase this inflated sounds bad.} inflated by \algo dropping entire throwaway reproduction scripts; the \emph{lower bound} (filtering to the pre-existing source and test files the agent edited) is still a $20.0\%$ line reduction, with $23.6\%$ of edits and $17.8\%$ of hunks removed. 
This $20.0\%$ is comparable to the $17.3\%$ that \algo achieves for \swe on Live-kBench at the same edit-action level granularity (Table~\ref{tab:agent_min_results}). Thus, \algo removes a similar amount of \aislop in a completely different domain. We also validate that \algo preserves the oracle performance on $327$ of the $330$ successful patches (only $3$ regress), and $18$ minimized patches are identical to the human fix, thus moving the agent's patch closer to the human's patch. \algo is thus not kernel or security-specific, generalizing across scaffolds and domains.

% \begin{table}[h]
% \centering
% \caption{SWE-Bench-Verified \patchdiff \% for \algo (edit-level) over the $327$
% oracle-preserved instances, after removing base-environment edits. ``Lines
% (whole)'' is the upper bound (no filtering); ``Lines (mod.\ files)'' is the lower
% bound, restricted to the pre-existing source and test files the agent edited.}
% \label{tab:swebench_pdiff}
% \resizebox{\linewidth}{!}{
% \begin{tblr}{
%   hlines,
%   vlines,
% }
%   Metric        & Edits  & Hunks  & Lines (whole)   & Lines (mod.\ files) \\
%   \patchdiff \% & 23.6\% & 17.8\% & \textbf{63.5\%} & 20.0\%
% \end{tblr}
% }
% \end{table}


\begin{table}[h]
\centering
\caption{SWE-Bench-Verified \patchdiff \% for \algo (edit-action level) over the $327$ oracle-preserved instances. ``Lines
(Total)'' is the \patchdiff upper bound (no filter); ``Lines (mod.\ files)'' is the \patchdiff lower bound---restricting minimization results to only pre-existing codebase files.}
\label{tab:swebench_pdiff}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\rowcolor{gray!15}
\textbf{Metric} & \textbf{Edits} & \textbf{Hunks} & \textbf{\makecell{Lines \\ (Total)}} & \textbf{\makecell{Lines \\ (Mod.\ files)}} \\
\midrule
\patchdiff \% & 23.6\% & 17.8\% & \textbf{63.5\%} & 20.0\% \\
\bottomrule
\end{tabular}
}
\end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{images/swe-bench-example.pdf}
% \caption{\shobini{to fix, this image is really small.} Agent patch ($\mathcal{AP}$) with \aislop generated by \swe with
% Claude-Sonnet-4 for SWE-Bench-Verified instance \texttt{sympy\_\_sympy-15017}, where \texttt{len()} of a rank-0 array wrongly returns $0$ instead of $1$. The agent edits three files with five hunks and nine trajectory edits, yet only a single one-line change (box with $\star$) is the true fix: it replaces \texttt{functools.reduce(lambda x,y: x*y, shape) if shape else 0} with the empty-product identity \texttt{functools.reduce(lambda x,y: x*y, shape, 1)}. \algo drops four of the five semantic nodes during node-level minimization and then prunes the survivors during the file- and edit-level phases ($9 \to 3 \to 2 \to 1$ edits), leaving only the $\star$ edit. The resulting $\mathcal{MP}$ is byte-identical to the committed fix $\mathcal{HP}$ and preserves the hidden oracle ($1/1$ fail-to-pass, $14/14$ pass-to-pass). This mirrors the kernel motivating example of Figure~\ref{fig:motiv_fig}, where \algo likewise recovers $\mathcal{HP}$ from \aislop.}
% \label{fig:swebench_example}
% \end{figure}




==> sections/backup/methodology_minimization_system.tex <==


\subsection{Minimization System}
\label{subsec:minimization_system}


\subsubsection{Trajectory Pre-Processing}
\label{subsec:preprocessing}

The first stage of the minimization system turns the agent's raw trajectory $Traj$ into the preprocessed trajectory $Traj'$ that the rest of \algo consumes (stage~\protect\blackcircled{2} of Figure~\ref{fig:system_overview}). $Traj$ records every action the agent took while solving the task, but most of those actions, such as searching the codebase, reading files, or listing directories, never change the code and are irrelevant to the agent patch $\mathcal{AP}$. Pre-processing scans $Traj$ and keeps only the two kinds of action that minimization needs: the edits $E$ the agent applied to the filesystem, and the feedback requests $FR$ at which it ran the task's test files $TF$ to ask the environment $Env$ whether its work so far was correct.

Recovering the edits $E$ is harness-specific, because each scaffold realizes an edit differently (Table~\ref{tab:defnitions}): \mini edits with \texttt{sed} commands, \swe and \openhands call a \texttt{str\_replace\_editor} tool, and \crashfixer calls a \texttt{replace} tool \shobini{To fix, Table uses a different font (italicized)}. We parse each harness's actions into one normalized edit record, namely the target file together with its before and after text, so that every later stage is agent-agnostic. We mark a feedback request $FR$ wherever the agent invokes the task's test files $TF$: for Linux kernel crashes this is the command that rebuilds and reruns the kernel, and for software issues it is the test command the agent itself wrote.

The difficulty is that not every applied edit survives into the submitted patch, because agents backtrack and $Traj$ records the backtracking verbatim. An agent
may undo an individual edit, revert a single file to its original contents with \texttt{git checkout} or \texttt{git restore}, discard all of its work with \texttt{git reset --hard}, or set work aside with \texttt{git stash} and restore
it later; it may also re-issue an edit that has no effect or repeat one it has already made. Pre-processing replays these so that $Traj'$ retains only the edits that are actually present in the final patch, in the order the agent applied them. We hold this step to a correctness criterion that we validate against the submitted patch: the surviving edits, applied in order, must reproduce the agent patch, i.e., $\mathcal{AP} = \operatorname{apply}(\mathcal{APE})$. This guarantees that, among the edits, pre-processing removes only non-editing actions (searches, file reads, listings) together with edits the agent later reverted or that had no effect, and never drops an edit the final patch depends on, which is what makes the intermediate representation $Traj\mathcal{IR}$ built next (Section~\ref{subsec:ir}) faithful to what the agent submitted.


$Traj'$ is the preprocessed trajectory, $E$ is an edit, $FR$ is a feedback request. For the sake of illustration, we qualify each edit $E$ as $E_{\langle feedback\_id \rangle \langle edit\_id \rangle}^{\langle file\_name \rangle}$ to explicitly show that this edit is applied to $file\_name$ and is the $edit\_id^{th}$ edit applied before the $feedback\_id^{th}$ feedback request.

$Traj' \gets [ E_{11}^{D}, FR_{1}, E_{21}^{A}, E_{22}^{B}, FR_{2}, E_{31}^{C}, E_{32}^{C}, FR_{3},
E_{41}^{B}, \\ E_{42}^{E}, FR_{4}, E_{51}^{A}, FR_{5}]$

In this trajectory the agent edits file $D$ and requests feedback ($FR_{1}$), edits files $A$ and $B$ and requests feedback again $FR_{2}$, makes two edits to file $C$ before $FR_{3}$, edits files $B$ and $E$ before $FR_{4}$, and finally edits file $A$ before its last feedback request $FR_{5}$. These subscripts follow the same $E_{\langle feedback\_id \rangle \langle edit\_id \rangle}$ convention as the motivating example of Figures~\ref{fig:agent_traj} and~\ref{fig:motiv_fig}, where \swe makes five edits ($E_{11}$, $E_{21}$, $E_{31}$, $E_{32}$, $E_{33}$) across its three feedback requests, grouped as the semantic node patches
$\{E_{11}\}$, $\{E_{21}\}$, and $\{E_{31}, E_{32}, E_{33}\}$. The only addition here is the file superscript: the edits of Figure~\ref{fig:motiv_fig} all lie in
one file, whereas ours are spread across files $A$ through $E$. \shobini{Alex, does this ground the motivating example correctly?} The preprocessed trajectory $Traj'$ is the input to the intermediate representation $Traj\mathcal{IR}$ that \algo minimizes (Section~\ref{subsec:ir}).

%Traj\mathcal{IR} \gets [\{E_{11}^{D}\}, \{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \\ \{E_{51}^{A}\}]$
% After MinimizeNodeSuffix (remove node 1)
% $[\{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\},
% \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$
% After node-level reduce (remove node 3)
% $[ \{E_{21}^{A}, E_{22}^{B}\},
% \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$
% Afer group-by-file
% $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{22}^{B}, E_{41}^{B} \}, \{ E_{42}^{E} \}  ]$
% After file-level reduce (remove file B)
% $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{42}^{E} \}  ]$
% After edit-level reduce (remove $E_{42}$)
% $E \gets [E_{21}^{A}, E_{42}^{E}, E_{51}^{A}]$
% $\mathcal{MPE} \gets [E_{21}^{A}, E_{51}^{A}]$



\subsubsection{Intermediate Representation}
\label{subsec:ir}
After successfully preprocessing $Traj$, we massage the extracted information into a structured intermediate representation called $Traj\mathcal{IR}$.  As explained above, the pre-processed trajectory $Traj'$ is an ordered sequence of edits and feedback requests carefully extracted from $Traj$. What remains is to formalize this representation into an IR that \algo can consume.

To do so, we introduce boundaries in $Traj'$ that are derived from requests for feedback ($FR$). Thus, a representative grouping of the above $Traj'$ example would be $[\{E_{11}^{D}\}, \{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$ - which we refer to as $Traj\mathcal{IR}$. For the sake of compactness, we denote each grouping as a semantic node patch (or $np_{i}$).
Thus $NP = \langle np_1, \ldots, np_{|NP|} \rangle$.
We use the term ``semantic node patch'' because, upon manual analysis, we find that the agent often implements and tests a unique ``overarching hypothesis'' (or thought)
in each semantic node. Thus, $Traj\mathcal{IR}$ is the list of semantic node patches $NP$ where  $NP = \langle np_1, \ldots, np_{|NP|} \rangle$ and each $np_i$ encompasses the edits made between $FR_{i-1}$ and $FR_{i}$. Moreover, $\textsc{Flatten}($NP$)$ should be equal to $\mathcal{APE}$ (the agent patch as edits) to ensure that all the important trajectory edits are present (\textsc{Flatten} converts a nested structure to one long list). In the next section, we use $Traj\mathcal{IR}$ to run our algorithm \algo.

\subsubsection{Minimization Algorithm}
\label{sec:min_algo}
In this section, we elaborate on the key insights behind our minimization algorithm (\algo) and also expand on all the implementation details that make it work. 

\textbf{(i) Key Insight} \label{sec:minimization} A repair trajectory typically contains far more edits than the fix actually requires: exploratory attempts, abandoned approaches, and incidental changes accumulate alongside the edits that carry the fix. These extraneous edits, when applied to the codebase, result in a larger than anticipated patch length - i.e. $\operatorname{len}(\mathcal{AP})$.
Our main conjecture in this paper is that a principled way to reduce $\operatorname{len}(\mathcal{AP})$ is to derive from $Traj\mathcal{IR}$ a minimized subset of patch edits ($\mathcal{MPE}$), that when applied, resolves the bug and compacts patch length (i.e. $\operatorname{len}( \operatorname{apply}( \mathcal{MPE}))<\operatorname{len}(\mathcal{AP})$). More specifically, our goal is to recover $\mathcal{MPE}$ - a \emph{one-minimal} (see \S\ref{subsec:algorithmic_analysis}) edit subset that resolves the bug and reduces \aislop. 

\textbf{(ii) Execution Invariant}. The important invariant we use in \algo is that the generated minimized patch must pass the agent's $TF$. As the oracle $O$ is hidden from the agent and the minimization procedure, this is the main invariance that guides \algo to \textbf{safely} reduce the patch length. However, exploiting this invariance is not free, as executing $TF$ in slow (or unobservable) environments can be very expensive (explained below). Thus, beyond the \patchdiff metric, it is also important to track the number of $TF$ executions to measure the efficiency of a minimization algorithm. 


\textbf{(iii) Costs}. The central constraint in \aislop minimization is the cost of executing the test files $TF$ invoked via a feedback request ($FR$). In some settings this feedback is expensive: resolving a Linux kernel crash, for instance, requires building the patched kernel ($20 min$) and then running a crash-reproducing script ($10 min$) before a verdict is reached — roughly 30 minutes per $TF$ \cite{mathai2024kgym}. Since a single complete minimization run issues many $FR$, this imposes two distinct costs. First, \textbf{wall-clock time}: a complete run accumulates these latencies serially and can take tens of hours per task (and up to a week), too slow to be practical. Second, \textbf{monetary cost}: each $FR$ consumes costly high-performance compute, so minimizing \aislop at scale quickly becomes prohibitively expensive. This key constraint guides our algorithmic design, as we aim for \algo to be both effective at patch minimization as well as efficient and cost-effective. 

\textbf{(iv) Coarse to Fine Minimization}. With the above in mind, we design an algorithm that takes advantage of the unique characteristics of our representation $Traj\mathcal{IR}$. To minimize the number of $TF$ executions, we progressively perform minimization at three granularities, with each subsequent granularity being \textit{finer} than the previous (see $node \rightarrow file \rightarrow edits$ in Algorithm \ref{alg:patchmin}). As shown in Algorithm \ref{alg:patchmin}, the inputs to \algo are the $Traj\mathcal{IR}$ (or $NP$), a flag to ensure a one-minimal guarantee (discussed later), a feedback receiver ($\mathcal{F}$), a rule engine ($\mathcal{R}$), and a truth table ($\mathcal{T}$).

\textbf{(v) Feedback Receiver} ($\mathcal{F}$): While we expand on most input parameters to \algo in later descriptions, we describe the feedback receiver here. As explained in previous sections, the agent routinely interacts with its environment $Env$ to receive feedback from $TF$. However, in \algo, we choose to perform minimization by collecting feedback not only from the agent's $Env$ but also from other ``constructed" environments that help ensure ``desirable" properties in the minimized patch.  We introduce $\mathcal{F}$ as a general abstraction to collect feedback from an arbitrary number of environments. $\mathcal{F}$ ensures that as we introduce additional environments, our core algorithm remains unchanged. In \algo, we add an extra constructed environment called $Env_{patch}$. $Env_{patch}$ takes as input a candidate patch and checks if the candidate patch is larger/smaller than the current smallest valid patch. During the minimization process, \algo uses this feedback to decide if it should update the value of the current best edit subset. While this version uses two environments, we envision future variants of \algo that use many other constructed environments (including LLM feedback).

\input{sections/Algorithms/final_algo.tex}

\input{sections/Algorithms/minimum_suffix.tex}

\input{sections/Algorithms/try_candidate.tex}

\input{sections/Algorithms/rule_engine.tex}

% \input{sections/Algorithms/reduce.tex}

% \input{sections/Algorithms/greedy_removal.tex}



\textbf{(vi) TrajMinimize-Overview}. Before diving into the weeds of \algo, we first provide a high-level overview of our algorithm to highlight its key steps. As seen in Algorithm \ref{alg:patchmin}, there are three main phases of minimization (coarser to finer). Lines $1-3$ perform minimization at the granularity of a semantic node patch. As a single semantic node patch can contain multiple edits affecting multiple files, this coarse granularity is an efficient means to drop many multi-file edits in one shot. After this, Lines $5-8$ perform minimization at the granularity of a file. This phase helps drop edits made to files unrelated to the bug. As the granularity in this phase is a file, it is possible to eliminate multiple edits affecting a single file in one shot. Finally, Lines $10-12$ perform minimization at the finest granularity of a single edit. At the end of this last phase, we derive $\mathcal{MPE}$ (Line $12$) - a subset of edits in $\mathcal{APE}$. \algo then returns $\mathcal{MP}$ by applying all the edits in $\mathcal{MPE}$. In what follows, we deep dive into each phase of \algo. We use $[\{E_{11}^{D}\}, \{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$ as our running example for the sake of illustration.


\textbf{(Phase 1) Node-level Minimization}. Algorithm \ref{alg:patchmin} begins with a call to \textit{MinimizeNodeSuffix} (Line $2$) - a subroutine performing minimization at the granularity of a semantic node patch. 

\textbf{(a) \textsc{MinimizeNodeSuffix}}: As depicted in Algorithm \ref{alg:minsuffix}, \textit{MinimizeNodeSuffix} returns the shortest semantic node suffix from $Traj\mathcal{IR}$ that passes the $TF$ and has shorter patch length. Line $1$ initializes the main variables with default values: $S_{best}$ (the current best edit subset) is set to $None$, and $k$ which determines the node suffix, is set to $|NP|$ - hence a single-node suffix as $S_k$ is derived from the suffix $np_{k}$ to $np_{|NP|}$. 

Lines $2$-$22$ iteratively perform the following steps: (i) increase the node suffix $S_k$ (Line $4$); (ii) call the \textsc{TryCandidate} routine (Line $9$) that saves the feedback from (a) running $TF$ with $S_{k}$ and (b) comparing $\operatorname{len}(S_k)$ against the current shortest patch; (iii) apply the rule engine $\mathcal{R}$ on the received feedback (Line $11$) and depending on the decision, either drop the semantic node (Line $13$-$14$), break early (Line $17$-$18$) or continue searching for a valid/better suffix (Line $21$). With this overview, we expand on the helper routine \textsc{TryCandidate} and the rule engine $\mathcal{R}$ below.

\textbf{(b) \textsc{TryCandidate}}: As seen in Algorithm \ref{alg:trycandidate}, this routine takes as input: $S$ - a candidate subset of edits, and $\mathcal{F}$ - the feedback receiver. It then proceeds to apply the patch (Lines $2$-$5$), execute $\mathcal{F}$ (Line $7$), and return the feedback received (Lines $8$-$10$). It is important to repeat that $\mathcal{F}$ has access to two environments - the agent's $Env$ and a constructed environment $Env_{patch}$. $\mathcal{F}$ then performs two steps: (i) it executes $Env_{\operatorname{apply}(S)}(TF)$ to receive $Obs_{Env}$ - runtime feedback when running the test files $TF$, and (ii) it compares  $\operatorname{len}(\operatorname{apply}(S))$ to the current shortest patch length to receive $Obs_{patch}$. Both observations are then fed to $\mathcal{R}$ that decides on the next action.

\textbf{(c) Rule Engine ($\mathcal{R}$)}: The rule engine (Table \ref{tab:ruleengine}) showcases the example policy \algo follows when deciding to \textsc{KEEP}/\textsc{DROP} an edit or a semantic node. Future iterations of \algo can use more sophisticated and nuanced rule engines. As shown, using the two observations ($Obs_{patch}$ and $Obs_{Env}$), $\mathcal{R}$ drops an edit/node only if $TF$ is satisfied and the resultant patch has the shortest patch length. In all other cases, the edit/node is retained.

At the end of \textit{MinimizeNodeSuffix}, we receive $NP_{best}$ - a semantic node patch suffix s.t. the resultant patch passes $TF$ and is smaller in patch length than $\mathcal{AP}$. Using our running example, we can imagine that $np_1$ was removed (i.e. $\{E_{11}^{D}\}$), leaving the suffix $\langle np_2, ..., np_{5} \rangle$ which is $[\{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$.

\input{sections/Algorithms/reduce.tex}

\input{sections/Algorithms/greedy_removal.tex}

\textbf{(d) \textsc{Reduce}}: On Line $3$, \algo calls the \textsc{Reduce} routine (Algorithm \ref{alg:reduce}) on the previous output. As shown, the \textsc{Reduce} routine is a simple wrapper around \textsc{GreedyRemoval}; that functions differently based on $oneMin$ - a flag that determines if we ensure one-minimality (discussed later). \textsc{Reduce} calls \textsc{GreedyRemoval}  once if $oneMin=false$, else it calls \textsc{GreedyRemoval} repeatedly until its output reaches a fixed-point and stops changing. Currently, we assume $oneMin=false$.

\textbf{(e) \textsc{GreedyRemoval}}: Unlike \textsc{MinimizeNodeSuffix} that derives a suffix, \textsc{GreedyRemoval} derives a subsequence. As shown in Algorithm \ref{alg:greedy}, Lines $7$-$20$ iteratively perform the following procedure: (1) remove intermediate element (Line $8$),  (2) similar to \textsc{MinimizeNodeSuffix}, call \textsc{TryCandidate} to collect feedback, and then pass the feedback to the rule engine $\mathcal{R}$ (Lines $12$-$15$), and finally (3) depending on the decision either drop the element (Line $17$) or continue the for-loop (Line $7$). 
Using our running example, let us assume that $np_3$ is dropped in this invocation. So the resultant sequence is now $[ \{E_{21}^{A}, E_{22}^{B}\},
\{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$. This marks the end of the node-level minimization (phase 1), leaving us with three semantic nodes: [$np_2$, $np_4$, $np_5$].

\textbf{(Phase 2) File-level Minimization}. The next phase of minimization is at the file granularity. To perform this minimization step, we first need to re-order the input into ``file groups" (Line $5$). Using our running example, the value of $G$ would be $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{22}^{B}, E_{41}^{B} \}, \{ E_{42}^{E} \}  ]$. As seen, we create groupings based on the file names ($A$, $B$, $E$), but are careful to retain the order of the edits, i.e., $E_{21}^{A}$ comes before $E_{51}^{A}$. Then this is fed to the \textsc{Reduce} routine to drop edits made to unrelated files. Using our running example, assume that File $B$ was dropped. Hence, the resultant output would be  $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{42}^{E} \}  ]$. We now proceed to the final phase: edit-level minimization.

\textbf{(Phase 3) Edit-level Minimization}. This phase is the ``finest" granularity of minimization that we perform. To perform this step, we first flatten $G$ while respecting the edit order (Line $10$). Thus, $E \gets [E_{21}^{A}, E_{42}^{E}, E_{51}^{A}]$. We then pass $E$ to the \textsc{Reduce} routine to drop edits one at a time (Line $11$). Using our running example, assume that the edit $E_{42}^{E}$ is dropped. This would make the final edit subset $\mathcal{MPE}$ equal to $[E_{21}^{A}, E_{51}^{A}]$. Finally, we use the ``$\operatorname{apply}$" operator on $\mathcal{MPE}$ to get the minimized patch $\mathcal{MP}$. This is the outcome of \algo on our example with $oneMin=False$.

\textbf{One-minimal Guarantee}. Although the above algorithm is effective and efficient, it would be ideal to guarantee certain properties of our final output. Hence, we introduce the optional flag ($oneMin$) that enforces a \textit{one-minimal} guarantee. A set is said to be \textit{one-minimal} with respect to a property $P$, if removing any element in that set violates $P$. Thus, for \algo, if we can prove that removing any edit from $\mathcal{MPE}$ causes $TF$ to fail, then $\mathcal{MPE}$ is provably one-minimal. Thus, when the $oneMin$ flag is $true$, it changes the behavior of the \textsc{Reduce} routine.  Specifically, the flag triggers the Lines $4$-$8$ in Algorithm \ref{alg:reduce}. As seen, \textsc{Reduce} iteratively performs \textsc{GreedyRemoval} until a fix-point is reached, i.e., no more elements can be \textbf{safely} removed without failing $TF$. This, by construction, is the definition of \textit{one minimality}. Thus, the final outcome ($\mathcal{MPE}$) is one minimal when the flag is $true$.

==> sections/backup/methodology_system_overview.tex <==
% \subsection{System Overview}
% \label{subsec:system_overview}

% ~\protect\blackcircled{1}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{images/system-overview.pdf}
  \caption{Overview of \algo. A coding agent fixes a bug and emits two  artifacts: the agent patch $\mathcal{AP}$ and the trajectory $Traj$ that produced it, that is, the ordered sequence of actions it took, such as searching the code, inspecting files, editing code ($E$), and running the test files $TF$, where each run is a feedback request $FR$ that returns a pass/fail observation $Obs$~\protect\blackcircled{1}. Pre-processing keeps only the edits $E$ and the feedback requests $FR$, yielding the preprocessed trajectory $Traj'$; we lay $Traj'$ out as a sequence of edits ($E_1,\dots,E_5$) separated by the $FR$ at which the agent ran $TF$, and group the edits made between two consecutive $FR$ into one \emph{semantic node patch} $np_i$ (shown as Node~1--3), giving the intermediate representation $Traj\mathcal{IR}$~\protect\blackcircled{2}. \shobini{Alex, hopefully the use of semantic node patch before it's defined in IR section isn't confusing?} \algo then shrinks $\mathcal{AP}$ from coarse to fine, trying to remove whole node
  patches, then whole files, then single edits, and accepting each removal only when the candidate still passes $TF$ and $\operatorname{len}$ gets smaller~\protect\blackcircled{3}. We draw the patch as a stack of changed lines: the orange line is the fix and the gray lines are unrelated edits (\aislop) that are dropped until only the fix (marked $\star$) remains. The result is the
  minimized patch $\mathcal{MP}\subseteq\mathcal{AP}$ that still resolves the bug and, in this example, equals the human patch $\mathcal{HP}$; Section~\ref{sec:expr} reports \patchdiff and how often this match occurs~\protect\blackcircled{4}. The nodes and edits correspond to the motivating example of Figures~\ref{fig:agent_traj} and ~\ref{fig:motiv_fig}.}
  \label{fig:system_overview}
\end{figure*}



\subsection{System Overview}
\label{subsec:system_overview}

\algo is a system that takes one successful agent patch $\mathcal{AP}$ and removes the edits that are not needed to fix the bug, returning a minimized patch $\mathcal{MP} \subseteq \mathcal{AP}$ that still satisfies the agent's own test files. It does not depend on which agent produced $\mathcal{AP}$ or on which benchmark the bug comes from. Following the \patchmin setup of \S\ref{subsec:problem_formulation}, its inputs are the trajectory $Traj$, the agent patch $\mathcal{AP}$, the environment $Env$, and one or more test files $TF$. Its output is a minimized patch $\mathcal{MP} \subseteq \mathcal{AP}$ with $Env_{\mathcal{MP}}(TF) = \{pass\}$, obtained by reducing the \aislop carried in $\mathcal{AP}$. Figure~\ref{fig:system_overview} shows the four stages of the
pipeline. We outline the role of each stage below and develop the details in the sections that follow.

\noindent\protect\blackcircled{1}~\textbf{Solve the task.} A coding agent, such as \swe, \mini, \openhands, or \crashfixer, fixes the bug and returns two artifacts, the agent patch $\mathcal{AP}$ and the trajectory $Traj$. We treat the agent as a black box, which is what lets the system work with any agent scaffold.


\noindent\protect\blackcircled{2}~\textbf{Trajectory pre-processing and intermediate representation.} From $Traj$ we keep only the edits $E$ and the feedback requests $FR$ at which the agent ran its test files $TF$, discarding actions such as code searches and file reads that never change the patch (Section~\ref{subsec:preprocessing}). We then group the edits of the preprocessed trajectory $Traj'$ that lie between two consecutive $FR$ into a \emph{semantic node patch} $np_i$, giving the intermediate representation $Traj\mathcal{IR} = NP = \langle np_1, \ldots, np_{|NP|} \rangle$ that \algo consumes, where $\textsc{Flatten}(NP) = \mathcal{APE}$ (Section~\ref{subsec:ir}).

\noindent\protect\blackcircled{3}~\textbf{Minimizing the patch (coarse to fine).} \algo shrinks $\mathcal{AP}$ over $Traj\mathcal{IR}$ in three passes of decreasing granularity, whole semantic node patches, then whole files, then single edits, accepting a removal only when the candidate still passes $TF$ and $\operatorname{len}$ gets smaller. The surviving edits form $\mathcal{MPE}$, and $\mathcal{MP} = \operatorname{apply}(\mathcal{MPE})$. The algorithm, its feedback receiver $\mathcal{F}$ and rule engine $\mathcal{R}$, and its variants are given in Section~\ref{sec:min_algo}.

\noindent\protect\blackcircled{4}~\textbf{Oracle evaluation.} The minimized patch $\mathcal{MP}$ passes $TF$ by construction; here we additionally check that it introduces no oracle regressions, that is, $Env_{\mathcal{MP}}(O) = \{pass\}$ whenever $Env_{\mathcal{AP}}(O) = \{pass\}$. We report \patchdiff, the reduction in \aislop, and how often $\mathcal{MP}$ recovers the human patch $\mathcal{HP}$ in Section~\ref{sec:expr}.

==> sections/backup/motivation_and_formulation.tex <==
\section{Motivating Example \& Problem Formulation}

In this section, we study how \aislop manifests during an agent's trajectory (\S\ref{subsec:motivation}). We also formally define \aislop and the task of Slop Minimization (\S\ref{subsec:problem_formulation})\footnote{Concurrent work uses ``slop'' for a
related but distinct notion: \textsc{SlopCodeBench}~\cite{orlanski2026slop}
defines it as a \emph{static} quality property of the code an agent retains
(verbosity and structural erosion). Our \textsc{Code Slop} instead denotes
edits that are \emph{functionally redundant}---removable while tests still
pass---regardless of how clean the retained code looks. We discuss the
distinction below.}.

%We point out that the main reason behind \aislop is extraneous and unnecessary ``\textbf{agent edits}".

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\columnwidth]
    {images/agent_traj.pdf}
    \caption{An agent harness (left) \alex{agent traj and agent harness} that is provided a codebase, a bug report, and a set of tools. Using this, the agent makes edits and intermittently seeks feedback from the environment (right) until it receives a positive response (\texttt{PASS}). There is a 1-to-1 correspondence between the nodes and edits in the trajectory to the patch in Figure \ref{fig:motiv_fig}. Edit $1$ corresponds to $E_{11}$; Edit $2$ to $E_{21}$; Edits $3$-$5$ to $E_{31}$-$E_{33}$. Except for Edit $3$, all other edits are \aislop.~\rayb{VM shows Linux specific, shouldn't it be oracle setting?}}
    \label{fig:agent_traj}
\vspace{-5mm}
\end{figure}

\subsection{Motivating Example}
\label{subsec:motivation}

We begin with a real-world motivating example that illustrates how \aislop emerges during agent-driven program repair. Consider the trajectory (Figure~\ref{fig:agent_traj}) and resulting patch (Figure~\ref{fig:motiv_fig}) generated by \swe~\cite{yang2024swe} while fixing a Linux kernel vulnerability~\cite{mem_leak}. As shown in Figure~\ref{fig:agent_traj}, the agent does not arrive at the correct fix immediately. Instead, it iteratively modifies the code and validates its progress by running tests. The first attempt fails, prompting additional changes and another round of testing, which also fails. Only after making several further modifications does the agent finally obtain a passing result. The trajectory therefore captures not only the successful fix, but also the exploratory changes that helped the agent reach it.

% We begin with a real-world motivating example to showcase the main reason behind \aislop in AI-generated code. For our discussion, we analyze the trajectory  (Figure \ref{fig:agent_traj}) and patch (Figure \ref{fig:motiv_fig}) generated by  \swe \cite{yang2024swe} for the Linux vulnerability \cite{mem_leak}. As seen in Figure \ref{fig:agent_traj}, \swe makes a total of five edits when trying to resolve this vulnerability. It also intermittently requests feedback from the environment using test files to validate its edits. In this example, \swe makes ``Edit $1$", then runs tests (feedback request $1$) and sadly receives a \texttt{FAIL} signal. So it proceeds to make ``Edit $2$", runs tests (feedback request $2$) once more, only to receive \texttt{FAIL} yet again. Finally, it makes a string of edits ``Edits $3$-$5$" and then validates them by running tests (feedback request $3$) and receives a \texttt{PASS} feedback.

\begin{figure}[t]
    \includegraphics[width=\columnwidth]
    {images/motivating_example_3.pdf}
    % \caption{Agent patch ($\mathcal{AP}$) with \aislop generated from the trajectory in Figure \ref{fig:agent_traj} for the Linux vulnerability \cite{mem_leak}. We highlight with bounding boxes how each edit in the trajectory can be mapped to regions in the final patch. The only important portion of the patch (box with $\star$) has the ``Human Patch" ($\mathcal{HP}$) label and can be mapped to edit $E_{31}$. Our algorithm \algo reduces $\mathcal{AP}$ to $\mathcal{HP}$ by eliminating $E_{11}$ and $E_{21}$ during the node-level minimization phase, followed by edit-level minimization that removes $E_{32}$ and $E_{33}$. This leaves $E_{31}$, which is the $\mathcal{HP}$ hidden in the slop.}
    \caption{Agent-generated patch ($\mathcal{AP}$) for a Linux vulnerability~\cite{mem_leak}. Bounding boxes map edits from the trajectory in Figure~\ref{fig:agent_traj} to regions of the final patch. The starred region (edit $E_{31}$) corresponds to the human patch ($\mathcal{HP}$), while the remaining regions are \aislop---residual edits from the agent's search process. \algo removes these redundant edits, revealing the human-equivalent fix hidden within the larger patch.}
    \label{fig:motiv_fig}
    \vspace{-5mm}
\end{figure}

We pause here to highlight a problem. Although the agent succeeded by repeatedly editing and validating edits using runtime feedback, it is unclear what exactly fixed the vulnerability. As we show in Figure \ref{fig:motiv_fig}, the actual ground truth (human patch) lies buried in a sea of unrelated changes (i.e. \aislop). 

In Figure \ref{fig:motiv_fig}, we hypothetically draw a connecting line between the trajectory edits and the modified lines in the agent patch. For each edit, we draw an edit-specific bounding box for the set of modified lines it introduces in the final patch. As shown (see the box with $\star$), only three modified lines corresponding to $E_{31}$ (i.e., Edit $3$) are truly needed for this vulnerability and are equivalent to the human patch. Everything else is unnecessary and AI-generated \aislop. 

With AI agents contributing more than $50\%$ of code in enterprise software \cite{To Cite}, the problem of \aislop is genuinely monumental. If left unresolved, \aislop poses to be the biggest hurdle the SE community will face in the next decade. This work aims to pave the path towards the effective resolution of this problem.

\subsection{Problem Formulation}
\label{subsec:problem_formulation}

In this section, we (i) formally define the meaning of \aislop, (ii) introduce \slopmin - a new task to minimize \aislop, and finally (iii) highlight the main objective function of this paper (\patchmin), which serves as a generalizable dual formulation of \slopmin.
We intend for this formulation to serve as a standardized notation for code slop minimization, allowing future work to state its assumptions explicitly and to articulate concretely where and why its approach departs from prior ones. Before we proceed to actual definitions, we first introduce some common terminology used in coding agents in Table \ref{tab:defnitions}. This will help ground the formal definitions that follow.

\input{sections/paper_notation_definitions}

\aislop: Using the notations in Table \ref{tab:defnitions}, we first define \aislop for a given task $T$. We compute $\aislop$ for $T$ by comparing a successful $\mathcal{AP}$ with its equivalent human implementation ($\mathcal{HP}$). Thus, this definition by construction requires that we have 
access to both human and agent implementations for a given task $T$.
%assumes that for a given task $T$, we have access to both a human and an agent implementation. 
This is typically not true for most instances when users interact with AI agents; however, starting with this definition allows us to extend this definition to more realistic scenarios.
%\petros{Given that we're calling this "slop" I would cap it below at 0. Also I'd point out that humans sometimes generated extra edits for a task, e.g., comments or drive-by formatting, but we assume, as research has shown, that humans are closer to minimal.}
We define \aislop \petros{Maybe AI Slop instead of CodeSlop?} for task $T$ with test file $TF$ as the difference in patch length between a human's implementation ($\mathcal{HP}$) and the corresponding successful agent implementation ($\mathcal{AP}$).
\begin{equation}
\label{eqn:ai_slop}
 \aislop(T, \mathcal{AP}, \mathcal{HP}) = \operatorname{len}(\mathcal{AP}) - \operatorname{len}(\mathcal{HP})
\end{equation}
\noindent where $Env_{\mathcal{AP}}(TF) = \{Pass\}$. While we acknowledge that humans occasionally generate extra edits for a task (such as modifying comments or formatting code), recent research \alex{To Cite} has shown that, on average, human-authored implementations are significantly less verbose and thus closer to minimal than agent-generated code. Thus, \aislop is almost always positive. 
%\shobini{Alex, should we mark this as an observation rather than making this claim? could cite our own compaction numbers} 
This leads us to the formal task definition of code slop minimization (or \slopmin). In simple terms, the objective of \slopmin is to \textbf{minimize} \aislop for a given task $T$ and human patch $HP$ by enumerating over all possible subsets ($\mathcal{MP}$) of the original agent patch $\mathcal{AP}$.  
%\petros{It's not clear what a subset of a patch is. You probably mean "the patch of a subset of edits". Maybe define that above?}
%\petros{The SlopMinimize definition seems awkward. ALthough we want to compare its output to the human patch, it shouldn't be taking it as an input. It should take the oracle and the trajectory and output AP*. Then the definition of a good SlopMinimize is one that minimizes the slop (that's where HP comes in). Also, while we're at it, I think it makes more sense notationally for SlopMinimize to return AP*, since it's a process not a metric, rather than returning a code slop value.}
\alex{Petros, please re-read this section until here, I think you will find this to be better.}
\begin{equation}
\label{eqn:slop_min}
  \slopmin(T, \mathcal{HP}) =
  \argmin_{\mathcal{MP}}\;
  \aislop(T, \mathcal{MP}, \mathcal{HP})
\end{equation}
where $\operatorname{Env}_{\mathcal{MP}}(TF) = \{pass\}$ and $\mathcal{MP} \subseteq \mathcal{AP}$. 
%\shobini{define the atomic unit of the subset (edits? hunks? lines?) subset is measured in lines 2 sentences later}
%\alex{Shobini, please read the ``Patch length" paragraph now, it has all the necessary details I believe}
It is important to note that, as $\mathcal{HP}$ is a constant, $\operatorname{len}(\mathcal{HP})$ is also a constant, and so
%to minimize \aislop, we must effectively minimize $\operatorname{len}(\mathcal{MP})$ while retaining a \texttt{pass} on the oracle $O$. \petros{...while retaining a pass on the oracle, of course}. 
%Thus, 
the \slopmin task simplifies to deriving $\mathcal{MP}$ -- a subset of the original agent patch $\mathcal{AP}$ s.t. its patch length is minimal, and it still passes the oracle (see below). 
\begin{equation}
\label{eqn:slop_min_simple}
  \slopmin(T, \mathcal{HP}) = 
  \argmin_{\mathcal{MP}}\;
  \operatorname{len}(\mathcal{MP}) = \mathcal{AP}^{*}
\end{equation}
where $\operatorname{Env}_{\mathcal{MP}}(TF) = \{pass\}$ and $\mathcal{MP} \subseteq \mathcal{AP}$. As shown, we refer to the global minimum of this problem as $\mathcal{AP}^{*}$.
%\petros{It's not obvious why the minimal patch must be the patch from a subset of edits, rather than of hunks, or even individual lines. This is a constraints on the solution we have imposed, not an intrinsic constraint.}
%\alex{The above definition is measured in individual lines.}
% We refer to the global minimum of this problem as $\mathcal{AP}^{*}$ - the most minimal patch subset that still satisfies the oracle.
% \begin{equation}
% \label{eqn:slop_min}
% \begin{aligned}
%   \mathcal{AP}^{*} = {} &
%   \argmin_{\mathcal{AP}_i \subseteq \mathcal{AP}}
%   \slopmin(T, \mathcal{HP}) \\
%   & \text{s.t.} \quad
%   \operatorname{Env_{\mathcal{AP}_i}}(O) = \{pass\}
% \end{aligned}
% \end{equation}
% \begin{equation}
% \label{eqn:ap_star}
%   \mathcal{AP}^{*} =
%   \argmin_{\substack{\mathcal{MP} \subseteq \mathcal{AP}; \operatorname{Env}_{\mathcal{MP}}(O) = \{pass\}}}
%   \operatorname{len}(\mathcal{MP})
% \end{equation}
%\noindent Thus, by construction, $\slopmin(T, \mathcal{HP})=\mathcal{AP}^{*}$ 
% are closely related as shown below. 
% \begin{equation}
% \label{eqn:relation}
% \slopmin(T, \mathcal{HP}) = \aislop(T, \mathcal{AP}^{*}, \mathcal{HP})
% \end{equation}



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/problem-formulation.pdf}
    \caption{The duality of minimizing \aislop. The horizontal line measures patch verbosity. The extreme left is the original verbose agent patch ($\mathcal{AP}$) and on the extreme right is the compact human patch ($\mathcal{HP}$). In the middle is the minimized patch ($\mathcal{MP}$). To minimize \aislop, we can decrease the $\mathcal{MP} \rightarrow \mathcal{HP}$ distance 
    %between $\mathcal{AP}_{min}$ \& $\mathcal{HP}$ 
    (i.e. \slopmin), or conversely, we can increase the $\mathcal{AP} \rightarrow \mathcal{MP}$ distance (i.e. \patchmin). These are dual problems.
    }
    \label{fig:problem_formulation}
    % \shobini{in this figure, can we label with AP, AP\_min, HP in parentheses? This is a helpful visual}
    \vspace{-10pt}
\end{figure}

\textbf{Note:} Deriving the most minimal subset ($\mathcal{AP}^{*}$) from the original patch $\mathcal{AP}$ is a known NP-Hard problem~\cite{To Cite}. Hence, attempting to develop algorithms that \textit{always} derive  $\mathcal{AP}^{*}$ is a fruitless exercise. Instead, it is useful to derive algorithms (like \algo) that heuristically reduce the patch size while maintaining functional properties (like passing oracles). 
%And as such, most research that revolves around this problem are polynomial time algorithms that minimize patches with 

\textbf{Blind Setting.} While the above definitions are a useful starting point, they only apply to carefully curated coding benchmarks such as SWE-Bench, Live-kBench and SWE-Bench Pro where \textbf{pairs} of human-authored and agent-authored implementations co-exist. Thus, \slopmin is not directly applicable to a blind setting where the $\mathcal{HP}$ is unknown (referred to as $\mathcal{HP}_{unk}$) - which is often the case when a human user interacts with an AI agent. As such, to make slop minimization generalizable to the blind setting, we introduce a new metric - patch diff (or \patchdiff) and the corresponding task (\patchmin). As we prove below, \patchmin applies to the blind setting and is also a dual problem to \slopmin (see Figure \ref{fig:problem_formulation}). Formally, \patchdiff is defined as the difference in patch length between \agentp and \minp.
\begin{equation}
\label{eqn:patch_diff}
\patchdiff(T, \mathcal{AP}, \mathcal{MP}) = \operatorname{len}(\mathcal{AP}) - \operatorname{len}(\mathcal{MP}) 
\end{equation}
And, the objective of the task \patchmin is to optimize for \patchdiff.
\begin{equation}
\label{eqn:patch_min}
\patchmin(T, \mathcal{AP}) = \argmax_{\mathcal{MP}}  \patchdiff(T, \mathcal{AP}, \mathcal{MP}) 
\end{equation}
where $\operatorname{Env}_{\mathcal{MP}}(TF) = \{pass\}$ and $\mathcal{MP} \subseteq \mathcal{AP}$. As \agentp is a constant, \patchmin is optimized when \minp passes $TF$ and $\operatorname{len}(\mathcal{MP})$ is minimized, which, as we noted before, is the definition of $\mathcal{AP}^{*}$. Thus, the following equation holds.
\begin{equation}
\label{eqn:patch_min_simple}
\patchmin(T, \mathcal{AP}) = \argmin_{\mathcal{MP}} \operatorname{len}(\mathcal{MP}) = \mathcal{AP}^{*}
\end{equation}
\noindent where $\operatorname{Env}_{\mathcal{MP}}(TF) = \{pass\}$ and $\mathcal{MP} \subseteq \mathcal{AP}$. From Equation (\ref{eqn:slop_min_simple}) and (\ref{eqn:patch_min_simple}), the following duality is proved.
\begin{equation}
\label{eqn:duality}
\slopmin(T,\mathcal{HP}) = \patchmin(T, \mathcal{AP})
\end{equation}

\textbf{Duality}. Thus, solving for \patchmin results in the minimized patch $\mathcal{AP}^{*}$ which is also the global minimum of \slopmin. Hence, we can achieve our goal of slop minimization by optimizing for patch minimization. This is very intuitive (see Figure \ref{fig:problem_formulation}), because as the difference in patch length between $\mathcal{AP}$ and $\mathcal{MP}$ increases, the smaller the resultant patch $\mathcal{MP}$ and thus the lower the slop. Thus, for the remainder of this work, we consider \patchmin as our main optimization task and design algorithms for the same.
%, and hence we design algorithms to perform \patchmin.

\textbf{Generalization Note}.  As \patchmin does not depend on the human patch ($\mathcal{HP}$), it is a generalizable task (applicable for blind settings) that is a provably dual problem to \slopmin. 

\textbf{Degree of Success}. As it is challenging to always derive $\mathcal{AP}^{*}$, we measure an algorithm's success by how much it can reduce \aislop between \agentp and \minp (i.e., $\delaislop(T,\mathcal{AP},\mathcal{MP}) $). We show below that this is exactly equal to $\patchdiff(T, \mathcal{AP}, \mathcal{MP})$.
\begin{equation}
\label{eqn:delta_slop}
\begin{gathered}
  \delaislop(T, \mathcal{AP}, \mathcal{MP}) = \\
  \aislop(T, \mathcal{AP}, \mathcal{HP}_{\text{unk}})
  - \aislop(T, \mathcal{MP}, \mathcal{HP}_{\text{unk}}) \\
   = (\operatorname{len}(\mathcal{AP}) - \operatorname{len}(\mathcal{HP}_{unk})) - (\operatorname{len}(\mathcal{MP}) - \operatorname{len}(\mathcal{HP}_{unk})) \\
   = \operatorname{len}(\mathcal{AP}) - \operatorname{len}(\mathcal{MP}) \\
   = \patchdiff(T,\mathcal{AP}, \mathcal{MP})
\end{gathered}
\end{equation}

\noindent Hence, the higher the value of \patchdiff, the more the reduction in \aislop. Thus, in our experimental sections, we report and compare results in terms of \patchdiff.

\textbf{Hidden Oracle Equivalence}. As we explained above, the minimization procedure does not have access to the hidden oracle $O$, but instead has access to the agent's $TF$. However, for a minimization algorithm to be practical and useful, it should not introduce any oracle regressions. Hence, if $\mathcal{AP}$ is a successful patch ($Env_{\mathcal{AP}}(O)=\{pass\}$), then $\mathcal{MP}$ must also satisfy $O$ (i.e. $Env_{\mathcal{MP}}(O)=\{pass\}$). Thus, we measure the hidden oracle equivalence after running \algo, as a means to justify our practical utility.

\textbf{Minimization Setup}. We now discuss the exact setup for the task of slop minimization, so that we can concretely specify the inputs, outputs, metrics and success critera.

\begin{itemize}
\item \textit{Inputs}: When performing slop minimization, any algorithm has access to the following inputs - (i) the trajectory ($Traj$), (ii) the original agent patch $\mathcal{AP}$, (iii) the environment ($Env$), and (iv) one or more test files ($TF$) 
%\petros{It's not clear why we are bothering to call out "oracle files". Just call it "oracle"?}.

\item \textit{Output}: Using the inputs specified above, a minimization procedure outputs $\mathcal{MP}$ - a minimized version of $\mathcal{AP}$ s.t. $\mathcal{MP} \subseteq \mathcal{AP}$ and $Env_{\mathcal{MP}}(TF) = \{pass\}$.

\item \textit{Metrics}: We measure the extent of slop minimization for task $T$ and agent patch $\mathcal{AP}$ by calculating $\patchdiff(T, \mathcal{AP}, \mathcal{MP})$.

\item \textit{Success}: A minimization procedure is said to be successful if the output patch $\mathcal{MP}$ satisfies three criteria - (a) $\mathcal{MP} \subseteq \mathcal{AP}$, (b) $Env_{\mathcal{MP}}(O) = \{pass\}$ (if $Env_{\mathcal{AP}}(O) = \{pass\}$), and finally (c) $\operatorname{len}(\mathcal{MP}) \leq \operatorname{len}(\mathcal{AP})$. Note, we can quantify the ``degree" of success using \patchdiff, but a ``successful" minimization run must at the very least satisfy the above three conditions.
\end{itemize}

\noindent As shown in Figure \ref{fig:motiv_fig}, $\mathcal{MP} = \operatorname{apply}([E_{31}]) \subset \mathcal{AP}$, and thus $\operatorname{len}(\mathcal{MP}) < \operatorname{len}(\mathcal{AP})$. As we know, this truly fixes the vulnerability (the $O$ check), $\mathcal{MP}$ is a valid minimization.

\textbf{Task Uniqueness}.  It is important to compare and contrast this slop minimization task to other similar yet different problem statements. For example, there is a lot of research that performs minimization \textit{across} versions, historical change sets, or the commit history of a codebase. Delta-Debugging \cite{318773.318946} localizes failure-inducing changes \textit{across} versions - finding a 1-minimal subset of changes between a passing and failing configuration. Similarly, \texttt{git-bisect} \cite{git_bisect}  localizes a bug-inducing commit \textit{across} the commit history of a codebase.
% Delta-Debugging localizes a bug inducing commit (or BIC) by a smart search across commit history. Thus, it localizes the smallest code change that induces the current bug under inspection. 

In contrast, our work looks at edits made ``\textit{within}'' an \textit{agent commit}. Unlike ``human-authored'' commits that typically do not surface all of the developer's failed attempts at debugging the issue (often spanning numerous code searches and code edits that were filtered out from the final commit); an ``agent-authored'' commit often includes many breadcrumbs (or markers) that are remnants leftover during the agent's debugging process. This is often apparent if one manually inspects the agent trajectory. As such, the task of minimizing \aislop is unique as we now have a new granularity of minimization - ``multiple" \textbf{edits} that compose together to make a ``single'' \textbf{commit}. Interestingly, this also exposes minimization at a level that is finer than a ``hunk'', as it is plausible for multiple edits to affect the same hunk. All of the above nuances suggest that minimizing \aislop is truly a fresh, unique, and extremely relevant problem.

==> sections/methodology.tex <==
\section{Methodology}
\label{sec:method}

In this section, we deep dive into our end-to-end minimization system. We start with a system overview (\S\ref{subsec:system_overview}). We then elaborate on each system component, including data pre-processing and the \algo algorithm. Finally, we end with a theoretical analysis of two variants of \algo. 

% \input{sections/methodology_system_overview}

\input{sections/methodology_minimization_system}

\input{sections/methodology_algorithm_analysis}

==> sections/methodology_algorithm_analysis.tex <==
\subsection{Algorithmic Analysis}
\label{subsec:algorithmic_analysis}


\textbf{Cost Complexity}. As explained in \S\ref{sec:min_algo}, the central constraint to minimization is the cost of invoking $TF$. To understand the cost imposed by \algo, we estimate its \textit{cost complexity} ($\mathcal{C}$) as measured in the number of \textsc{TryCandidate} calls (equivalent to $TF$ invocations). $\mathcal{C}$ helps quantify how the cost of minimizing \agentp scales as the number of edits varies. For simplicity, we first derive the $\mathcal{C}$ of \algo \textit{without} guarantees, termed as \algoNG (i.e., no guarantee), followed by the complexity for \algoG (i.e., with one minimal guarantee)

The $\mathcal{C}$ of \algoNG is determined by the complexities of the individual sub-routines called in Algorithm \ref{alg:patchmin}. Hence, below, we first determine the $\mathcal{C}$ of each subroutine and then combine them to determine the final complexity.

\begin{itemize}
    \item \textsc{MinimumNodeSuffix}. As this algorithm has a \texttt{while} loop (Lines $2$-$22$) that runs at most $|NG|$ times, it can issue at most $|NG|$ invocations to \textsc{TryCandidate}. Hence, the cost complexity is $\mathcal{O}(|NG|)$.
    \item \textsc{Reduce} ($oneMin$ is $false$). With $oneMin$ set to $false$, \textsc{Reduce} simply calls \textsc{GreedyRemoval} once. As shown in Algorithm \ref{alg:greedy}, the maximum cost complexity in  \textsc{GreedyRemoval} is $\mathcal{O}(|V|)$ where $|V|$ is the number of elements in the input sequence. We arrive at this complexity as there is a single \texttt{for} loop (Lines $7$-$20$) that can run at most $|V|$ times.
    \item \textsc{GroupByFile}, \textsc{Flatten}, and ``$\operatorname{apply}$" are simple linear-time routines that iterate over their input sequence once, but do not call \textsc{TryCandidate}. As such, Lines $6$, $10$ and $12$ can be ignored.
\end{itemize}

\noindent With the above information in hand, the cost complexity for \algoNG $=$ $\mathcal{O}(|NP|)$ (Line $2$) + $\mathcal{O}(|NP|)$ (Line $3$) + $\mathcal{O}(|F|)$ (Line $7$, $F$ is the set of edited files) + $\mathcal{O}(|E|)$ (Line $11$). As $|E| >> |NP| > |F|$, the final cost complexity is $\mathcal{O}(|E|)$. Hence, the cost complexity grows \textbf{linearly} with the number of edits in $Traj\mathcal{IR}$. This proves that \algoNG is an extremely efficient algorithm.

The procedure to measure the cost complexity for \algoG is almost identical to the above process. The only difference is that we must derive the cost complexity for \textsc{Reduce} when $oneMin$ is $true$.

\begin{itemize}
\item \textsc{Reduce} ($oneMin$ is $true$). With $oneMin$ set to $true$, the Lines $4$-$8$ call \textsc{GreedyRemoval} repeatedly until its output stops changing and reaches a fix-point. In the worst case, \textsc{GreedyRemoval} can be invoked $|V|$ times, and as each \textsc{GreedyRemoval} itself has $\mathcal{O}(|V|)$ complexity, the final cost complexity is $\mathcal{O}(|V|^{2})$.
\end{itemize}


\noindent Thus, the cost complexity for \algoG $=$ $\mathcal{O}(|NP|)$ (Line $2$) + $\mathcal{O}(|NP|^{2})$ (Line $3$) + $\mathcal{O}(|F|^{2})$ (Line $7$, $F$ is the set of edited files) + $\mathcal{O}(|E|^{2})$ (Line $11$). As $|E| >> |NP| > |F|$, the final cost complexity is $\mathcal{O}(|E|^{2})$. Hence, the cost complexity grows \textbf{quadratically} with the number of edits in $Traj\mathcal{IR}$. The addition of this provable guarantee adds to the cost complexity of the minimization procedure.

In \S\ref{sec:expr}, we show empirically how the results from \algoNG and \algoG are almost identical. We also show that although the worst-case cost complexity grows from linear to quadratic, the increase in the number of \textsc{TryCandidate} calls is not as high. Thus, \textsc{Reduce} even with $oneMin$ set to $true$ is still \textit{empirically} linear time.  

\textbf{Time Complexity}. Similarly, it can be shown that the time complexity of \algoNG is $\mathcal{O(|E|)}$ and the time complexity of \algoG is $\mathcal{O}(|E|^{2})$.

==> sections/methodology_minimization_system.tex <==


\subsection{Minimization System}
\label{subsec:minimization_system}




\subsubsection{Minimization Algorithm}
\label{sec:min_algo}
In this section, we elaborate on the key insights behind our minimization algorithm (\algo) and also expand on all the implementation details that make it work. 

\textbf{(i) Key Insight} \label{sec:minimization} A repair trajectory typically contains far more edits than the fix actually requires: exploratory attempts, abandoned approaches, and incidental changes accumulate alongside the edits that carry the fix. These extraneous edits, when applied to the codebase, result in a larger than anticipated patch length - i.e. $\operatorname{len}(\mathcal{AP})$.
Our main conjecture in this paper is that a principled way to reduce $\operatorname{len}(\mathcal{AP})$ is to derive from $Traj\mathcal{IR}$ a minimized subset of patch edits ($\mathcal{MPE}$), that when applied, resolves the bug and compacts patch length (i.e. $\operatorname{len}( \operatorname{apply}( \mathcal{MPE}))<\operatorname{len}(\mathcal{AP})$). More specifically, our goal is to recover $\mathcal{MPE}$ - a \emph{one-minimal} (see \S\ref{subsec:algorithmic_analysis}) edit subset that resolves the bug and reduces \aislop. 

\textbf{(ii) Execution Invariant}. The important invariant we use in \algo is that the generated minimized patch must pass the agent's $TF$. As the oracle $O$ is hidden from the agent and the minimization procedure, this is the main invariance that guides \algo to \textbf{safely} reduce the patch length. However, exploiting this invariance is not free, as executing $TF$ in slow (or unobservable) environments can be very expensive (explained below). Thus, beyond the \patchdiff metric, it is also important to track the number of $TF$ executions to measure the efficiency of a minimization algorithm. 


\textbf{(iii) Costs}. The central constraint in \aislop minimization is the cost of executing the test files $TF$ invoked via a feedback request ($FR$). In some settings this feedback is expensive: resolving a Linux kernel crash, for instance, requires building the patched kernel ($20 min$) and then running a crash-reproducing script ($10 min$) before a verdict is reached — roughly 30 minutes per $TF$ \cite{mathai2024kgym}. Since a single complete minimization run issues many $FR$, this imposes two distinct costs. First, \textbf{wall-clock time}: a complete run accumulates these latencies serially and can take tens of hours per task (and up to a week), too slow to be practical. Second, \textbf{monetary cost}: each $FR$ consumes costly high-performance compute, so minimizing \aislop at scale quickly becomes prohibitively expensive. This key constraint guides our algorithmic design, as we aim for \algo to be both effective at patch minimization as well as efficient and cost-effective. 

\textbf{(iv) Coarse to Fine Minimization}. With the above in mind, we design an algorithm that takes advantage of the unique characteristics of our representation $Traj\mathcal{IR}$. To minimize the number of $TF$ executions, we progressively perform minimization at three granularities, with each subsequent granularity being \textit{finer} than the previous (see $node \rightarrow file \rightarrow edits$ in Algorithm \ref{alg:patchmin}). As shown in Algorithm \ref{alg:patchmin}, the inputs to \algo are the $Traj\mathcal{IR}$ (or $NP$), a flag to ensure a one-minimal guarantee (discussed later), a feedback receiver ($\mathcal{F}$), a rule engine ($\mathcal{R}$), and a truth table ($\mathcal{T}$).

\textbf{(v) Feedback Receiver} ($\mathcal{F}$): While we expand on most input parameters to \algo in later descriptions, we describe the feedback receiver here. As explained in previous sections, the agent routinely interacts with its environment $Env$ to receive feedback from $TF$. However, in \algo, we choose to perform minimization by collecting feedback not only from the agent's $Env$ but also from other ``constructed" environments that help ensure ``desirable" properties in the minimized patch.  We introduce $\mathcal{F}$ as a general abstraction to collect feedback from an arbitrary number of environments. $\mathcal{F}$ ensures that as we introduce additional environments, our core algorithm remains unchanged. In \algo, we add an extra constructed environment called $Env_{patch}$. $Env_{patch}$ takes as input a candidate patch and checks if the candidate patch is larger/smaller than the current smallest valid patch. During the minimization process, \algo uses this feedback to decide if it should update the value of the current best edit subset. While this version uses two environments, we envision future variants of \algo that use many other constructed environments (including LLM feedback).

\input{sections/Algorithms/final_algo.tex}

\input{sections/Algorithms/minimum_suffix.tex}

\input{sections/Algorithms/try_candidate.tex}

\input{sections/Algorithms/rule_engine.tex}

% \input{sections/Algorithms/reduce.tex}

% \input{sections/Algorithms/greedy_removal.tex}



\textbf{(vi) TrajMinimize-Overview}. Before diving into the weeds of \algo, we first provide a high-level overview of our algorithm to highlight its key steps. As seen in Algorithm \ref{alg:patchmin}, there are three main phases of minimization (coarser to finer). Lines $1-3$ perform minimization at the granularity of a semantic node patch. As a single semantic node patch can contain multiple edits affecting multiple files, this coarse granularity is an efficient means to drop many multi-file edits in one shot. After this, Lines $5-8$ perform minimization at the granularity of a file. This phase helps drop edits made to files unrelated to the bug. As the granularity in this phase is a file, it is possible to eliminate multiple edits affecting a single file in one shot. Finally, Lines $10-12$ perform minimization at the finest granularity of a single edit. At the end of this last phase, we derive $\mathcal{MPE}$ (Line $12$) - a subset of edits in $\mathcal{APE}$. \algo then returns $\mathcal{MP}$ by applying all the edits in $\mathcal{MPE}$. In what follows, we deep dive into each phase of \algo. We use $[\{E_{11}^{D}\}, \{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$ as our running example for the sake of illustration.


\textbf{(Phase 1) Node-level Minimization}. Algorithm \ref{alg:patchmin} begins with a call to \textit{MinimizeNodeSuffix} (Line $2$) - a subroutine performing minimization at the granularity of a semantic node patch. 

\textbf{(a) \textsc{MinimizeNodeSuffix}}: As depicted in Algorithm \ref{alg:minsuffix}, \textit{MinimizeNodeSuffix} returns the shortest semantic node suffix from $Traj\mathcal{IR}$ that passes the $TF$ and has shorter patch length. Line $1$ initializes the main variables with default values: $S_{best}$ (the current best edit subset) is set to $None$, and $k$ which determines the node suffix, is set to $|NP|$ - hence a single-node suffix as $S_k$ is derived from the suffix $np_{k}$ to $np_{|NP|}$. 

Lines $2$-$22$ iteratively perform the following steps: (i) increase the node suffix $S_k$ (Line $4$); (ii) call the \textsc{TryCandidate} routine (Line $9$) that saves the feedback from (a) running $TF$ with $S_{k}$ and (b) comparing $\operatorname{len}(S_k)$ against the current shortest patch; (iii) apply the rule engine $\mathcal{R}$ on the received feedback (Line $11$) and depending on the decision, either drop the semantic node (Line $13$-$14$), break early (Line $17$-$18$) or continue searching for a valid/better suffix (Line $21$). With this overview, we expand on the helper routine \textsc{TryCandidate} and the rule engine $\mathcal{R}$ below.

\textbf{(b) \textsc{TryCandidate}}: As seen in Algorithm \ref{alg:trycandidate}, this routine takes as input: $S$ - a candidate subset of edits, and $\mathcal{F}$ - the feedback receiver. It then proceeds to apply the patch (Lines $2$-$5$), execute $\mathcal{F}$ (Line $7$), and return the feedback received (Lines $8$-$10$). It is important to repeat that $\mathcal{F}$ has access to two environments - the agent's $Env$ and a constructed environment $Env_{patch}$. $\mathcal{F}$ then performs two steps: (i) it executes $Env_{\operatorname{apply}(S)}(TF)$ to receive $Obs_{Env}$ - runtime feedback when running the test files $TF$, and (ii) it compares  $\operatorname{len}(\operatorname{apply}(S))$ to the current shortest patch length to receive $Obs_{patch}$. Both observations are then fed to $\mathcal{R}$ that decides on the next action.

\textbf{(c) Rule Engine ($\mathcal{R}$)}: The rule engine (Table \ref{tab:ruleengine}) showcases the example policy \algo follows when deciding to \textsc{KEEP}/\textsc{DROP} an edit or a semantic node. Future iterations of \algo can use more sophisticated and nuanced rule engines. As shown, using the two observations ($Obs_{patch}$ and $Obs_{Env}$), $\mathcal{R}$ drops an edit/node only if $TF$ is satisfied and the resultant patch has the shortest patch length. In all other cases, the edit/node is retained.

At the end of \textit{MinimizeNodeSuffix}, we receive $NP_{best}$ - a semantic node patch suffix s.t. the resultant patch passes $TF$ and is smaller in patch length than $\mathcal{AP}$. Using our running example, we can imagine that $np_1$ was removed (i.e. $\{E_{11}^{D}\}$), leaving the suffix $\langle np_2, ..., np_{5} \rangle$ which is $[\{E_{21}^{A}, E_{22}^{B}\}, \{E_{31}^{C}, E_{32}^{C}\}, \{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$.

\input{sections/Algorithms/reduce.tex}

\input{sections/Algorithms/greedy_removal.tex}

\textbf{(d) \textsc{Reduce}}: On Line $3$, \algo calls the \textsc{Reduce} routine (Algorithm \ref{alg:reduce}) on the previous output. As shown, the \textsc{Reduce} routine is a simple wrapper around \textsc{GreedyRemoval}; that functions differently based on $oneMin$ - a flag that determines if we ensure one-minimality (discussed later). \textsc{Reduce} calls \textsc{GreedyRemoval}  once if $oneMin=false$, else it calls \textsc{GreedyRemoval} repeatedly until its output reaches a fixed-point and stops changing. Currently, we assume $oneMin=false$.

\textbf{(e) \textsc{GreedyRemoval}}: Unlike \textsc{MinimizeNodeSuffix} that derives a suffix, \textsc{GreedyRemoval} derives a subsequence. As shown in Algorithm \ref{alg:greedy}, Lines $7$-$20$ iteratively perform the following procedure: (1) remove intermediate element (Line $8$),  (2) similar to \textsc{MinimizeNodeSuffix}, call \textsc{TryCandidate} to collect feedback, and then pass the feedback to the rule engine $\mathcal{R}$ (Lines $12$-$15$), and finally (3) depending on the decision either drop the element (Line $17$) or continue the for-loop (Line $7$). 
Using our running example, let us assume that $np_3$ is dropped in this invocation. So the resultant sequence is now $[ \{E_{21}^{A}, E_{22}^{B}\},
\{E_{41}^{B}, E_{42}^{E}\}, \{E_{51}^{A}\}]$. This marks the end of the node-level minimization (phase 1), leaving us with three semantic nodes: [$np_2$, $np_4$, $np_5$].

\textbf{(Phase 2) File-level Minimization}. The next phase of minimization is at the file granularity. To perform this minimization step, we first need to re-order the input into ``file groups" (Line $5$). Using our running example, the value of $G$ would be $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{22}^{B}, E_{41}^{B} \}, \{ E_{42}^{E} \}  ]$. As seen, we create groupings based on the file names ($A$, $B$, $E$), but are careful to retain the order of the edits, i.e., $E_{21}^{A}$ comes before $E_{51}^{A}$. Then this is fed to the \textsc{Reduce} routine to drop edits made to unrelated files. Using our running example, assume that File $B$ was dropped. Hence, the resultant output would be  $[\{E_{21}^{A},E_{51}^{A}\}, \{ E_{42}^{E} \}  ]$. We now proceed to the final phase: edit-level minimization.

\textbf{(Phase 3) Edit-level Minimization}. This phase is the ``finest" granularity of minimization that we perform. To perform this step, we first flatten $G$ while respecting the edit order (Line $10$). Thus, $E \gets [E_{21}^{A}, E_{42}^{E}, E_{51}^{A}]$. We then pass $E$ to the \textsc{Reduce} routine to drop edits one at a time (Line $11$). Using our running example, assume that the edit $E_{42}^{E}$ is dropped. This would make the final edit subset $\mathcal{MPE}$ equal to $[E_{21}^{A}, E_{51}^{A}]$. Finally, we use the ``$\operatorname{apply}$" operator on $\mathcal{MPE}$ to get the minimized patch $\mathcal{MP}$. This is the outcome of \algo on our example with $oneMin=False$.

\textbf{One-minimal Guarantee}. Although the above algorithm is effective and efficient, it would be ideal to guarantee certain properties of our final output. Hence, we introduce the optional flag ($oneMin$) that enforces a \textit{one-minimal} guarantee. A set is said to be \textit{one-minimal} with respect to a property $P$, if removing any element in that set violates $P$. Thus, for \algo, if we can prove that removing any edit from $\mathcal{MPE}$ causes $TF$ to fail, then $\mathcal{MPE}$ is provably one-minimal. Thus, when the $oneMin$ flag is $true$, it changes the behavior of the \textsc{Reduce} routine.  Specifically, the flag triggers the Lines $4$-$8$ in Algorithm \ref{alg:reduce}. As seen, \textsc{Reduce} iteratively performs \textsc{GreedyRemoval} until a fix-point is reached, i.e., no more elements can be \textbf{safely} removed without failing $TF$. This, by construction, is the definition of \textit{one minimality}. Thus, the final outcome ($\mathcal{MPE}$) is one minimal when the flag is $true$.

==> sections/paper_notation_definitions.tex <==

% \begin{itemize}
% \item \textbf{User Instruction} ($\mathcal{UI}$) \& \textbf{Task} ($T$) - Users often provide natural language instructions ($\mathcal{UI}$) to LLM-based agents that concretely define a task ($T$) for the agent to implement, such as bug fixing, feature implementation, test generation, etc. In our motivating example (Figures \ref{fig:agent_traj} and \ref{fig:motiv_fig}), $T$ is the task to resolve the Linux Vulnerability and $\mathcal{UI}$ is the instructions associated with this task.

% \item \textbf{Agent Patch} (\agentp) \& \textbf{Minimized Patch} (\minp) - We term the final patch that an agent submits for a task $T$ as the agent patch (\agentp). In this work, we represent \agentp as the set of all of the modified (added and deleted) lines in the patch. As explained in previous sections, our main aim is to derive a minimized patch (\minp), which is a subset of \agentp, where ``subset" implies that the lines in \minp are a subset of the lines in \agentp (i.e. \minp $\subseteq$ \agentp). In our motivating example, $\mathcal{AP}$ is the entire patch seen in Figure \ref{fig:motiv_fig}, and $\mathcal{MP}$ is the box with the ``$\star$" containing three modified lines.
%However, \minp must still be functionally equivalent with respect to task criteria like task oracles (explained below).

% \item \textbf{Hidden Oracles} ($O$) - An oracle ($O$) for task $T$ is its ultimate judge of success. $O$ is used to generate the final success/failure verdict for every agent-generated patch. For some tasks like crash resolution in the Linux kernel \cite{mathai2024kgym}, $O$ is provided as part of the crash metadata. For other tasks like Github issue resolution \cite{deng2025swe}, $O$ is often a hidden fail-to-pass ($F2P$) test used for final benchmark evaluation. As $O$ is often hidden from the agent, it is also kept hidden from our minimization algorithm. However, it is ideal if our predicted minimized patch \minp satisfies $O$ if \agentp initially satisfied $O$. Thus, \textbf{minimization must not introduce any oracle regressions}.
%\shobini{Alex, this is SWE bench specific no? so the use of O in below formulas can be confusing} 
%\alex{Shobhi, how is it now?}
%(like temporary test files) so that each part of its implementation is thoroughly tested.   
%As explained below, oracles help agents collect finer-level feedback.
%\petros{Oracles are a little confusing here. Not all tests are oracles. Oracles are ultimate judges of success. An agent may produce some tests trying to approximate what the oracle would say, but not all tests are oracles. Oracles are privileged. Agents don't build privileged data from thin air. It would be good not to confuse oracles with testing during implementation.}
% \alex{Shobini and Petros, how is this now?}

% \item \textbf{Environments} ($Env$), \textbf{Feedback Requests} ($FR$), \textbf{Test Files} ($TF$), \& \textbf{Observations} ($Obs$) - When implementing a task $T$, LLM-based agents interact with their executable environments ($Env$) by issuing feedback requests ($FR$). A $FR$ is typically a bash command that invokes one (or many) test files ($TF$) that agents leverage ``mid-trajectory" as functional guardrails. For crash resolution in the Linux kernel \cite{mathai2024kgym}, the benchmark provides a fixed $TF$. For Github issue resolution \cite{deng2025swe}, ``\textit{during}'' the trajectory, the agent creates and executes many $TF$, to test each part of its implementation thoroughly.  Depending on the task, the $TF$ can remain static (or evolve) during the course of the agent's trajectory. When running these $TF$, the agent receives observations ($Obs$) such as (i) runtime feedback measuring functional correctness ($Env_{\mathcal{AP}}(TF)$), or (ii) compilation feedback like whether a patch compiles. This fine-grained feedback enables agents to course-correct mid-trajectory. Typically, the agent patch \agentp satisfies multiple $TF$ by the end of the trajectory, i.e., $Env_{\mathcal{AP}}(TF) =\{pass\}$. In our motivating example, the VM machine is the $Env$, the \texttt{PASS}/\texttt{FAIL} outcomes are the $ Obs$, and $FR$ is the set of ``feedback request" lines from the agent to the VM machine.
%In our algorithms, we leverage multiple environments (explained later) to assess if our minimization is proceeding in the right direction.  

% \item \textbf{Edits} ($E$) - To generate code that implements the task $T$, LLM-based agents make changes to their environment's filesystem by issuing ``edit'' actions. The exact realization of an ``edit'' depends on the specific agentic harness - for \mini \cite{yang2024swe} it is typically an \textit{sed} call, for \swe \cite{yang2024swe} and \openhands \cite{wang2024openhands} it is a call to the \textit{str\_replace\_editor} tool, and for \crashfixer \cite{mathai2025crashfixer} it is an invocation to the \textit{replace} tool. In our motivating example, we show five example edits.

% \item \textbf{Trajectory} ($Traj$) - LLM-based agents typically detail all their interactions with the environment $Env$ in the form of a ``trajectory'' ($Traj$). This trajectory encompasses all the actions of the agent and the observations it receives during the course of implementing task $T$. Hence, $Traj$ can be viewed as an ordered list of actions and observations spanning the entire duration of the trajectory - $[A_{0}, Obs_{0}, A_{1}, Obs_{1}, ..., A_{N}, Obs_{N}]$. We show a compacted version of a trajectory in Figure \ref{fig:agent_traj}.

% \item \textbf{Agent Patch as Edits} ($\mathcal{APE}$) \& \textbf{Minimized Patch as Edits} ($\mathcal{MPE}$) - In later sections, we use a different notation ($\mathcal{APE}$) for an agent's patch, which makes explicit the causal relationship between the edits $E$ made during $Traj$ and the final agent patch. More specifically, $\mathcal{APE} = [E_1, E_2, E_3,...,E_N]$ where $E_1$ to $E_N$ are the agent's edits made during $Traj$. Thus, with this definition, the corresponding minimized patch ($\mathcal{MPE}$) is the subset of edits in $\mathcal{APE}$. A concrete example of $\mathcal{MPE}$ is $[E_1, E_5, ..., E_{N-2}, E_{N}]$, which is a subset of the original list $[E_1, E_2, E_3,...,E_N]$. To convert from the ``edits" representation to the ``patch" representation, we use the ``$\operatorname{apply}()$" operator. For example, $\mathcal{AP} = \operatorname{apply}(\mathcal{APE})$. In our motivating example, $\mathcal{APE} = [E_{11}, E_{21}, E_{31}, E_{32}, E_{33} ]$ and $\mathcal{MPE} = [E_{31}]$.

% \item \textbf{Patch Length} - We define a function operator ``$\operatorname{len}$'' (applicable to both representations i.e. $\mathcal{AP}$ and $\mathcal{APE}$), that returns what we term as the ``patch length".  
%We refer to the final state of the environment's filesystem at the end of $Traj$ as $\mathcal{AP}$ - i.e., the agent patch. While $\mathcal{AP}$ (like any generic patch) can be compactly described using \texttt{git diff}, in this paper, we sometimes refer to the agent patch as a list of edits. This notation makes explicit that the final patch is the cumulative effect of many agent edits ($ \mathcal{AP} = \operatorname{Apply}([E_1, E_2, E_3,...,E_N])$) issued during $Traj$. Thus, we define a function operator ``$\operatorname{len}$'' (applicable to both representations) that returns what we term as the ``patch length". 
% For the $\mathcal{AP}$ representation, ``$\operatorname{len}(\mathcal{AP})$'' computes the patch length by summing up the total number of added and deleted lines. For the $\mathcal{APE}$ representation, ``$\operatorname{len}(\mathcal{APE})$'' first applies all the edits in the list and then computes the total number of added and deleted lines.
% \shobini{Alex, this part is well defined how we get from $Traj \to AP$, but what can be more clearly defined : $Traj \to E$: edit actions are subsequence of traj (this is implicit when we describe what an edit is). but more importantly, $E \to AP$ and $ E \to AP_i$. I think this would make $\mathcal{AP}_i \subseteq \mathcal{AP}$ make more sense} 
% \alex{Shobini, how is it now?} \petros{I don't think it's an improvement. AP is the same, whether you consider edits that have been applied or a single giant edit. Perhaps you mean that AP is about the one giant patch at the end, but $AP_i$ is the patch for an $Edit_i$? If I understand your point here, you're trying to make a distinction about the one true patch at the end of a trajectory, and a sequence of patching induced by individual edit actions. Spelling this out might help.}
% \alex{Shobini and Petros, please see the new sections for agent patch, agent patch as edits, and patch length. I think it covers all the feedback. Please let me know if you still think something is missing.}
% \item \textbf{Task Success} - We denote that a task $T$ has been successfully completed by the agent, if after applying its patch ($\mathcal{AP}$) to the environment (i.e. $Env_{\mathcal{AP}}$), the hidden oracle ($O$) passes. Thus when $Env_{\mathcal{AP}}(O) = \{pass\}$, $\mathcal{AP}$ successfully implements $T$. It is ideal if the minimized patch \minp has the same outcome as \agentp. So if $Env_{\mathcal{AP}}(O)=\{pass\}$, so also must \minp (i.e. $Env_{\mathcal{MP}}(O)=\{pass\}$). If \minp causes oracle regressions, then the minimization has introduced a loss in intended functionality.
% \end{itemize}




\begin{table*}[t]
    \centering
    \scriptsize
    % \footnotesize
    \caption{Definitions of Terminologies used in the formulation of \aislop and in \algo.}
    \label{tab:defnitions}
    \renewcommand{\arraystretch}{0.95}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|p{0.85\linewidth}}
    \toprule
\makecell[tl]{
    \textbf{User Instruction} \\ 
    ($\mathcal{UI}$) \\
    \textbf{Task} ($T$)
    } & Users often provide natural language instructions ($\mathcal{UI}$) to LLM-based agents that concretely define a task ($T$) for the agent to implement, such as bug fixing, feature implementation, test generation, etc. In our motivating example (Figures \ref{fig:agent_traj} and \ref{fig:motiv_fig}), $T$ is the task to resolve the Linux Vulnerability and $\mathcal{UI}$ is the instructions associated with this task. \\
         \midrule
\makecell[tl]{
    \textbf{Agent Patch} \\ 
    (\agentp), \\
    \textbf{Minimized Patch} \\ 
    (\minp)
    } & We term the final patch that an agent submits for a task $T$ as the agent patch (\agentp). In this work, we represent \agentp as the set of all of the modified (added and deleted) lines in the patch. As explained in previous sections, our main aim is to derive a minimized patch (\minp), which is a subset of \agentp, where ``subset" implies that the lines in \minp are a subset of the lines in \agentp (i.e. \minp $\subseteq$ \agentp). In our motivating example, $\mathcal{AP}$ is the entire patch seen in Figure \ref{fig:motiv_fig}, and $\mathcal{MP}$ is the box with the ``$\star$" containing three modified lines. \\
\midrule
\makecell[tl]{
    \textbf{Hidden Oracles} \\ 
    ($O$) 
} & 
An oracle ($O$) for task $T$ is its ultimate judge of success. $O$ is used to generate the final success/failure verdict for every agent-generated patch. For some tasks like crash resolution in the Linux kernel \cite{mathai2024kgym}, $O$ is provided as part of the crash metadata. For other tasks like Github issue resolution \cite{deng2025swe}, $O$ is often a hidden fail-to-pass ($F2P$) test used for final benchmark evaluation. As $O$ is often hidden from the agent, it is also kept hidden from our minimization algorithm. However, it is ideal if our predicted minimized patch \minp satisfies $O$ if \agentp initially satisfied $O$. Thus, \textbf{minimization must not introduce any oracle regressions}. \alex{Shobini and Petros, how is this now?}
\\ \midrule
\makecell[tl]{\textbf{Environments} \\ 
    ($Env$), \\
    \textbf{Observations} \\ 
    ($Obs$), \\
    \textbf{Test Files} \\ 
    ($TF$), \\
    \textbf{Feedback} \\
    \textbf{Requests} ($FR$)
    } & When implementing a task $T$, LLM-based agents interact with their executable environments ($Env$) by issuing feedback requests ($FR$). A $FR$ is typically a bash command that invokes one (or many) test files ($TF$) that agents leverage ``mid-trajectory" as functional guardrails. For crash resolution in the Linux kernel \cite{mathai2024kgym}, the benchmark provides a fixed $TF$. For Github issue resolution \cite{deng2025swe}, ``\textit{during}'' the trajectory, the agent creates and executes many $TF$, to test each part of its implementation thoroughly.  Depending on the task, the $TF$ can remain static (or evolve) during the course of the agent's trajectory. When running these $TF$, the agent receives observations ($Obs$) such as (i) runtime feedback measuring functional correctness ($Env_{\mathcal{AP}}(TF)$), or (ii) compilation feedback like whether a patch compiles. This fine-grained feedback enables agents to course-correct mid-trajectory. Typically, the agent patch \agentp satisfies multiple $TF$ by the end of the trajectory, i.e., $Env_{\mathcal{AP}}(TF) =\{pass\}$. In our motivating example, the VM machine is the $Env$, the \texttt{PASS}/\texttt{FAIL} outcomes are the $ Obs$, and $FR$ is the set of ``feedback request" lines from the agent to the VM machine.
\\ \midrule
    \textbf{Edits} ($E$) & To generate code that implements the task $T$, LLM-based agents make changes to their environment's filesystem by issuing ``edit'' actions. The exact realization of an ``edit'' depends on the specific agentic harness - for \mini \cite{yang2024swe} it is typically an \textit{sed} call, for \swe \cite{yang2024swe} and \openhands \cite{wang2024openhands} it is a call to the \textit{str\_replace\_editor} tool, and for \crashfixer \cite{mathai2025crashfixer} it is an invocation to the \textit{replace} tool. In our motivating example, we show five example edits.
\\ \midrule
\makecell[tl]{
   \textbf{Trajectory} \\ 
   ($Traj$) 
}& LLM-based agents typically detail all their interactions with the environment $Env$ in the form of a ``trajectory'' ($Traj$). This trajectory encompasses all the actions of the agent and the observations it receives during the course of implementing task $T$. Hence, $Traj$ can be viewed as an ordered list of actions and observations spanning the entire duration of the trajectory - $[A_{0}, Obs_{0}, A_{1}, Obs_{1}, ..., A_{N}, Obs_{N}]$. We show a compacted version of a trajectory in Figure \ref{fig:agent_traj}. \\ \midrule
\makecell[tl]{
   \textbf{Agent Patch} \\
   \textbf{as Edits} ($\mathcal{APE}$), \\ 
   \textbf{Minimized Patch} \\
   \textbf{as Edits} ($\mathcal{MPE}$)
}& In later sections, we use a different notation ($\mathcal{APE}$) for an agent's patch, which makes explicit the causal relationship between the edits $E$ made during $Traj$ and the final agent patch. More specifically, $\mathcal{APE} = [E_1, E_2, E_3,...,E_N]$ where $E_1$ to $E_N$ are the agent's edits made during $Traj$. Thus, with this definition, the corresponding minimized patch ($\mathcal{MPE}$) is the subset of edits in $\mathcal{APE}$. A concrete example of $\mathcal{MPE}$ is $[E_1, E_5, ..., E_{N-2}, E_{N}]$, which is a subset of the original list $[E_1, E_2, E_3,...,E_N]$. To convert from the ``edits" representation to the ``patch" representation, we use the ``$\operatorname{apply}()$" operator. For example, $\mathcal{AP} = \operatorname{apply}(\mathcal{APE})$. In our motivating example, $\mathcal{APE} = [E_{11}, E_{21}, E_{31}, E_{32}, E_{33} ]$ and $\mathcal{MPE} = [E_{31}]$. \\ \midrule
\makecell[tl]{
   \textbf{Patch Length}
} & We define a function operator ``$\operatorname{len}$'' (applicable to both representations i.e. $\mathcal{AP}$ and $\mathcal{APE}$), that returns what we term as the ``patch length". For the $\mathcal{AP}$ representation, ``$\operatorname{len}(\mathcal{AP})$'' computes the patch length by summing up the total number of added and deleted lines. For the $\mathcal{APE}$ representation, ``$\operatorname{len}(\mathcal{APE})$'' first applies all the edits in the list and then computes the total number of added and deleted lines. \alex{Shobini and Petros, please see the new sections for agent patch, agent patch as edits, and patch length. I think it covers all the feedback. Please let me know if you still think something is missing.} \\ \midrule
\makecell[tl]{
   \textbf{Task Success}
} & We denote that a task $T$ has been successfully completed by the agent, if after applying its patch ($\mathcal{AP}$) to the environment (i.e. $Env_{\mathcal{AP}}$), the hidden oracle ($O$) passes. Thus when $Env_{\mathcal{AP}}(O) = \{pass\}$, $\mathcal{AP}$ successfully implements $T$. It is ideal if the minimized patch \minp has the same outcome as \agentp. So if $Env_{\mathcal{AP}}(O)=\{pass\}$, so also must \minp (i.e. $Env_{\mathcal{MP}}(O)=\{pass\}$). If \minp causes oracle regressions, then the minimization has introduced a loss in intended functionality. \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}


